A Decision Procedure for Guarded Separation Logic: Complete Entailment Checking for Separation Logic with Inductive Definitions

We develop a doubly-exponential decision procedure for the satisfiability problem of guarded separation logic -- a novel fragment of separation logic featuring user-supplied inductive predicates, Boolean connectives, and separating connectives, including restricted (guarded) versions of negation, magic wand, and septraction. Moreover, we show that dropping the guards for any of the above connectives leads to an undecidable fragment. We further apply our decision procedure to reason about entailments in the popular symbolic heap fragment of separation logic. In particular, we obtain a doubly-exponential decision procedure for entailments between (quantifier-free) symbolic heaps with inductive predicate definitions of bounded treewidth (SLIDbtw) - one of the most expressive decidable fragments of separation logic. Together with the recently shown 2ExpTime-hardness for entailments in said fragment, we conclude that the entailment problem for SLIDbtw is 2ExpTime-complete - thereby closing a previously open complexity gap.

==> ArticleConclusion.tex <==
\section{Conclusion}\label{ch:article-conclusion}
\cmtodo{ToDo: Overhaul}
We presented a completely revised, extended version of the entailment-checking procedure for the bounded-treewidth (BTW) fragment of
SL that we proposed in~\cite{katelaan2019effective}.
In particular, we have fixed the incompleteness issues of \cite{katelaan2019effective}, 
while extending the result beyond symbolic heaps and retaining the same asymptotic complexity as in \cite{katelaan2019effective}.
To this end, we generalized the \emph{$\Sid$-profile} abstraction of \cite{katelaan2019effective} to the \emph{$\Sid$-type} abstraction by adding (limited) support for existential quantifiers
(see \cref{ch:types}).
We then used $\Sid$-types to develop a
sound and complete, double-exponential decision procedure for guarded separation logic over the bounded-treewidth fragment of separation
logic (\cref{ch:deciding-btw}).


\paragraph*{Stack--heap semantics.} We used the standard stack--heap
model of separation logic instead of the heap-graph model used in
\cite{katelaan2019effective}.
%
This allowed us to drop several simplifying assumptions; in
particular, our new approach can handle pure formulas, parameter
repetitions, and SIDs that admit unsatisfiable unfoldings.

\paragraph*{Entailment checking for positive formulas.} In
\cite{katelaan2019effective}, we only addressed entailment checking
between pairs of predicate calls.
%
In the present article,
we showed that the type
abstraction refines the satisfaction relation for a larger class of
separation-logic formulas
(\cref{sec:deciding-btw:types-capture-sat}).
%
This insight allowed us to beyond predicate calls and even beyond the
symbolic-heap fragment, allowing conjunction, disjunction, and guarded
forms of negation, septraction and the magic wand in addition to the
separating conjunction (\cref{sec:deciding-btw:toplevel-types}).
%
We thus obtained the first decision procedure for a separation logic
that combines user-defined inductive definitions, Boolean structure
and some uses of the magic wand.

\paragraph*{In summary,} we fixed the incompleteness issues of
\cite{katelaan2019effective}, switched to the standard stack--heap
model of separation logic, and extended the decision procedure to
positive separation-logic formulas.

% TODO: Describe extensions / future work?
% - relaxing BTW assumptions to capture MSO
% - allowing true, at least for unambiguous SIDs?
% - switching to strong-separation semantics and allowing magic wand and negation
% - limited support for (orthogonal) data constraints?

\subsection{Discussion}

We now have a good picture of the decidability landscape for
separation logics built on top of $\IDbtw$ SIDs:
%
\begin{itemize}
\item As we saw in \cref{ch:deciding-btw}, we can decide
  $\SLIDguarded$, in which any combination of the operators $\sep$, $\wedge$
  and $\vee$ and guarded occurrences of the operators
  $\neg$, $\mw$, and $\sept$ are allowed.
%
\item As we saw in \cref{sec:unguarded-undec}, all extensions of
  $\SLIDguarded$ in which one of the guards
  is removed are undecidable.
\end{itemize}
%
It is, of course, also conceivable to remove some of operators from
$\SLIDguarded$ prior to removing the guards.
%
I did this to some extent for all of the undecidability proofs in
\cref{sec:unguarded-undec}, but leave open the question whether there
are restrictions of $\SLop{\wedge,\sep,\true}$,
$\SLop{\wedge,\sep,\neg}$ and $\SLop{\wedge,\sep,\mw}$ that remain
undecidable.

\paragraph*{Decidability and dangling pointers.} What is the
fundamental difference between the logics studied in
\cref{sec:unguarded-undec} and the guarded separation logic
$\SLIDguarded$ that explains the undecidability of the former and the
decidability of the latter?

If you examine the undecidability proofs, you will see that all of
them rely on the possibility to decompose the heap into parts
with unboundedly many dangling pointers. Specifically, by splitting
the CFG encoding into the ``non-word'' part of the derivation and the
induced word $w$ introduces $\size{w}$ dangling pointers.

Conversely, the number of dangling pointers in the models of
$\SLIDguarded$ formulas is always bounded by the number of free
variables of the formula---a simple consequence of
\cref{lem:btw:pos-non-dangling}.

I conjecture that generalizations of $\SLIDbtw$ that retain this
property remain decidable. Such generalizations would still
have the property that all models have bounded treewidth.
%
Other interesting questions include: Is it possible to change the
restrictions of the $\SLIDbtw$ fragment to capture exactly all
MSO-definable models of bounded treewidth? And are there, perhaps,
even decidable SLs that admit models of unbounded treewidth? Both of
these questions remain open at the time of writing.

% Finally, it would be interesting to try and integrate the results of
% \cref{pt:ssl,pt:btw}, i.e., to investigate whether we can remove the
% guardedness restrictions if we assume strong-separation semantics.
% %
% This is not as trivial as adding the ``garbage components'' of the AMS
% abstraction to the $\Sid$-type abstraction, because there is, in
% general, no unique way to split a model of an $\IDbtw$ predicate into
% positive chunks and negative chunks (as defined in
% \cref{pt:ssl}).

\paragraph*{Strong-separation semantics.}
%  I do not know if
% \cref{cor:undec-mw,cor:undec-neg} can be strengthened to fewer
% operators. I would not be surprised if that is possible, but do not
% attempt a proof here.

Another research direction would be to give $\sep$ the
strong-separation semantics from \cref{pt:ssl} and investigate whether
we can remove the guardedness restrictions under this semantics.
%
This would rule out the introduction of an unbounded number of
dangling pointers and thus invalidate the undecidability proofs from
\cref{sec:unguarded-undec}. It makes sense to try and adapt the
``garbage-chunk'' idea from \cref{pt:ssl}, but because of the possible
ambiguity in the SIDs in $\IDbtw$, there is \emph{no} analog of
decomposing the ``non-garbage part'' of the model in a unique way,
i.e., no unique way to split a model into positive chunks and negative
chunks.

% \begin{example}
%    \TODO{Add example of ambiguous SID that does not admit a unique split.}
% \end{example}

\paragraph*{Data constraints.} In my opinion, the most interesting
type of extension would be to add some way to combine the shape
constraints imposed by the $\IDbtw$ predicates with data constraints.
%
Not much is known about the decidability of SLs that combine
user-defined predicates with data constraints; see \cref{ch:related-work}.
%
One approach would be to augment $\IDbtw$ predicates with a variant of
the data constraints from \cref{pt:ssl}. I refrain from speculating
about the decidability status of such an extension.

% This could be done with data
% predicates, like the ones we used in \cref{pt:ssl}, or by allowing
% some limited form of data constraints in the inductive definitions
% themselves, as has been done by other research groups.
%
% \TODO{Cite madhusudan, qiu, the Singapore guys with their SAT CAV
%   paper(s), the list-with-data paper(s) e.g. at ATVA. Also refer
%   to related work section.}
% %
% Overall,
% %
% I will refrain from conjecturing the

%
% I have no idea whether entailment in the symbolic-heap fragment or
% guarded fragment of $\SLIDqf$ any extension of the full
% $\SLIDbtw$ logic with data constraints would be decidable.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Journal"
%%% End:


==> ArticleIntro.tex <==
\section{Introduction}\label{ch:intro}
\cmtodo{ToDo: Overhaul}

In our recent work \cite{katelaan2019effective}, we proposed a new
decision procedure for solving the entailment problem for
symbolic-heap separation logic with user-defined inductive definitions
from the bounded-treewidth fragment (BTW fragment) as introduced
in~\cite{iosif2013tree}.
%
The original decision procedure for the BTW fragment
in~\cite{iosif2013tree} relied on a reduction to monadic second-order
logic (MSO) over graphs of bounded treewidth, yielding a decision
procedure that was of elementary complexity but impractical.
%
In \cite{katelaan2019effective}, we instead solved the entailment problem
directly, without a reduction to MSO. We proved a double-exponential
upper bound for our procedure.
%
Our decision procedure was based on a novel abstract domain called
\emph{profiles}.
%
We claimed that profile-based entailment checking is a sound and
complete decision procedure for the BTW fragment.
%
Unfortunately, the decision procedure we proposed
in~\cite{katelaan2019effective} is, in fact, incomplete.

In this article, we develop an extension of the profile abstraction we
call the \emph{type abstraction}.
%
The type abstraction extends the profile abstraction with (limited)
support for existential quantifiers.
%
We prove that by computing types rather than profiles, we obtain a
sound and complete decision procedure for the BTW fragment while
retaining the double-exponential complexity bound.
%
Moreover, we drop several simplifying assumptions made in
\cite{katelaan2019effective}:
\begin{enumerate}
\item We use the standard \emph{stack--heap model} of separation logic
  instead of the non-standard heap-graph model used
  in~\cite{katelaan2019effective}. This allows us to deal with
  \emph{aliasing} between stack variables, which we ignored in
  \cite{katelaan2019effective}. It also allows us to reason more
  explicitly about the assumptions of the BTW fragment, in particular
  about \emph{establishment}.
\item We allow \emph{equalities and disequalities} both in the
  inductive data-structure definitions and in the entailment queries.
\item We allow \emph{parameter repetitions} in predicate calls.
\item We drop the assumption that all ``unfoldings'' of all inductive
  predicates are \emph{satisfiable}.
\end{enumerate}

Furthermore, we go beyond the symbolic-heap fragment and consider
\emph{positive quantifier-free separation logic}, in which formulas
are built using the separating conjunction, classical conjunctions,
classical disjunctions, and guarded occurrences of
negation,\footnote{As far as we know, guarded negation has not been
  studied in the context of separation logic; see
  e.g.~\cite{barany2015guarded} for guarded negation in first-order
  logic.} the magic wand, and septraction (see
e.g.~\cite{brochenin2012almighty}).

The technical development in this article is self contained.
%
For a systematic discussion of related work and an informal motivation
of the proof approach, we refer the interested reader to \cite{katelaan2019effective}.

\paragraph*{Outline.}

In \cref{ch:seplog}, we introduce separation logic and its
bounded-treewidth fragment. It is worth reading this chapter even if
you are an expert, as we use a slightly non-standard semantics
(\cref{sec:sid:semantics}) and prove some properties of the BTW fragment
that are essential for the technical development later in the article
(\cref{sec:sid:dangling}).

\cref{ch:types} introduces the $\Sid$-type abstraction, based on a
variant of \emph{unfolding trees} of inductive predicates and their
projection onto formulas. Roughly, every model is abstracted by the
set of formulas that can be obtained as projections of a certain set
of forests that correspond to (partial) unfoldings of inductive predicates.

In \cref{ch:deciding-btw}, we show that it is possible to compute the
types of the models of any positive separation-logic formula. Once we
have this result, it is straightforward to obtain a decision procedure
for satisfiability and entailment.

We conclude in \cref{ch:article-conclusion}.

\paragraph*{Changes w.r.t.~the previous version of this article.} In
the first version of this article, we erroneously claimed that the
$\Sid$-type abstraction can be used to decide formulas with arbitrary
(as opposed to guarded) occurrences of the septraction operator. This
is not the case.

Moreover, we changed the projection functions in \cref{ch:types} to
use guarded quantifiers, which is necessary to correctly handle pure
constraints with the $\Sid$-type abstraction.

We have also simplified and reordered parts of the article to improve
readability.

\paragraph*{Acknowledgments.} 
We thank Mnacho Echenim, Radu Iosif, and
Nicolas Peltier for their outstandingly thorough study of our
paper~\cite{katelaan2019effective} and their help in discovering the
incompleteness issues in the aforementioned paper.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Journal"
%%% End:


==> Journal/app-projection-composition.tex <==
\subsection{Old material about composition of forests and projections}



\begin{example}[Composing
  projections]\label{ex:pcompose-motivating-example}
  %
  To illustrate the main steps of composing projections,
  we consider three $\Sid$ forests
  with
  We illustrate the additional steps when composing forest projections
  for three $\Sid$-forests $\frst_1$, $\frst_2$, and $\frst_3$
  with $\frst_1 \funion \frst_2 \fderivestar \frst_0$.
  To this end, recall from \cref{ex:types:forest}
  the SID $\Sid$ and the trees $\ftree_1,\ftree_2,\ftree_3$.
  We set $\frst_1 \defn \set{\ftree_1,\ftree_2}$ and
  $\frst_2 \defn \set{\ftree_3}$.
  Moreover, consider the states
  $\SHi{1}$ and $\SHi{2}$ below, which are also depicted in
  \cref{fig:types:cex:f1,fig:types:cex:f2} on p.~\pageref{fig:types:cex}.
  \begin{align*}
    & \S = \set{x_1 \mapsto l_1, x_2 \mapsto l_2, x_3 \mapsto l_3},\\
    %
    & \H_1 \defn \set{l_1 \mapsto \tuple{l_4,l_3}, l_2\mapsto l_4, l_4
    \mapsto l_2}, \text{ and}\\
    %
    &\H_2 \defn \set{l_3 \mapsto l_2}.
    %
  \end{align*}
  Note that $\H_1 = \fheapof{\frst_1}$ and $\H_2 = \fheapof{\frst_2}$.
  The third forest is $\frst_0 \defn \set{\ftree_0}$, where the $\Sid$-tree $\ftree_0$ is
  given by
  \begin{align*}
    \ftree_0 = \{ &
%
   l_1 \mapsto \big\langle\tuple{l_4,l_3}, \PredName{p_1}(l_1,l_2,l_3)
      %\phantom{l_1 \mapsto\big\langle\tuple{l_4,l_3},}
                      \Rule
                      \ppto{l_1}{\tuple{l_4, l_3}} \sep
                      \PredName{ptr}(l_4, l_2) \sep
                      \PredName{p_2}(l_3, l_2, l_4)\big\rangle, \\
  %
& l_2 \mapsto \tuple{\emptyset, \PredName{ptr}(l_2,l_4)
      \Rule \pto{l_2}{l_4}},\\
%
& l_3 \mapsto \tuple{l_2, \PredName{p_2}(l_3,l_2,l_4)
    \Rule \ppto{l_3}{l_2} \sep \PredName{ptr}(l_2, l_4)}, \\
    & l_4 \mapsto \tuple{\emptyset, \PredName{ptr}(l_4,l_2) \Rule
    \pto{l_4}{l_2}} \}
  \end{align*}
  %
  Since indeed $\frst_1 \funion \frst_2 \fderivestar \frst_0$,
  our desired composition operation $\PCompose$ should satisfy
  \[
    \sfproj{\S}{\frst_0} \in \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2},
  \]
  where the involved projections are as follows:
  %
  \begin{align*}
& \sfproj{\S}{\frst_0} = \emp
                   \mw \PredName{p_1}(x_1,x_2,x_3),\\
                   %
    &\sfproj{\S}{\frst_1} = \EEX{e_1} (\PredName{p_2}(x_3, x_2, e_1) \mw
      \PredName{p_1}(x_1,x_2,x_3)) \sep
    (\emp\mw\PredName{ptr}(x_2,e_1)), \\
    %
    &\sfproj{\S}{\frst_2} = \FFA{a_1}\PredName{ptr}(x_2,a_1) \mw \PredName{p_2}(x_3,x_2,a_1).
  \end{align*}
  %
  To this end, we execute the following two steps.
  \begin{description}
    \item[Re-scoping.] We push the existential $\eexists e_1$ out using the operation
    $\rescopeOP$, in the process
    instantiating the universally quantified variable $a_1$ with $e_1$:
    \begin{align*}
      \phi ~\defn~ &\EEX{e_1} (\PredName{p_2}(x_3, x_2, e_1) \mw
      \PredName{p_1}(x_1,x_2,x_3))
      %\\&\qquad
      \sep
    (\emp\mw\PredName{ptr}(x_2,e_1))
      %\\&\qquad\sep
      (\PredName{ptr}(x_2,e_1) \mw \PredName{p_2}(x_3,x_2,e_1))
      \\
      %
      ~\in~ &(\EEX{e_1} (\PredName{p_2}(x_3, x_2, e_1) \mw
      \PredName{p_1}(x_1,x_2,x_3))
      %\\&\qquad
      \sep
    (\emp\mw\PredName{ptr}(x_2,e_1)))
      %\\&\;
      \rescopeOP\; (\FFA{a_1}\PredName{ptr}(x_2,a_1) \mw \PredName{p_2}(x_3,x_2,a_1)).
    \end{align*}
  %
  \item[Merge steps.] We apply the modus-ponens variant,
    \cref{lem:gmp}, twice to subformulas of the re-scoped formula
    $\phi$; each of these applications is denoted by \gls{--derive-pderive}:
  \begin{align*}
    \phi ~\deriveqf~ & \EEX{e_1} (\PredName{p_2}(x_3, x_2, e_1) \mw
      \PredName{p_1}(x_1,x_2,x_3)) %\\&\phantom{\EEX{e_1} (}\;
      \sep
                (\emp\mw\PredName{p_2}(x_3,x_2, e_1)) \\
    ~\deriveqf~ & \emp
                   \mw \PredName{p_1}(x_1,x_2,x_3) ~=~ \sfproj{\S}{\frst_0}.
  \end{align*}
  \end{description}


  %
  Assume we define the operation $\PCompose$ as re-scoping $\rescopeOP$
  followed by arbitrarily many merge steps:
  %
  \begin{align*}
    \phi_1 \PCompose \phi_2 \defn \{\phi \mid & \text{there exist a
                                             $k\geq1$ and
                                             $\zeta_1,\ldots,\zeta_k$}
                                             \\ &\text{s.t.~$\zeta_1$ is a re-scoping of $\phi_1$ and $\phi_2$,}
                                             \text{ $\zeta_i \deriveqf \zeta_{i+1}$ for all $1 \leq i < k$, and $\zeta_k
                                                  = \phi$}\}.
  \end{align*}
  %
  Then, as desired, we obtain
    $\sfproj{\S}{\frst_0} \in \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2}$.
\end{example}

\noindent
Formalizing the operations $\rescopeOP$ and $\deriveqf$ is technically involved, but does not contain any deep insights that are relevant for the development of our decision procedure.
In the remainder of this section, we thus only summarize the key properties; a precise formalization as well as proofs of said properties are found in \cref{app:projection-composition}.
First, we remark that we can construct suitable operators $\rescopeOP$ and $\deriveqf$:
%
\begin{lemma}[Existence of re-scoping operation $\rescopeOP$]\label{lem:ex:rescoping:sound}
   There exists a re-scoping operation $\rescopeOP$ such that, for all
   stacks $\S$ and $\Sid$-forests $\frst_1,\frst_2$ with
   $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$, we have
   \[
        \phi \in \rescope{\sfproj{\S}{\frst_1}\,}{\,\sfproj{\S}{\frst_2}}
        \quad\text{implies}\quad
        \sfproj{\S}{\frst_1} \sep \sfproj{\S}{\frst_2} \sidmodels \phi.
   \]
\end{lemma}
%
\begin{lemma}[Existence of merge operation $\deriveqf$]\label{lem:ex:deriveqf:sound}
   There exists a merge operation $\deriveqf$ such that, for all
   stacks $\S$, $\Sid$-forests $\frst$, and $\phi \in \USH{\Sid}$, we have
   \[
     \sfproj{\S}{\frst} \deriveqf \phi
     \quad\text{implies}\quad
     \sfproj{\S}{\frst} \sidmodels \phi.
   \]
\end{lemma}
%
Based on the above two operations, we then compose forest projections as defined below.
%
\begin{definition}[Projection composition]\label{def:pcompose-old}
  For a stack $\S$ and $\Sid$-forests $\frst_1, \frst_2$, we define
  \[
      \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
      \defn
      \{ \phi \mid \zeta \derivestar \phi ~\text{for some}~\zeta \in \rescope{\sfproj{\S}{\frst_1}}{\sfproj{\S}{\frst_2}}.
  \]
  % Let $\phi_1,\phi_2\in\USH{\Sid}$.
\end{definition}
%
\begin{corollary}[Soundness of $\PCompose$]\label{lem:pcompose:sound}
  Let $\S$ be a stack and let $\frst_1,\frst_2$ be $\Sid$-forests
  such that
  $\frst_1\funion\frst_2\neq\bot$ and
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$.
  Then
  \[
    \psi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
    \quad\text{implies}\quad
    \sfproj{\S}{\frst_1} \sep \sfproj{\S}{\frst_2}\sidmodels \psi.
  \]
\end{corollary}
\begin{proof}
  Follows immediately from \cref{lem:ex:rescoping:sound,lem:ex:deriveqf:sound}
  and transitivity of implication.
\end{proof}
%
\subsubsection{Relating Forest Composition and Projection Composition}\label{sec:composing:correctness}
%
Recall our design goal that the projection function $\sfproj{\S}{\cdot}$
should be a homomorphism from forests and forest composition $\FCompose$ (\cref{def:forest-composition}) to projections
and projection composition $\PCompose$, i.e.,
\begin{align*}
  \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2} \overset{?}{=}
  \set{\sfproj{\S}{\frst} \mid \frst \in \frst_1 \FCompose \frst_2}. %\tag*{\tagA}
\end{align*}
%
\noindent
%
In one direction, our composition defined in \cref{def:pcompose} achieves this (cf. \cref{app:fcompose-to-pcompose}):
%
\begin{lemma}\label{cor:fcompose-to-pcompose}
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$, we have
  \[
    \frst \in \frst_1\FCompose\frst_2
    \quad\text{implies}\quad
    \sfproj{\S}{\frst} \in \sfproj{\S}{\frst_1} \PCompose
    \sfproj{\S}{\frst_2}.
  \]
\end{lemma}
%
\noindent
Unfortunately, as demonstrated below, the homomorphism breaks in the other direction:
%
\begin{example}[Projection is not homomorphic]\label{ex:proj-no-homo}
  Consider the $\Sid$-forests $\frst_2$ and $\frst_2$ given by:
  \begin{align*}
    & \ftree_1 \defn \set{l_1 \mapsto \tuple{\emptyset, (\odd(l_1,m_1)
      \Rule \ppto{l_1}{l_2} \sep \even(l_2,m_1)) }} \\
    %
    & \ftree_2 \defn \set{l_2 \mapsto \tuple{\emptyset, (\even(l_2,m_2)
      \Rule \ppto{l_2}{l_3} \sep \odd(l_3,m_2)) }}\\
  %
    & \frst_1 \defn \set{\ftree_1}, \frst_2\defn \set{\ftree_2} \\
    %
    & \S \defn \set{x_1 \mapsto l_1, x_2 \mapsto l_2, x_3 \mapsto l_3}
  \end{align*}
  %
  The corresponding projections are
  %
  \begin{align*}
    & \sfproj{\S}{\frst_1} = \FFA{a_1} \even(x_2,a_1) \mw
      \odd(x_1,a_1),~\text{and} \\
      %
    & \sfproj{\S}{\frst_2} = \FFA{a_1} \odd(x_3,a_1) \mw
      \even(x_2,a_1).
  \end{align*}
  Moreover, we have
  \begin{align*}
    & \FFA{a_1} \odd(x_3,a_1) \mw \odd(x_1,a_1) \in \sfproj{\S}{\frst_1}
    \PCompose \sfproj{\S}{\frst_2}.
  \end{align*}
  %
  However, since different locations, namely $m_1$ and $m_2$, are unused in the two forests,
  there is only one forest in $\frst_1 \FCompose \frst_2$:
  $\set{\ftree_1,\ftree_2}$. It is not possible to merge the trees, because the hole predicate of the first tree,
  $\even(l_2,m_1)$, is different from the root of the second tree,
  $\even(l_2,m_2)$.
  %
  In particular, there does \emph{not} exist a forest $\frst$ with
  $\frst \in \frst_1\FCompose\frst_2$ and
  $\sfproj{\S}{\frst}=\FFA{a_1} \odd(x_3,a_1) \mw \odd(x_1,a_1)$.
\end{example}
%
\noindent
The essence of \cref{ex:proj-no-homo} is that while $\PCompose$ allows
renaming universals, $\FCompose$ does not allow renaming unused
locations, breaking the homomorphism.
%
To get a correspondence between the two notions of composition,  we
therefore allow renaming the
location terms in forests that do \emph{not} occur in any points-to
assertion. We capture this in the notion of \emph{$\alpha$-equivalence}.
%
\begin{definition}[$\alpha$-equivalence]\label{def:alpha-eq}\index{alpha-equivalence@$\alpha$-equivalence}
  Two $\Sid$-trees $\ftree_1,\ftree_2$ are \emph{$\alpha$-equivalent},
  denoted $\ftree_1\gls{--eq-AEQ}\ftree_2$, iff there exist locations $\vec{v_1} \in
  {(\Loc\setminus\locs{\fheapof{\ftree_1}})}^{*}$ and $\vec{v_2}\in\Loc^{*}$ such that
  \begin{align*}
    \ftree_2 = \set{ l \mapsto \tuple{\tsucc{\ftree_1}{l},
    \pinst{\truleinst{\ftree_1}{l}}{\vec{v_1}}{\vec{v_2}} \mid l \in
      \dom(\ftree_1)}},
  \end{align*}
  where the substitution is given by
  $
  \pinst{(\pred(\vec{l}) \Rule \phi)}{\vec{v_1}}{\vec{v_2}} \defn
  \pred(\pinst{\vec{l}}{\vec{v_1}}{\vec{v_2}}) \Rule
  \pinst{\phi}{\vec{v_1}}{\vec{v_2}}
  $.
  %

  Moreover, two $\Sid$-forests
$\frst_1=\ktrees,\frst_2=\set{\bartree_1,\ldots\bartree_k}$ are
\emph{$\alpha$-equivalent}, also denoted $\frst_1\AEQ\frst_2$, iff
$\ftree_i\AEQ\bartree_i$ holds for all $1 \leq i \leq k$.
\end{definition}
%
\noindent
Hence, $\frst_1 \AEQ \frst_2$ holds if the
location terms in $\frst_1$ that do \emph{not} occur in points-to
assertions can be renamed a way such that we obtain $\frst_2$.
%
Consequently, $\alpha$-equivalent forests induce the same heap.

\begin{lemma}\label{lem:aeq-same-projections}
  If $\frst_1\AEQ\frst_2$ then $\fheapof{\frst_1}=\fheapof{\frst_2}$.
\end{lemma}
\begin{proof}
  The forest $\frst_2$ differs from $\frst_1$ only in locations that are not in $\fheapof{\frst_1}$.
\end{proof}
%
\noindent
Considering forests up to $\alpha$-equivalence then yields the desired connection between forests and their projections
(cf. \cref{app:pcompose-to-fcompose} for a proof):

\begin{lemma}\label{lem:pcompose-to-fcompose}
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\frst_1\funion\frst_2\neq\bot$ and
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$,
  %
  \begin{align*}
    \phi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
    \quad\text{implies}\quad
      \exists \frst \in \bigcup_{\barfrst_1 \AEQ \frst_1, \barfrst_2 \AEQ \frst_2} \barfrst_1 \FCompose \barfrst_2 .\quad
      \phi=\sfproj{\S}{\frst}.
    %\text{ex.}~ \barfrst_1 \AEQ \frst_1,\, \barfrst_2 \AEQ \frst_2, \frst \in \barfrst_1 \FCompose \barfrst_2~\text{s.t.}~
    %\phi=\sfproj{\S}{\frst}.
  \end{align*}
\end{lemma}

\begin{theorem}\label{thm:fcompose-eq-pcompose}
  \index{homomorphism!of forest projection}
  %
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\frst_1\funion\frst_2\neq\bot$ and
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$,
\begin{align*}
  \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2} ~=~
  \set{\sfproj{\S}{\frst} \mid
  \frst \in \barfrst_1 \FCompose \barfrst_2,~
  \barfrst_1\AEQ\frst_1,~
  \barfrst_2\AEQ\frst_2
  }.
\end{align*}
\end{theorem}
\begin{proof}
  Immediate from
  \cref{cor:fcompose-to-pcompose,lem:pcompose-to-fcompose}.
\end{proof}




We now formalize the operations
$\rescopeOP$ and $\deriveqf$, and then show that the combination of both
``almost'' yields the desired composition $\PCompose$ of forest projections
motivated in \cref{sec:forests:composing}, i.e.,
\begin{align*}
  \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2} \overset{?}{=}
  \set{\sfproj{\S}{\frst} \mid \frst \in \frst_1 \FCompose \frst_2}. \tag*{\tagA}
\end{align*}
Our formalization only almost matches the above definition due to one technical issue that is
addressed in \cref{sec:composing:correctness}: we have to account for renamings of universally quantified variables.

\subsubsection{Formal Definition of Projection Composition}\label{sec:composing:formal}
%
We write
% $\euinst{\FFA{\vec{a}}\phi}{\vec{e}}{\vec{u}}{\FFA{\vec{b}}\phi'}$
$\FFA{\vec{a}}\phi \gls{--euinst} \FFA{\vec{b}}\phi'$
%
if
there exist disjoint subsets
$\bar{\vec{a}_1},\bar{\vec{a}_2}\subseteq\vec{a}$ and subsets
$\bar{\vec{u}}\subseteq\vec{u}$, $\bar{\vec{e}}\subseteq\vec{e}$ such
that
$\phi'=\pinst{\phi}{\bar{\vec{a_1}}\concat\bar{\vec{a_2}}}{\bar{\vec{u}}\concat\bar{\vec{e}}}$
and
$\vec{b}=\vec{a}\setminus (\bar{\vec{a_1}}\cup\bar{\vec{a_2}}) \cup
\bar{\vec{u}}$.

\begin{example}
  Let
  $\phi \defn \FFA{\tuple{a_1,a_2}} (\odd(y, a_2) \mw \odd(e_1, a_2)) \sep
    (\even(e_1, a_1) \mw \odd(x, a_1))$. Then:
  %
  \begin{align*}
      & \phi \xrightarrow{\eexistsSMALL e_2 / \fforallSMALL u_1} \FFA{{u_1}} (\odd(y, e_2) \mw
      \odd(e_1, e_2)) \sep (\even(e_1, u_1) \mw \odd(x, u_1)), \\
    %
      & \phi \xrightarrow{\eexistsSMALL e_2 / \fforallSMALL u_1} \FFA{{u_1}} (\odd(y, u_1) \mw
      \odd(e_1, u_1)) \sep (\even(e_1, e_2) \mw \odd(x, e_2)) ,
      \text{ and} \\
      %
      & \phi \xrightarrow{\eexistsSMALL e_2 / \fforallSMALL u_1} \FFA{{a_1}} (\odd(y, e_2) \mw
      \odd(e_1, e_2)) \sep (\even(e_1, a_1) \mw \odd(x, a_1)).
  \end{align*}
  % \begin{enumerate}
  % \item
  %   $\euinst{ \phi }{ e_2 }{u_1}{ \FFA{{u_1}} (\odd(y, e_2) \mw
  %     \odd(e_1, e_2)) \sep (\even(e_1, u_1) \mw \odd(x, u_1)) } $, but
  %   also
  % \item
  %   $\euinst{ \phi }{ e_2 }{u_1}{ \FFA{{u_1}} (\odd(y, u_1) \mw
  %     \odd(e_1, u_1)) \sep (\even(e_1, e_2) \mw \odd(x, e_2)) }$, and
  % \item
  %   $\euinst{ \phi }{ e_2 }{u_1}{ \FFA{{a_1}} (\odd(y, e_2) \mw
  %     \odd(e_1, e_2)) \sep (\even(e_1, a_1) \mw \odd(x, a_1)) }$, etc.
  % \end{enumerate}
\end{example}
\noindent
Based on this auxiliary definition, we
formalize the two ingredients of $\PCompose$:
\emph{re-scoping} and \emph{derivability}.
%
\begin{definition}[Re-scoping]\label{def:rescope}\index{re-scoping}
  %
  Let $n \in \N$ and
  $\phi_i = \EEX{\vec{e_i}}\IteratedStar_{1 \leq j \leq n}\psi_{i,j}$
    for $i \in \{1,2\}$ such that $\vec{e_1}\cap\vec{e_2}=\emptyset$.
%
  We say that $\zeta$ is a \emph{re-scoping} of $\phi_1$ and $\phi_2$,
  written $\zeta \in \rescope{\phi_1}{\phi_2}$,
  if there exist formulas $\psi'_{1,1},\ldots,\psi'_{2,n_2}$ such that
  \begin{enumerate}
      \item $\euinst{\psi_{i,j}}{\vec{e_{3-i}}}{\emptyseq}{\psi'_{i,j}}$ for
  all $i,j$, and
  \item
  $\zeta = \EEX{\vec{e_1}\concat\vec{e_2}} \IteratedStar_{1\leq j \leq
    n_1} \psi'_{1,j} \sep \IteratedStar_{1\leq j \leq n_2}
  \psi'_{2,j}$.
  \end{enumerate}
\end{definition}
%
\paragraph{Soundness of re-scoping}
The above definition yields a sound notion notion of re-scoping as required in
\cref{lem:ex:rescoping:sound}.
That is, re-scoping is sound in the following sense:

%\begin{lemma}[Soundness of re-scoping]\label{lem:rescoping:sound}
  Let $\S$ be a stack and let $\frst_1,\frst_2$ be $\Sid$-forests with
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$.
  %
  Define
  $\phi_i \defn \sfproj{\S}{\frst_i}$.
  %
  Finally, assume $\phi_3 \in \rescope{\phi_1}{\phi_2}$.
  %
  Then $\phi_1\sep\phi_2 \sidmodels \phi_3$.
%\end{lemma}
\begin{proof}
  By \cref{lem:guarded-semi-distributive}, it is sound to move the
  guarded existential quantifiers to the front.

  It remains to be shown that instantiation of guarded universals with
  guarded existentials as in \cref{def:rescope} is sound.

  Specifically, re-scoping instantiates the universals in $\phi_1$ only with
  existentials from $\phi_2$ and vice-versa.
  %
  We show the soundness of the former; the argument for the latter is
  completely analogous.

  Let
  $\SHprime \sidmodels (\EEX{\vec{e_1}}\psi_1) \sep
  (\EEX{\vec{e_2}}\psi_2)$. Then there exist models $\H'_1,\H'_2$ such
  that $\SHpair{\S}{\H'_i}\sidmodels\EEX{\vec{e_i}}\psi_i$ and
  $\H' = \H'_1 \stdunion \H'_2$.

  We have to show that the interpretation of the existentials
  $\vec{e_2}$ does not overlap with $\locs{\H_1}$, because guarded
  universals may only be instantiated with locations that don't occur
  in the model.

  Let $e \in \vec{e_2}$. By the semantics of $\eexists$, there
  then exists a location $l \in \dom(\H'_2)\setminus\img(\S)$ such that
  $\SHpair{\S}{\H_2'}\sidmodels \pinst{\psi_2}{e}{l}$.
  %
  Because $\H'_1\stdunion\H'_2\neq \bot$, it follows that $l \notin
  \dom(\H'_1)$.
  %
  Because $\SHpair{\S}{\H_1'} \in \Mpos{\Sid}$ and
  $l \notin \img(\S)$, we have by \cref{lem:btw:pos-non-dangling} that
  $l \notin \danglinglocs{\H'_1}$.
  %
  Consequently, $l \notin \locs{\H'_1}$.
  %
  It is thus sound w.r.t.~the semantics of guarded universals to
  instantiate a universal quantifier $a$ by $e$ in $\psi_1$.
\end{proof}

\cmtodo{Do we have to mention the lemma in the definition below?}
\begin{definition}[Derivability]\label{def:derive}\index{derivability!between
    projections}
  %
    The formula $\psi$ is \emph{derivable} from
  $\zeta = \EEX{\vec{e}}\IteratedStar_{1 \leq i \leq
    n}\FFA{\vec{a_i}}\zeta_i$, written $\zeta \deriveqf \psi$, iff
  there exist indices $m_1$ and $m_2$, variables
  $\vec{u_1},\vec{u_2},\vec{b_1},\vec{b_2},\vec{b}$, and formulas
  $\phi_1,\phi_2,\phi$ such that
  \begin{enumerate}
      \item $\euinst{\FFA{\vec{a_{m_i}}}\zeta_{m_i}}{\emptyseq}{\vec{u_i}}{\FFA{\vec{b}_i}\phi_i}$ for $i \in \{1,2\}$,
    \item $\phi_1 \sep \phi_2 \implies \phi$ holds via \cref{lem:gmp},
    \item $\vec{b}=(\vec{b_1}\cup\vec{b_2})\cap \fvs{\phi}$, and
    \item $\psi$ is obtained from $\zeta$ by removing the subformulas
          $\FFA{\vec{a_{m_i}}}\zeta_{m_i}$ and adding the subformula
          $\FFA{\vec{b}} \phi$.
  \end{enumerate}


  We write $\gls{--derive-pderivestar}$ for the reflexive--transitive
closure of $\deriveqf$.
\end{definition}

\paragraph{Soundness of $\deriveqf$}
As for re-scoping, the above definition yields a sound notion of derivability in the sense of
\cref{lem:ex:deriveqf:sound}.
Formally,
%\begin{lemma}[Soundness of $\deriveqf$]\label{lem:deriveqf:sound}
  % Let $\phi_1,\phi_2\in\USH{\Sid}$
  let $\phi_1,\phi_2$ be such that $\phi_1=\sfproj{\S}{\frst}$ for
  some choice of $\S$, $\frst$ and such that
  $\phi_1\deriveqf\phi_2$. Then $\phi_1\sidmodels\phi_2$.
  %
  % \TODO{This is the first use of the $\USH{\Sid}$ macro. If we avoid
  %   this here, we could defer the definition of the fragment to the
  %   next chapter?}
%\end{lemma}
\begin{proof}[Proof sketch]
  Because of the soundness of the modus-ponens variant used in
  $\deriveqf$, \cref{lem:gmp}, it suffices to show that the
  instantiation
  %
  \[\euinst{\FFA{\vec{a_{m_i}}}\zeta_{m_i}}{\emptyseq}{\vec{u_i}}{\FFA{\vec{b_i}}\phi_i}, \tag*{\tagB}\]
  %
  carried out to obtain matching predicate calls prior to applying
  \cref{lem:gmp}, is sound.
%
  Since we only rename guarded universals to other guarded universals,
  this follows immediately from the injectivity of the instantiation
  carried out by \tagB{}: every variable among $\vec{u_i}$
  instantiates at most one of the variables $\vec{a_{m_i}}$, ensuring
  that we do not ``merge'' distinct variables from $\vec{a_{m_i}}$ by
  renaming them to the same variable in $\vec{b_i}$.
%
This is necessary for soundness, because distinct universals have to
be interpreted by distinct locations according to the semantics of
guarded universals.
\end{proof}
%
\begin{example}
As explained in \cref{sec:composing:motivation}, we integrate
re-scoping $\rescopeOP$ and derivability, $\derivestar$, into the
composition operation $\PCompose$.
%
We conclude this section with examples of the projection composition.
  \begin{itemize}
  \item For $\phi_1=\ls(x_2,x_3) \mw \ls(x_1,x_3)$ and
    $\phi_2=\emp \mw \ls(x_2,x_3)$, it holds that
    $\phi_1 \sep \phi_2 \deriveqf \emp \mw \ls(x_1,x_3)$.
    %
    Hence, $(\emp \mw \ls(x_1,x_3)) \in \phi_1\PCompose\phi_2$.
    %
  % \item Let $\phi_1=\FFA{a}\ls(x_2,a) \mw \ls(x_1,a)$ and
  %   $\phi_2=\FFA{b}\ls(x_3,b) \mw \ls(x_2,b)$,
  %   $\phi_1' = \FFA{c}\ls(x_2,c) \mw \ls(x_1,c)$, and
  %   $\phi_2' = \FFA{c}\ls(x_3,c) \mw \ls(x_2,c)$. Observe that
  %   $\euinst{\phi_i}{\emptyseq}{c}{\phi_i'}$ and that $(\ls(x_2,c) \mw
  %   \ls(x_1,c)) \sep (\ls(x_3,c) \mw \ls(x_2,c)) \deriveqf \ls(x_3,c)
  %   \mw \ls(x_1,c)$.
  %   Hence,
  %   $(\FFA{c}\ls(x_3,c) \mw \ls(x_1,c)) \in \phi_1\PCompose\phi_2$.
  %   %
  % \item Let
  %   $\phi_1 = \EEX{e_1} (\treerp(y,e_1) \mw \treerp(x,e_1)) \sep (\emp
  %   \mw \treerp(y,e_1))$ and $\phi_2 = \emp$. Then
  %   $\psi = \EEX{e_1} (\treerp(y,e_1) \mw \treerp(x,e_1)) \sep (\emp
  %   \mw \treerp(y,e_1))$ is a re-scoping of $\phi_1$ and $\phi_2$ and
  %   $(\treerp(y,e_1) \mw \treerp(x,e_1)) \sep (\emp \mw
  %   \treerp(y,e_1)) \deriveqf \emp \mw \treerp(x,e_1)$, so
  %   $(\EEX{e_1}\emp \mw \treerp(x,e_1)) \in \phi_1\PCompose\phi_2$.
  \item Let
    $\begin{aligned}[t]
      & \phi_1=\FFA{a}\ls(x_2,a) \mw \ls(x_1,a),
      & \phi_2=\FFA{b}\ls(x_3,b) \mw \ls(x_2,b),\\
      & \phi_1' = \FFA{c}\ls(x_2,c) \mw \ls(x_1,c)\text{ and}
      & \phi_2' = \FFA{c}\ls(x_3,c) \mw \ls(x_2,c).
    \end{aligned}$

    Observe that
    $\euinst{\phi_i}{\emptyseq}{c}{\phi_i'}$ and that $(\ls(x_2,c) \mw
    \ls(x_1,c)) \sep (\ls(x_3,c) \mw \ls(x_2,c)) \deriveqf \ls(x_3,c)
    \mw \ls(x_1,c)$.
    Hence,
    $(\FFA{c}\ls(x_3,c) \mw \ls(x_1,c)) \in \phi_1\PCompose\phi_2$.
    %
  \item Let
      $\phi_1 = \EEX{e_1} (\treerp(y,e_1) \mw \treerp(x,e_1))
                \sep (\emp \mw \treerp(y,e_1))$
      and
      $\phi_2 = \emp$.
      Then
    \[\psi = \EEX{e_1} (\treerp(y,e_1) \mw \treerp(x,e_1)) \sep (\emp
      \mw \treerp(y,e_1))\] is a re-scoping of $\phi_1$ and $\phi_2$
    and
    \[ (\treerp(y,e_1) \mw \treerp(x,e_1)) \sep (\emp \mw \treerp(y,e_1)) \deriveqf \emp \mw \treerp(x,e_1). \]
    Hence, we have
    $(\EEX{e_1}\emp \mw \treerp(x,e_1)) \in \phi_1\PCompose\phi_2$.
    %
  \item
    \cref{ex:pcompose-motivating-example} also works for the precise definition of $\PCompose$
    as formalized in this section.
  \end{itemize}
\end{example}
%
\subsection{Proof of \cref{cor:fcompose-to-pcompose}}\label{app:fcompose-to-pcompose}
%
\paragraph{Claim}
%
For all $\Sid$-forests $\frst_1,\frst_2$ with
$\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$, we have
\[
    \frst \in \frst_1\FCompose\frst_2
    \quad\text{implies}\quad
    \sfproj{\S}{\frst} \in \sfproj{\S}{\frst_1} \PCompose
    \sfproj{\S}{\frst_2}.
\]
%

\begin{proof}
We first show the claim for single-step derivations $\fderive$ and $\deriveqf$ in \cref{lem:fderive-to-derive} below.
A straightforward inductive argument then allows us to lift
that lemma from $\fderive$ to arbitrary derivations $\fderivestar$ and thus to $\FCompose$, which proves the claim.
\end{proof}


\begin{lemma}\label{lem:fderive-to-derive}
  Let $\frst_1,\frst_2$ be $\Sid$-forests with
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$.
  If $\frst_1\funion\frst_2 \fderive \frst$ then
  $\sfproj{\S}{\frst} \in \sfproj{\S}{\frst_1} \PCompose
  \sfproj{\S}{\frst_2}$.
\end{lemma}
\begin{proof}
  Let $\frst' \defn \frst_1\funion\frst_2$.
  Since $\frst' \fderive \frst$, there exists a location
  $l \in \dom(\frst)$ with $\frst' = \fsplit{\frst}{\set{l}}$.
  %
  In particular, there then exist trees
  $\ftree_1,\ftree_2 \in \frst'$ and $\ftree \in \frst$ such that
  \begin{enumerate}
  \item $\dom(\ftree_1)\cup\dom(\ftree_2)=\dom(\ftree)$,
  \item $\fruleinst{\set{\ftree_1,\ftree_2}}{l'} =
    \fruleinst{\set{\ftree}}{l'}$ for all $l'$,
  \item $l = \troot{\ftree_1}$, $l \in \tallholes{\ftree_2}$ and
    $(\tallholes{\ftree_1} \cup \tallholes{\ftree_2})\setminus \set{l}
    = \tallholes{\ftree}$.
  \end{enumerate}
  %
  This implies that the projections of $\ftree_1$ and $\ftree_2$ are
  mergeable into the the projection of $\ftree$ via generalized ponens
  (\cref{lem:gmp}). Let us examine this claim in more detail. By
  definition of stack--forest projection, we have for $1 \leq i \leq
  2$ and appropriate choices of $\vec{w_i}$, $\vec{e_i}$ that
  %
  \begin{align*}
    \sfproj{\S}{\frst_i} = & \EEX{\vec{e_i}}
                             \pinst{\zeta}{\dom(\stkchc)\concat\vec{w}}{\img(\stkchc)\concat\vec{e}},
    \text{ for}\\
    \zeta = & (\FFA{a_{i,1}} \pinst{\psi_{i,1}}{\vec{v_{i,1}}}{\vec{a_{i,1}}})
      \sep \cdots \sep(\FFA{a_{i,n_1}} \pinst{\psi_{i,n_1}}{\vec{v_{i,n_1}}}{\vec{a_{i,n_1}}}).
  \end{align*}
  %
  We construct a formula
  $\psi \in \rescope{\sfproj{\S}{\frst_1}}{\sfproj{\S}{\frst_2}}$ as
  follows:
  \begin{enumerate}
  \item We push $\vec{e_1}$ and $\vec{e_2}$ out.
    %
  \item For all $1 \leq j \leq n_1$ and every location
    $v \in \vec{v_{1,j}}$, if $v \in \vec{w_2}$---that is, if $v$ is a
    location that is existentially quantified in
    $\sfproj{\S}{\frst_2}$ and thus universally quantified in
    $\sfproj{\S}{\frst_1}$---then we instantiate
    the universal $\pinst{v}{\vec{v_{1,j}}}{\vec{a_{1,j}}}$
    with the existential
    $\pinst{v}{\vec{w_2}}{\vec{e_2}}$ in $\psi_{1,j}$.
    %
  \item Symmetrically, for all $1 \leq j \leq n_2$ and every
    location $v \in \vec{v_{2,j}}$, if $v \in \vec{w_1}$ then we
    instantiate $\pinst{v}{\vec{v_{2,j}}}{\vec{a_{2,j}}}$ with
    $\pinst{v}{\vec{w_1}}{\vec{e_1}}$ in $\psi_{2,j}$.
  \end{enumerate}
  Observe that in the resulting formula $\psi$, it holds for every
  location $v \in \locs{\fheapof{\frst_1\funion\frst_2}}$ that this
  location corresponds to a fixed variable in $\psi$, namely one of
  the variables in $\dom(\S)\cup\vec{e_1}\cup{\vec{e_2}}$.
  %
  In particular, this means that the thus-renamed projections of
  $\ftree_1$ and $\ftree_2$ can be merged via \cref{lem:gmp}, implying
  $\psi \deriveqf \sfproj{\S}{\frst}$.
\end{proof}

\subsection{Proof of \cref{lem:pcompose-to-fcompose}}\label{app:pcompose-to-fcompose}
%
We need a few auxiliary results in order to prove \cref{lem:pcompose-to-fcompose}.

First, merging two subformulas in $\deriveqf$ corresponds
exactly to merging two trees in $\frst_1$, which then yields the
desired forest $\frst_2$.
  %
  It might, however, be necessary to rename some locations that occur
  in predicate calls in $\frst_1$ that end up universally quantified
  so as to obtain trees to which we can apply $\fderive$;
  hence, the need to apply $\fderive$ to an $\alpha$-equivalent forest
  $\frst_1'$, not directly to $\frst_1$, in the lemma below.
  %
\begin{lemma}\label{lem:derive-to-fderive}
  Let $\frst_1$ be a $\Sid$-forest with
  $\fheapof{\frst_1}\in\Mpos{\Sid}$ and let $\phi$ be such that
  $\sfproj{\S}{\frst_1}\deriveqf \phi$. Then there exist forests
  $\frst_1',\frst_2$ with $\frst_1\AEQ\frst_1'$,
  $\frst_1'\fderive\frst_2$ and $\sfproj{\S}{\frst_2}=\phi$.
\end{lemma}
\begin{proof}
  % Let us examine this issue in more detail.
  %
  Assume
  $\sfproj{\S}{\frst_1} = \EEX{\vec{e_1}} \psi_{1,1} \sep \cdots \sep
  \psi_{1,n_1}$ and
  $\phi = \EEX{\vec{e_2}} \psi_{2,1} \sep \cdots \sep \psi_{2,n_2}$.
  %
  Because $\sfproj{\S}{\frst_1}\deriveqf \phi$, there exist indices
  $m_1,m_2,m_3$, sequences of variables $\vec{u_1},\vec{u_2}$, and
  formulas $\psi'_{1,m_1},\psi'_{1,m_2}$ such that
  %
  \begin{enumerate}
  \item  $\euinst{\psi_{1,m_i}}{\emptyseq}{\vec{u_i}}{\psi'_{1,m_i}}$
  for $1\leq i \leq 2$,
\item $\psi'_{1,m_1} \sep \psi'_{1,m_1} \implies \psi_{2,m_2}$ by
  \cref{lem:gmp}, and
\item $\phi \rewreq \IteratedStar
  ((\set{\psi_{1,1},\ldots,\psi_{1,n_1}}\setminus
  \set{\psi_{1,m_1},\psi_{1,m_2}}) \cup \psi_{2,m_2})$.
  \end{enumerate}
%
  Let $\ftree_1,\ftree_2 \in \frst_1$ and
  $\vec{v},\vec{e_1}$ be such that
  %
  \[\psi_{1,m_i} = \pinst{
      \ltproj{\img(\S)\cup\vec{v}}{\ftree_i}}{\vec{v}}{\vec{e_1}} ,\]
  %
  $1 \leq i \leq 2$.
  %
  There then exist variable sequences
  $\vec{a_1},\vec{a_2}$ and location sequences $\vec{v_1},\vec{v_2}$ such that
  \[
    \psi_{1,m_i} = \FFA{\vec{a_i}} \pinst{ \left(\IteratedStar\tallholepreds{\ftree_i}\right) \mw
      \trootpred{\ftree_i} }{\vec{v} \cdot
        \vec{v_i}}{\vec{e_1} \cdot \vec{a_i}}
  \]
  %
  We assume w.l.o.g.~that in the derivation
  $\sfproj{\S}{\frst_1} \deriveqf \phi$, the predicate call
  $\trootpred{\ftree_1}$ is merged with a call
  $\pred(\vec{l}) \in \tallholepreds{\ftree_2}$. (If this is not the
  case, simply swap $\ftree_1$ and $\ftree_2$.)

  Because $\euinst{\psi_{1,m_i}}{\emptyseq}{\vec{u_i}}{\psi'_{1,m_i}}$
  for $1\leq i \leq 2$ and
  $\psi'_{1,m_1} \sep \psi'_{1,m_1} \implies \psi_{2,m_2}$ by
  \cref{lem:gmp}
  there exist variable sequences $\vec{b_1}
  \subseteq\vec{a_1}\cup\vec{u_1}$ and
  $\vec{b_2}\subseteq\vec{a_2}\cup\vec{u_2}$
  such that
  \[ \pinst{ \trootpred{\ftree_1} }{\vec{v} \cdot
        \vec{v_1}}{\vec{e_1} \cdot
        \vec{a_1}}\pinstINST{\vec{a_1}}{\vec{b_1}} = \pinst{ \pred(\vec{l}) }{\vec{v} \cdot
        \vec{v_2}}{\vec{e_1} \cdot
        \vec{a_2}}\pinstINST{\vec{a_2}}{\vec{b_2}}. \]
    %
    A simplification step yields
    \[
      \pinst{ \trootpred{\ftree_1} }{\vec{v} \cdot
        \vec{v_1}}{\vec{e_1} \cdot
        \vec{b_1}} = \pinst{ \pred(\vec{l}) }{\vec{v} \cdot
        \vec{v_2}}{\vec{e_1} \cdot
        \vec{b_2}}.
    \]
  %
In general, there is, however, no guarantee that
$\trootpred{\ftree_1}=\pred(\vec{l})$: the calls only need to match
after variable introduction.

To ensure that the predicate calls in the trees match exactly, which
is required to apply $\fderive$, we therefore rename the locations in
$\vec{v_1}$ and $\vec{v_2}$ to fresh locations $\vec{v_1'}$ and
$\vec{v_2'}$ in such a way that for all $w_1\in\vec{v_1}$ and
$w_2 \in \vec{v_2}$, if
$\pinst{ w_1 }{\vec{v} \cdot
        \vec{v_1}}{\vec{e_1} \cdot
        \vec{b_1}} = \pinst{ w_2 }{\vec{v} \cdot
        \vec{v_2}}{\vec{e_1} \cdot
        \vec{b_2}}$
 then also
$\pinst{w_1}{\vec{v_1}}{\vec{v_1}'}=\pinst{w_2}{\vec{v_2}}{\vec{v_2}'}$.

We then rename the locations $\vec{v_1}$ in $\ftree_1$ to $\vec{v_1}'$
and the locations $\vec{v_2}$ in $\ftree_2$ to $\vec{v_2}'$, obtaining
$\ftree_1'$ and $\ftree_2'$.
%
We define
$\frst_1' \defn (\frst_1 \setminus \set{\ftree_1,\ftree_2}) \cup
\set{\ftree_1',\ftree_2'}$. Observe that $\frst_1\AEQ\frst_1'$,
because we have only renamed locations that were replaced by universal
quantifiers, i.e., locations that are \emph{not} in
$\locs{\fheapof{\frst_1}}$.
  %

  Now that the root call and hole call in the renamed trees match
  exactly, i.e., now that there exists a call
  $\pred(\vec{l'})\in\tallholepreds{\ftree_2'}$ with
  $\pred(\vec{l'})=\trootpred{\ftree_1'}$, we can apply $\fderive$ to
  the forest with the renamed trees, $\frst_1'$. We call the result
  $\frst_2$.
  %
  % TODO: Might want to add that the \fderive application corresponds
  % to splitting at \proot{\ftree_1}.
  %
  It is easy to verify that the projection of the merged trees is
  exactly $\psi_{2,m_3}$.
  %
  Consequently, $\sfproj{\S}{\frst_2}\rewreq \phi$.
\end{proof}

\begin{lemma}\label{lem:derivestar-to-fderivestar}
  If $\sfproj{\S}{\frst_1} \derivestar \phi$, then there exist $\Sid$-forests
  $\frst_1',\frst_2$ such that
  \begin{enumerate}
      \item $\frst_1\AEQ\frst_1'$,
      \item $\frst_1'\fderivestar\frst_2$, and
      \item $\sfproj{\S}{\frst_2} \rewreq \phi$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  We proceed by induction on the number $n$ of steps of the derivation
  $\sfproj{\S}{\frst_1} \derivestar \phi$.
  %
  If $n=0$, set $\frst_1'=\frst_2=\frst_1$.

  If $n>0$, let $\psi$ be such that $\sfproj{\S}{\frst_1} \derivestar
  \psi \deriveqf \phi$.
  %
  By the induction hypothesis, there exist forests
  $\frst_1'',\frst_3$ with $\frst_1\AEQ\frst_1''$,
  $\frst_1''\fderivestar\frst_3$ and $\sfproj{\S}{\frst_3}=\psi$.
  %
  By \cref{lem:derive-to-fderive}, there exist forests
  $\frst_3',\frst_2$ with $\frst_3\AEQ\frst_3'$,
  $\frst_3'\fderive\frst_2$ and $\sfproj{\S}{\frst_2}=\phi$.
  %

  Let $\vec{v_1},\vec{v_2}$ be the location sequences that witness
  $\frst_3\AEQ\frst_3'$, i.e., such that renaming $\vec{v_1}$ to
  $\vec{v_2}$ in $\frst_3$ yields $\frst_3'$.
%
  Also rename $\vec{v_1}$ to $\vec{v_2}$ in $\frst_1''$ to obtain a
  forest $\frst_1'$ with $\frst_1''\AEQ\frst_1'$.
  %
  Observe that because $\frst_1''\fderivestar\frst_3$, it holds that
  $\frst_1'\fderivestar \frst_3'$.
  %
  Combining this derivation with $\frst_3'\fderive\frst_2$, we obtain
  $\frst_1'\fderivestar \frst_2$. As we have already shown that
  $\sfproj{\S}{\frst_2}=\phi$, this proves the claim.
\end{proof}

We are now ready to prove~\cref{lem:pcompose-to-fcompose}:

\paragraph{Claim}
%\begin{lemma}\label{lem:pcompose-to-fcompose}
  Let $\frst_1,\frst_2$ be $\Sid$-forests with
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$
  and $\frst_1\funion\frst_2\neq\bot$.
  %
  If $\phi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}$,
  then there exist forests $\frst_1',\frst_2',\frst$ such that
  \begin{enumerate}
    \item $\frst_1\AEQ\frst_1'$,
    \item $\frst_2\AEQ\frst_2'$,
    \item $\frst\in\frst_1'\FCompose\frst_2'$, and
    \item $\phi=\sfproj{\S}{\frst}$.
  \end{enumerate}
%\end{lemma}
\begin{proof}
  Since
  $\phi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}$,
  there exists a formula $\psi$ such that
  \[
    \psi \in \rescope{\sfproj{\S}{\frst_1}}{ \sfproj{\S}{\frst_2}}
    ~\text{and}~
    \psi \derivestar \phi.
  \]

  We first construct forests $\frst_1''$ and $\frst_2''$ that are
  $\alpha$-equivalent to $\frst_1$ and $\frst_2$ in a way that
  corresponds to the instantiation steps that produced the re-scoping
  $\psi$:
  %
  For example, let $\ftree \in \frst_1$ and let $\FFA{\vec{a}}\zeta$ be
  the formula corresponding to $\ftree$ in
  $\sfproj{\S}{\frst_1}$. Assume that in the re-scoping, the variable
  $a \in \vec{a}$ was instantiated with the variable $e \in
  \vec{e_2}$, where $\vec{e_2}$ are the existential quantifiers in
  $\sfproj{\S}{\frst_2}$.
  %
  Assume further that the variable $a$ replaced the location $v_1$ in
  $\sfproj{\S}{\frst_1}$ and that the variable $e$ replaced the
  location $v_2$ in $\sfproj{\S}{\frst_2}$.

  Note that $v_2 \notin \locs{\fheapof{\frst_1}}$: By the semantics of
  the guarded existential $\eexists$,
  $v_2 \in \dom(\fheapof{\frst_2})$, so
  $v_2 \notin \dom(\fheapof{\frst_1})$.
  %
  Moreover, because $\SHpair{\S}{\fheapof{\frst_1}} \in \Mpos{\Sid}$
  and $v_2 \notin \img(\S)$, we have by
  \cref{lem:btw:pos-non-dangling} that
  $v_2 \notin \danglinglocs{\H_1}$.
  %
  Consequently, $v_2 \notin \locs{\fheapof{\frst_1}}$.
%
  This implies that renaming $v_1$ to $v_2$ in $\ftree$ yields a tree
  $\ftree'$ with $\ftree\AEQ\ftree'$.

  We repeat this process until we have renamed the appropriate
  location in $\frst_1\funion\frst_2$ for every instantiation in the
  re-scoping.
  %
  This yields a forest $\frst_1''\funion\frst_2''$ with
  $\frst_1\AEQ\frst_1''$, $\frst_2\AEQ\frst_2''$, and
  \[\sfproj{\S}{\frst_1''\funion\frst_2''} = \psi. \]

  We apply \cref{lem:derivestar-to-fderivestar} and obtain forests
  $\frst_1'$, $\frst_2'$, and $\frst$ with
  $\frst_1''\funion\frst_2'' \AEQ \frst_1'\funion\frst_2'$ (and thus
  $\frst_1''\AEQ\frst_1'$ and $\frst_2''\AEQ\frst_2'$),
  $\frst_1'\funion\frst_2' \fderivestar \frst$, and
  $\sfproj{\S}{\frst}=\phi$.
  %
  By definition, $\frst\in\frst_1'\FCompose\frst_2'$ and by
  transitivity of $\AEQ$, $\frst_1\AEQ\frst_1'$ and
  $\frst_1\AEQ\frst_2'$, proving the claim.
\end{proof}



==> Journal/cm-current.tex <==
\cmtodo{BEGIN: Everything below should be (re)moved}
\section{DEPOSIT}
%
%%
%\noindent
%\cmtodo{CMFIXME: heavily referenced, but we have proved another version before that does not consider aliasing constraints}
%Hence, it suffices to work with stack-aliasing constraints instead of individual stacks.
%In particular, for every fixed stack-aliasing constraint $\scls \in \EqClasses{\vec{x}}$, the induced set of $\vec{x}$-types is indeed finite:
%\begin{lemma}\label{lem:types-finite}
% Let $\Sid\in\IDbtw$, $\vec{x} \subseteq \Var$ finite, 
% and $n \defn \size{\Sid} + \size{\vec{x}}$.
% Then, for every stack-aliasing constraint
%  $\scls \in \EqClasses{\vec{x}}$, we have
%  $\size{\phitypes{\scls}{\true}} \in 2^{2^{\bigO(n^2 \log(n))}}$.
%\end{lemma}
%\begin{proof}
%  Let $\S$ be a stack with $\eqclasses{\S} = \scls$ and, consequently,
%  $\dom(\S) = \vec{x}$.
%  Then, every $\Sid$-type in $\phitypes{\scls}{\true}$ is a subset of 
%    $\DUSHx{\Sid}{\vec{x}}$.
%  By \cref{lem:dush-finite}, 
%    $\DUSHx{\Sid}{\vec{x}}$ is of size $2^{\bigO(n^2 \log(n))}$
%  and thus any subset is of size at most
%  $2^{2^{\bigO(n^2 \log(n))}}$.
%\end{proof}
%
%
%
%\cmtodo{CMFIXME: the definition below has not been introduced anywhere else yet; it should be replaced by $\phitypes{\eqclasses{\S}}{\fa}$}
%\begin{align*}
%& \gls{Types-sPhi} \defn \set{\sidtypeof{\S,\H} \mid \H \in \HH}
%  \subseteq \allsidtypes{\Sid}.
%\end{align*}
%
%\cmtodo{CMFIXME: the definition below has not been introduced anywhere else yet; it is only used in this section}
%\begin{definition}[$\S$-Types of a
%  formula]\label{def:types:s-phi-types}\index{s-types@$\S$-types}
%  \index{abstraction!of SLIDg formulas@of $\SLIDguarded$ formulas}
%  %
%  Let $\phi \in \SLIDguarded$ be a guarded formula. The
%  \emph{$\S$-types} of $\phi$ are given by
%  \[\gls{Typess-phi} \defn \set{ \sidtypeof{\S,\H} \mid \H \in \HH,
%      \SH \sidmodels \phi}.\]
%\end{definition}
%
%Note that $\phitypes{\S}{\phi} \subseteq \ssidtypes{\S}{\Sid}$.
%
%Furthermore, we denote by $\eqrestr{\scls}{\vec{y}}$ the \emph{restriction} of $\scls$ to the variables in $\vec{y}$, i.e.,
%$\eqrestr{\scls}{\vec{y}} \defn \scls \cap (\vec{y} \times \vec{y})$.
%
%\cmtodo{This should be a remark but where should we put it? The position in Sec. 9.2 did not seem appropriate. Also, is the example still up to date?}
%\paragraph*{The completeness of $\PCompose$ on the DUSH fragment.}
%We lift \cref{lem:delimited-forest-delimited-sub-forests} from
%$\S$-delimited forests and $\FCompose$ to DUSHs and $\PCompose$.
%
%\begin{infobox}{Understanding the incompleteness of~\cite{katelaan2019effective}}
%  In the extended version of~\cite{katelaan2019effective} available at
%  \cite{katelaan2019supplement}, we made a similar claim about
%  \emph{context decompositions} (cf.~\cite[Lemma
%  33]{katelaan2019supplement}), which, roughly speaking, correspond to
%  DUSHs without existential quantifiers. Unfortunately,
%  \cref{lem:heap-dush-to-subheap-dush} fails to hold when disallowing
%  (guarded) existentials in projections.
%  %
%  That is because the lemma depends on
%  \cref{lem:delimited-forest-delimited-sub-forests}, which only holds
%  for the ``full'' DUSH fragment, including guarded existentials.
%  %
%  This is the source of the
%  incompleteness of the approach of~\cite{katelaan2019effective}. I
%  illustrate this problem in the example immediately below this box.
%\end{infobox}
%
%\begin{example}[Necessity to allow existentials in DUSHs]\label{ex:dush:existentials-required}
%
%  Recall the forests $\frst_1,\frst_2$ from
%  \cref{ex:pcompose-motivating-example}.
%  Then
%  $\sfproj{\S}{\frst_0} \in \sfproj{\S}{\frst_1} \PCompose
%  \sfproj{\S}{\frst_2}$, because it holds for
%  %
%  \begin{align*}
%    \psi \defn \EEX{e_1} & (\PredName{p_2}(x_3, x_2, e_1) \mw
%      \PredName{p_1}(x_1,x_2,x_3)) \sep
%    (\emp\mw\PredName{ptr}(x_2,e_1))\\& \sep (\PredName{ptr}(x_2,e_1) \mw \PredName{p_2}(x_3,x_2,e_1))
%  \end{align*}
%  %
%  that $\psi \in \rescope{\sfproj{\S}{\frst_1}}{\sfproj{\S}{\frst_2}}$ and
%  %
%\begin{align*}
%   \psi \deriveqf & \EEX{e_1} (\PredName{p_2}(x_3, x_2, e_1) \mw
%      \PredName{p_1}(x_1,x_2,x_3)) \sep
%                (\emp\mw\PredName{p_2}(x_3,x_2, e_1)) \\
%    \deriveqf & \emp
%                   \mw \PredName{p_1}(x_1,x_2,x_3) = \sfproj{\S}{\frst_0},
%  \end{align*}
%  %
%  witnessing \cref{lem:heap-dush-to-subheap-dush}.
%  %
%  % In the first $\deriveqf$ step, we instantiate the
%  % universally-quantified variable $a_1$ with $e_1$ and then merge the
%  % projections of $\ftree_2$ and $\ftree_3$. In the second step, we
%  % then merge the two remaining formulas and drop the existential
%  % quantifier, since $e_1$ no longer occurs in any predicate call after
%  % merging the subformulas.
%
%  In contrast, there do \emph{not} exist forests $\frst_1'$,
%  $\frst_2'$ such that $\frst_i'\in \sidfrstsof{\H_i}$, neither
%  $\sfproj{\S}{\frst_1'}$ nor $\sfproj{\S}{\frst_2'}$ contains
%  existentials, and
%  \[\sfproj{\S}{\frst_0} \in \sfproj{\S}{\frst_1'} \PCompose
%    \sfproj{\S}{\frst_2}.\]
%  %
%  This illustrates that it is crucial to allow existential quantifiers
%  in DUSHs---for the set of all DUSHs that do not contain
%  existentials, \cref{lem:heap-dush-to-subheap-dush} does not
%  hold. This is the key distinction between the context decompositions
%  of \cite{katelaan2019effective} and the DUSHs I use in this thesis.
%\end{example}
%
%
%\begin{corollary}\label{cor:s-types-are-aliasing-types}
%  $\phitypes{\S}{\phi}=\phitypes{\eqclasses{\S}}{\phi}$ for all
%  $\S\in\SS$ and all $\phi\in\SLIDguarded$ with
%  $\locs{\phi}=\emptyset$.
%\end{corollary}
%
%\begin{corollary}\label{cor:x-types-union-of-aliasing-types}
%  $\phitypes{\vec{x}}{\phi}=\bigcup \set{\phitypes{\scls}{\phi} \mid
%    \scls \in \EqClasses{\vec{x}}}$ for all $\phi\in\SLIDguarded$ with
%  $\locs{\phi}=\emptyset$.
%\end{corollary}

%\input{PartC/DecidingBTW-SatCapture}

%\begin{lemma}[Isomorphic states have identical types]\label{lem:iso-same-type}
%    For all isomorphic states $\SH \Iso \SHpprime$ with $\dom(\S)=\dom(\S')$, we have $\sidtypeof{\S,\H}=\sidtypeof{\S',\H'}$.
%\end{lemma}
%
%\begin{proof}
%  Let $\typ\defn\sidtypeof{\S,\H}$ and $\typ' \defn
%  \sidtypeof{\S',\H'}$.
%  %
%  Let $\renfun$ be the function that witnesses the isomorphism, i.e.,
%  such that (1) for all $x$, $\S'(x) = \renfun(\S(x))$ and (2)
%  $\H' = \{ \renfun(l) \mapsto \renfun(\H(l)) \mid l \in \dom(\H)\}$.
%
%  Let
%  $\fa \in \sidtypeof{\S,\H}$. Then there exists a
%  forest $\frst \in \sidfrstsof{\H}$ such that
%  $\fa \in \sfproj{\S}{\frst}$.
%  %
%  We let $\frst'$ be the forest obtained from $\frst$ by renaming
%  every location in $\frst$ with $\renfun$, i.e.,
%  \begin{align*}
%    &\frst' \defn \set{\funapp{\renfun}{\ftree} \mid \ftree \in \frst},
%      \text{ where} \\
%    %
%    & \funapp{\renfun}{\ftree} \defn \bigg\{ \renfun(a) \mapsto
%    \big\langle \renfun(\tsucc{\ftree}{a}),\\&
%    \qquad\qquad\qquad\qquad\funapp{\renfun}{\thead{\ftree}{a}} \Rule
%      \funapp{\renfun}{a \mapsto \vec{b}}\sep
%      \funapp{\renfun}{\IteratedStar\tcalls{\ftree}{a}} \big\rangle \mid \\&\qquad\qquad a \in \dom(\ftree),
%      \locheapof{\ftree}{a}=\set{a \mapsto \vec{b}} \bigg\}.
%  \end{align*}
%  %
%  Note that by construction, $\fheapof{\frst'} = \renfun \funcomp
%  \fheapof{\frst} = \renfun\funcomp \H = \H'$.
%  %
%  Consequently, we have forest $\frst' \in \sidfrstsof{\H'}$ and
%  $\fa = \sfproj{\S'}{\frst'}$ and thus
%  $\fa \in \sidtypeof{\S',\H'}$.
%  %
%  Since $\fa$ was arbitrary, this proves that
%  $\sidtypeof{\S,\H}\subseteq\sidtypeof{\S',\H'}$. By a completely
%  symmetric argument, we can show the other inclusion,
%  $\sidtypeof{\S,\H}\supseteq\sidtypeof{\S',\H'}$.
%\end{proof}


%\subsection{Proof of \cref{lem:instantiation-models-call}}\label{app:instantiation-models-call}
%\paragraph{Claim}
%  Let $\vec{x}$ be a sequence of pairwise distinct variables,  let $\vec{y}$ be a sequence of (not necessarily pairwise distinct) variables with $|\vec{y}| = |\vec{x}|$ and let $\S$ be a stack with $\vec{y} \subseteq \dom(\S)$ and $\vec{x} \cap \dom(\S) = \emptyset$.
%  Let $\fa$ be a $\SLgeneric$ formula with free variables $\vec{x}$.
%  Then, $\SHpair{\pinst{\S}{\vec{x}}{\vec{y}}^{-1}}{\H} \sidmodels \fa$ if and only if
%  $\SHpair{\S}{\H}\sidmodels \pinst{\fa}{\vec{x}}{\vec{y}}$.
%
%\begin{proof}
%    Let $\S' = \pinst{\S}{\vec{x}}{\vec{y}}^{-1}$ and $\vec{z} = \dom(\S) \setminus \vec{y}$.
%    By definition of reverse stack instantiation, it holds that
%      \begin{align*}
%    \S'(x)&=\S(\pinst{x}{\vec{x}}{\vec{y}})& & \quad \text{for all } x \in \dom(\S) \cap \vec{x} \\
%    \S'(x)&=\S(x) &&\quad \text{for all } x \in \dom(\S) \setminus \vec{x} \tag*{\tagA}.
%  \end{align*}
%
%  Using this identity, we obtain
%  \begin{align*}
%    & \SHpair{\S'}{\H}\sidmodels\fa \\
%    %
%    \iff & \SHpair{\_}{\H} \sidmodels \pinst{\fa}{\dom(\S')}{\img(\S')}
%    \tag*{(by \cref{lem:existential-variable-stack-extension})}\\
%    %
%    \iff & \SHpair{\_}{\H} \sidmodels \pinst{\fa}{\vec{z}}{\S'(\vec{z})}\pinstINST{\vec{x}}{\S'(\vec{x})}
%    \tag*{(because of $\vec{x} \cap \vec{z} = \emptyset$)}\\
%    \iff & \SHpair{\_}{\H} \sidmodels
%               \pinst{\fa}{\vec{z}}{\S(\vec{z})}\pinstINST{\vec{x}}{\vec{y}}\pinstINST{\vec{y}}{\S(\vec{y})}
%               \tag*{(by \tagA)}\\
%    %
%    \iff & \SHpair{\_}{\H} \sidmodels
%               \pinst{\fa}{\vec{x}}{\vec{y}}\pinstINST{\vec{z}}{\S(\vec{z})}\pinstINST{\vec{y}}{\S(\vec{y})}
%               \tag*{(because of $\vec{x} \cap \vec{z} = \emptyset$ and $\vec{y} \cap \vec{z} = \emptyset$)}\\
%    %
%    \iff & \SHpair{\_}{\H} \sidmodels
%               \pinst{\fa}{\vec{x}}{\vec{y}}\pinstINST{\dom(\S)}{\img(\S)} \tag*{(because of $\vec{y} \cap \vec{z} = \emptyset$)}\\
%    %
%    \iff & \SHpair{\S}{\H} \sidmodels \pinst{\fa}{\vec{x}}{\vec{y}} \tag*{(by \cref{lem:existential-variable-stack-extension})},
%  \end{align*}
%  where we use $\_$ do denote an arbitrary stack.
%\end{proof}



==> Journal/deposit.tex <==
\section{Temporary storage for definitions and theorems}

\subsection{Removable theorems}
\begin{corollary}\label{cor:btw:star-model-to-oursunion}
  Let $\phi_1,\phi_2 \in \SLIDguarded$ be guarded formulas and let
  $\Sid\in\IDbtw$. Let $\SH \sidmodels \phi_1\sep\phi_2$.
  %
  Then there exist heaps $\H_1,\H_2$ such that
  $\SHi{1},\SHi{2}\in\Mpos{\Sid}$, $\H = \H_1\stdunion\H_2$,
  $\SHi{1} \sidmodels \phi_1$ and $\SHi{2} \sidmodels \phi_2$.
\end{corollary}
\begin{proof}
  By the semantics of $\sep$, there exist $\H_1$, $\H_2$ with $\H =
  \H_1 \stdunion \H_2$, $\SHi{1}\sidmodels\phi_1$ and $\SHi{2}\sidmodels\phi_2$.
  %
  By \cref{lem:pos-formula-pos-model}, $\SHi{1},\SHi{2}\in\Mpos{\Sid}$.
\end{proof}
\cmtodo{This is already covered by \cref{lem:pos-formula-pos-model}}

\subsection{Non-standard Terminology: Stack Inverse, Aliasing Constraints, Isomorphisms}
\label{sec:sl-preliminaries:non-standard}
%
\cmtodo{Some items in this section may still be moved further down into other sections.}
%
We conclude this section with a few technical definitions that frequently appear throughout this article; they are collected here to have an easily accessible reference.
It is safe to skip it for now and return later---the first occurrence of each definition below will refer back to this section.
%
%
\subsubsection{Locations in formulas}
%
The syntax of $\SLgeneric$ in \Cref{fig:sl:generic-syntax} admits locations to directly appear in formulas (cf.~\cite{reynolds2002separation}).
We collect all locations in formula $\phi$ in the set $\locs{\phi}$.
For example, we have $\locs{\EXO{x} \pto{7}{\tuple{x,0,3}}} = \set{3,7}$.
%
\cmtodo{END: Temporary storage for definitions and theorems}


==> Journal/projection-composition.tex <==
\noindent
Formalizing the operations $\rescopeOP$ and $\deriveqf$ is technically involved, but does not contain any deep insights that are relevant for the development of our decision procedure. 
In the remainder of this section, we thus only summarize the key properties; a precise formalization as well as proofs of said properties are found in \cref{app:projection-composition}. 
First, we remark that we can construct suitable operators $\rescopeOP$ and $\deriveqf$:
%
\begin{lemma}[Existence of re-scoping operation $\rescopeOP$]\label{lem:ex:rescoping:sound}
   There exists a re-scoping operation $\rescopeOP$ such that, for all
   stacks $\S$ and $\Sid$-forests $\frst_1,\frst_2$ with
   $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$, we have
   \[ 
        \phi \in \rescope{\sfproj{\S}{\frst_1}\,}{\,\sfproj{\S}{\frst_2}}
        \quad\text{implies}\quad
        \sfproj{\S}{\frst_1} \sep \sfproj{\S}{\frst_2} \sidmodels \phi.
   \]
\end{lemma}
%
\begin{lemma}[Existence of merge operation $\deriveqf$]\label{lem:ex:deriveqf:sound}
   There exists a merge operation $\deriveqf$ such that, for all
   stacks $\S$, $\Sid$-forests $\frst$, and $\phi \in \USH{\Sid}$, we have 
   \[
     \sfproj{\S}{\frst} \deriveqf \phi 
     \quad\text{implies}\quad
     \sfproj{\S}{\frst} \sidmodels \phi.
   \]
\end{lemma}
%
Based on the above two operations, we then compose forest projections as defined below.
%
\begin{definition}[Projection composition]\label{def:pcompose}
  For a stack $\S$ and $\Sid$-forests $\frst_1, \frst_2$, we define
  \[
      \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
      \defn
      \{ \phi \mid \zeta \derivestar \phi ~\text{for some}~\zeta \in \rescope{\sfproj{\S}{\frst_1}}{\sfproj{\S}{\frst_2}}.
  \]
  % Let $\phi_1,\phi_2\in\USH{\Sid}$.
\end{definition}
%
\begin{corollary}[Soundness of $\PCompose$]\label{lem:pcompose:sound}
  Let $\S$ be a stack and let $\frst_1,\frst_2$ be $\Sid$-forests
  such that
  $\frst_1\funion\frst_2\neq\bot$ and 
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$.
  Then 
  \[
    \psi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
    \quad\text{implies}\quad
    \sfproj{\S}{\frst_1} \sep \sfproj{\S}{\frst_2}\sidmodels \psi.
  \]
\end{corollary}
\begin{proof}
  Follows immediately from \cref{lem:ex:rescoping:sound,lem:ex:deriveqf:sound}
  and transitivity of implication.
\end{proof}
%
\subsubsection{Relating Forest Composition and Projection Composition}\label{sec:composing:correctness}
%
Recall our design goal that the projection function $\sfproj{\S}{\cdot}$
should be a homomorphism from forests and forest composition $\FCompose$ (\cref{def:forest-composition}) to projections
and projection composition $\PCompose$, i.e.,
\begin{align*}
  \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2} \overset{?}{=}
  \set{\sfproj{\S}{\frst} \mid \frst \in \frst_1 \FCompose \frst_2}. %\tag*{\tagA}
\end{align*}
%
\noindent
%
In one direction, our composition defined in \cref{def:pcompose} achieves this (cf. \cref{app:fcompose-to-pcompose}):
%
\begin{lemma}\label{cor:fcompose-to-pcompose}
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$, we have
  \[
    \frst \in \frst_1\FCompose\frst_2
    \quad\text{implies}\quad
    \sfproj{\S}{\frst} \in \sfproj{\S}{\frst_1} \PCompose
    \sfproj{\S}{\frst_2}.
  \]
\end{lemma}
%
\noindent
Unfortunately, as demonstrated below, the homomorphism breaks in the other direction:
%
\begin{example}[Projection is not homomorphic]\label{ex:proj-no-homo}
  Consider the $\Sid$-forests $\frst_2$ and $\frst_2$ given by:
  \begin{align*}
    & \ftree_1 \defn \set{l_1 \mapsto \tuple{\emptyset, (\odd(l_1,m_1)
      \Rule \ppto{l_1}{l_2} \sep \even(l_2,m_1)) }} \\
    %
    & \ftree_2 \defn \set{l_2 \mapsto \tuple{\emptyset, (\even(l_2,m_2)
      \Rule \ppto{l_2}{l_3} \sep \odd(l_3,m_2)) }}\\
  %
    & \frst_1 \defn \set{\ftree_1}, \frst_2\defn \set{\ftree_2} \\
    %
    & \S \defn \set{x_1 \mapsto l_1, x_2 \mapsto l_2, x_3 \mapsto l_3}
  \end{align*}
  %
  The corresponding projections are
  %
  \begin{align*}
    & \sfproj{\S}{\frst_1} = \FFA{a_1} \even(x_2,a_1) \mw
      \odd(x_1,a_1),~\text{and} \\
      %
    & \sfproj{\S}{\frst_2} = \FFA{a_1} \odd(x_3,a_1) \mw
      \even(x_2,a_1).
  \end{align*}
  Moreover, we have
  \begin{align*}
    & \FFA{a_1} \odd(x_3,a_1) \mw \odd(x_1,a_1) \in \sfproj{\S}{\frst_1}
    \PCompose \sfproj{\S}{\frst_2}.
  \end{align*}
  %
  However, since different locations, namely $m_1$ and $m_2$, are unused in the two forests,
  there is only one forest in $\frst_1 \FCompose \frst_2$: 
  $\set{\ftree_1,\ftree_2}$. It is not possible to merge the trees, because the hole predicate of the first tree,
  $\even(l_2,m_1)$, is different from the root of the second tree,
  $\even(l_2,m_2)$.
  %
  In particular, there does \emph{not} exist a forest $\frst$ with
  $\frst \in \frst_1\FCompose\frst_2$ and
  $\sfproj{\S}{\frst}=\FFA{a_1} \odd(x_3,a_1) \mw \odd(x_1,a_1)$.
\end{example}
%
\noindent
The essence of \cref{ex:proj-no-homo} is that while $\PCompose$ allows
renaming universals, $\FCompose$ does not allow renaming unused
locations, breaking the homomorphism.
%
To get a correspondence between the two notions of composition,  we
therefore allow renaming the
location terms in forests that do \emph{not} occur in any points-to
assertion. We capture this in the notion of \emph{$\alpha$-equivalence}.
%
\begin{definition}[$\alpha$-equivalence]\label{def:alpha-eq}\index{alpha-equivalence@$\alpha$-equivalence}
  Two $\Sid$-trees $\ftree_1,\ftree_2$ are \emph{$\alpha$-equivalent},
  denoted $\ftree_1\gls{--eq-AEQ}\ftree_2$, iff there exist locations $\vec{v_1} \in
  {(\Loc\setminus\locs{\fheapof{\ftree_1}})}^{*}$ and $\vec{v_2}\in\Loc^{*}$ such that
  \begin{align*}
    \ftree_2 = \set{ l \mapsto \tuple{\tsucc{\ftree_1}{l},
    \pinst{\truleinst{\ftree_1}{l}}{\vec{v_1}}{\vec{v_2}} \mid l \in
      \dom(\ftree_1)}},
  \end{align*}
  where the substitution is given by
  $ 
  \pinst{(\pred(\vec{l}) \Rule \phi)}{\vec{v_1}}{\vec{v_2}} \defn
  \pred(\pinst{\vec{l}}{\vec{v_1}}{\vec{v_2}}) \Rule
  \pinst{\phi}{\vec{v_1}}{\vec{v_2}}
  $.
  %

  Moreover, two $\Sid$-forests
$\frst_1=\ktrees,\frst_2=\set{\bartree_1,\ldots\bartree_k}$ are
\emph{$\alpha$-equivalent}, also denoted $\frst_1\AEQ\frst_2$, iff
$\ftree_i\AEQ\bartree_i$ holds for all $1 \leq i \leq k$.
\end{definition}
%
\noindent
Hence, $\frst_1 \AEQ \frst_2$ holds if the
location terms in $\frst_1$ that do \emph{not} occur in points-to
assertions can be renamed a way such that we obtain $\frst_2$.
%
Consequently, $\alpha$-equivalent forests induce the same heap.

\begin{lemma}\label{lem:aeq-same-projections}
  If $\frst_1\AEQ\frst_2$ then $\fheapof{\frst_1}=\fheapof{\frst_2}$.
\end{lemma}
\begin{proof}
  The forest $\frst_2$ differs from $\frst_1$ only in locations that are not in $\fheapof{\frst_1}$.
\end{proof}
%
\noindent
Considering forests up to $\alpha$-equivalence then yields the desired connection between forests and their projections
(cf. \cref{app:pcompose-to-fcompose} for a proof):

\begin{lemma}\label{lem:pcompose-to-fcompose}
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\frst_1\funion\frst_2\neq\bot$ and
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$,
  %
  \begin{align*}
    \phi \in \sfproj{\S}{\frst_1} \PCompose \sfproj{\S}{\frst_2}
    \quad\text{implies}\quad
      \exists \frst \in \bigcup_{\barfrst_1 \AEQ \frst_1, \barfrst_2 \AEQ \frst_2} \barfrst_1 \FCompose \barfrst_2 .\quad
      \phi=\sfproj{\S}{\frst}.
    %\text{ex.}~ \barfrst_1 \AEQ \frst_1,\, \barfrst_2 \AEQ \frst_2, \frst \in \barfrst_1 \FCompose \barfrst_2~\text{s.t.}~
    %\phi=\sfproj{\S}{\frst}.
  \end{align*}
\end{lemma}

\begin{theorem}\label{thm:fcompose-eq-pcompose}
  \index{homomorphism!of forest projection}
  %
  For all $\Sid$-forests $\frst_1,\frst_2$ with
  $\frst_1\funion\frst_2\neq\bot$ and
  $\SHpair{\S}{\fheapof{\frst_1}},\SHpair{\S}{\fheapof{\frst_2}}\in\Mpos{\Sid}$,
\begin{align*}
  \sfproj{\S}{\frst_1}\PCompose\sfproj{\S}{\frst_2} ~=~
  \set{\sfproj{\S}{\frst} \mid 
  \frst \in \barfrst_1 \FCompose \barfrst_2,~
  \barfrst_1\AEQ\frst_1,~
  \barfrst_2\AEQ\frst_2
  }.
\end{align*}
\end{theorem}
\begin{proof}
  Immediate from
  \cref{cor:fcompose-to-pcompose,lem:pcompose-to-fcompose}.
\end{proof}



==> Journal/related-work.tex <==
\section{Related Work}\label{sec:related-work}
%
\cmtodo{ToDo}
%
%
\cmtodo{ToDo End}
%


==> Journal/using-types.tex <==
\section{Using Types to Decide Guarded Separation Logic}
%
We now argue that satisfiability of Guarded Separation Logic ($\SLIDguarded$) can be decided by computing a (finite) set of types; a corresponding algorithm is discussed afterward in \cref{ch:deciding-btw}.

The main idea is to the reduce the satisfiability problem for $\SLIDguarded$---``given a $\SLIDguarded$ formula $\fa$, does $\fa$ have a model $\SH \sidmodels \fa$?''---to the question of whether some type $\typ$ can be computed from a model of $\fa$, i.e., $\typ = \sidtypeof{\S,\H}$ should hold for some $\SH \sidmodels \fa$; the set of all such types is formally defined below.
To conveniently reason about such sets, we additionally group types by aliasing constraint; types in the same set thus have the same free variables and the same aliases.

%
\begin{definition}[$\scls$-Types]\label{def:types:x-phi-types}
 Let $\scls$ be an aliasing constraint (cf. \cref{sec:aliasing-constraint}).
 Then the set
 $\phitypes{\scls}{\phi}$ of \emph{$\scls$-types} of $\SLIDguarded$ formula $\phi$
 is defined as 
\begin{align*}
  \phitypes{\scls}{\phi}
  \defn
    \set{ \sidtypeof{\S,\H} \mid \S \in \SS,~ \H \in \HH,~ \eqclasses{\S} = \scls,~ \SH \sidmodels \phi }.
\end{align*}
\end{definition}
%
%
\noindent
By the above definition, a $\SLIDguarded$ formula $\fa$ with at least
one non-empty set of $\scls$-types is satisfiable: some type coincides with $\sidmodels{\S,\H}$, where
$\SH \sidmodels \fa$.
Conversely, if $\fa$ is satisfiable, then there exists a model $\SH \sidmodels \fa$ and the set 
$\phitypes{\eqclasses{\S}}{\fa}$ is non-empty. In summary:
\[
  \fa~\text{is satisfiable} \quad\text{iff}\quad
  \exists \scls.~\phitypes{\scls}{\fa} \neq \emptyset.
\]
On a first glance, finding a suitable aliasing constraint $\scls$ and proving non-emptiness of $\phitypes{\scls}{\fa}$
might appear as difficult as finding a state $\SH$ such that $\SH \sidmodels \fa$ holds due to two concerns:
%
\begin{enumerate}
%
\item There are, in general, both infinitely many aliasing constraints and infinitely many $\Sid$-types, because the size of stacks---and thus the number of free variables to consider---is unbounded.
%
\item Deciding whether a type $\typ$ belongs to $\phitypes{\scls}{\fa}$ seems non-trivial:
assume that $\SH \sidmodels \fa$, $\SHpprime \not\sidmodels \fa$,
and both states yield the same type, i.e., $\typ = \sidtypeof{\S,\H} = \sidtypeof{\S',\H'}$.
Determining that $\typ \in \phitypes{\scls}{\fa}$ would then require us to know that $\typ$ can be computed from a specific state, namely $\SH$.
%
\end{enumerate}
%
We will address both concerns in the remainder of this section.
%

%
Regarding (1), we note that both aliasing constraints and types can be safely restricted to a finite set $\vec{x}$ of variables as long as $\vec{x}$ covers at least the free variables of the formula $\fa$ under consideration, i.e., $\vec{x} \supseteq \fvs{\fa}$.
The number of aliasing constraints to consider---those in $\EqClasses{\vec{x}}$---then equals the $\size{\vec{x}}$-th Bell number, bounded by $n^n \in \bigO(2^{n \log(n)})$, where $n = \size{\Sid} + \size{\vec{x}}$.
We will show in \cref{sec:using-types:finiteness} that the total number of $\scls$-types over all $\SLIDguarded$ formulas is bounded, too.
In total, determining whether $\exists \scls.~\phitypes{\scls}{\fa} \neq \emptyset$ holds thus amounts to computing finitely many finite sets.
%

%
Regarding (2), we show that the careful definition of $\scls$-types allows us to decide whether a type $\typ$ belongs 
to $\phitypes{\scls}{\fa}$ \emph{without reverting to any state underlying $\typ$}.
In particular, we will show a \emph{refinement theorem} in \cref{sec:using-types:refinement}, which ensures that states yielding the same $\Sid$-type satisfy the same $\SLIDguarded$ formulas---thus ruling out the issue raised in (2).
%
%
\subsection{Finiteness}\label{sec:using-types:finiteness}
%
To ensure finiteness of the type abstraction, we only consider stacks with variables taken from some fixed finite set $\vec{x}$.
In order to prove that this restriction admits only finitely many types, we collect in $\allxtypes$ all $\scls$-types over $\Sid$ and $\vec{x}$, i.e.,
\[
  \allxtypes
  \defn
  \bigcup_{\scls \in \EqClasses{\vec{x}}} \bigcup_{\phi \in \SLIDguarded} \phitypes{\scls}{\phi}.
\]
%
\begin{theorem}\label{thm:types-finite}
 Let $\vec{x} \subseteq \Var$ be finite and $n \defn \size{\Sid} + \size{\vec{x}}$.
 Then $\size{\allxtypes} \in 2^{2^{\bigO(n^2 \log(n))}}$.
\end{theorem}
\begin{proof}
  Recall from \cref{lem:dush-finite} that
  the set $\DUSHx{\Sid}{\vec{x}}$ of DUSHs over $\Sid$
  with free variables taken from $\vec{x}$ is of size
  $2^{\bigO(n^2 \log(n))}$.
  %
  We show below that every type $\typ \in \allxtypes$ is a subset of $\DUSHx{\Sid}{\vec{x}}$.
  Hence, the size of $\allxtypes$ is bounded by the number of subsets of $\DUSHx{\Sid}{\vec{x}}$, i.e.,
  $\size{\allxtypes} \in 2^{2^{\bigO(n^2 \log(n))}}$.

  It remains to show that, for every $\typ \in \allxtypes$, we have $\typ \subseteq \DUSHx{\Sid}{\vec{x}}$:
  \begin{itemize}
      \item By definition of $\allxtypes$, there exists 
          an aliasing constraint $\scls \in \EqClasses{\vec{x}}$  and
          a $\SLIDguarded$ formula $\fa$ and 
          such that $\typ \in \phitypes{\scls}{\fa}$.
    \item Since $\Sid \in \IDbtw$ and $\fa \in \SLIDguarded$, \cref{lem:pos-formula-pos-model} yields that every model of $\fa$ is a \emph{guarded} state.
    \item Then, by \cref{def:types:x-phi-types}, there exists a guarded state $\SH \in \Mpos{\Sid}$ such that
          $\dom(\S) = \dom(\scls) \subseteq \vec{x}$, $\SH \sidmodels \fa$, and $\typ = \sidtypeof{\S,\H}$.
    \item By \cref{def:sid-type},
          $\typ = \sidtypeof{\S,\H} = \set{\sfproj{\S}{\frst} \mid \frst \in \sidfrstsof{\H} } \cap \DUSH{\Sid}$.
    \item Since $\SH \in \Mpos{\Sid}$, \cref{lem:sf-projection-sound} yields, for each $\fa \in \typ$, that $\SH \sidmodels \fa$; in particular, this means $\fvs{\fa} \subseteq \dom(\S) \subseteq \vec{x}$.
  \end{itemize}
  Hence, $\fa \in \DUSH{\Sid}$ and $\fvs{\fa} \subseteq \vec{x}$.
  In other words, $\fa \in \DUSHx{\Sid}{\vec{x}}$, which concludes the proof.
\end{proof}
%
\subsection{Type Refinement}\label{sec:using-types:refinement}
%
The main insight required for effectively deciding whether a type $\typ$ belongs to $\phitypes{\scls}{\fa}$ is that
states with identical $\Sid$-types satisfy the same $\SLIDguarded$ formulas---a statement we formalize below.
%
This property is perhaps surprising, as types only contain formulas from the
DUSH fragment, which is largely orthogonal to $\SLIDguarded$. For
example, $\SLIDguarded$ formulas allow guarded negation and guarded
septraction, but neither quantifiers nor unguarded magic wands,
whereas DUSHs allow limited use of guarded quantifiers and unguarded
magic wands, but neither Boolean structure nor septraction.
%
\subsubsection{Assumptions}\label{sec:using-types:assumptions}
For a concise formalization, we assume---in addition to our global assumptions stated in \cref{sec:sl-basics:sid-assumptions}---that 
%all SIDs considered in the remainder of this section are (a) in the bounded treewidth fragment $\IDbtw$ and (b) pointer-closed, i.e., 
%contain a dedicated predicate simulating each points-to assertion (cf. \cref{def:ptrclosed}).
%Moreover, since we allowed concrete locations in $\SLIDguarded$ formulas only as an auxiliary construct, we assume that 
all formulas $\phi$ under consideration are $\SLIDguarded$ formulas without location terms, i.e., $\locs{\phi} = \emptyset$ (note that the null pointer $\nil$ is still permitted as it is not a location).

\subsubsection{The refinement theorem}
With these assumptions in mind, our goal is to show the following:
%
\begin{theorem}[Refinement theorem]\label{thm:types-capture-sat}
  For all stacks $\S$, heaps $\H_1$, $\H_2$, and $\SLIDguarded$ formulas $\fa$, 
  \[
      \sidtypeof{\S,\H_1} = \sidtypeof{\S,\H_2}
      \qquad\text{implies}\qquad
      \SHi{1} \sidmodels \phi ~~\text{iff}~~ \SHi{2} \sidmodels \phi~.
  \]
\end{theorem}
%
\noindent
Before we prove the above theorem, we remark that
\Cref{thm:types-capture-sat} immediately implies that, if the type of a
guarded state $\SH$ is equal to some already-known type of some other state $\SHpprime$ satisfying formula $\fa$, then
$\SH$ satisfies $\fa$---a crucial property for the correctness of our approach.

\begin{corollary}\label{cor:phi-typ-satisfies-phi}
    Let $\SH \in \Mpos{\Sid}$. If there exists a type $\typ$ such that $\typ \in \phitypes{\eqclasses{\S}}{\fa}$
  and $\sidtypeof{\S,\H} = \typ$, then $\SH \sidmodels \fa$.
\end{corollary}
\begin{proof}
  Since $\typ \in \phitypes{\eqclasses{\S}}{\fa}$, there exists a state $\SHpprime$ such that
  (1) $\typ = \sidtypeof{\S',\H'}$, 
  (2) $\eqclasses{\S'} = \eqclasses{\S}$, and 
  (3) $\SHpprime \sidmodels \fa$.
  Due to (2), we have $\S = \S'$ and thus $\SHprime \sidmodels \fa$.
  By assumption, we have $\sidtypeof{\S,\H'} = \typ = \sidtypeof{\S,\H}$.
  Hence, by \cref{thm:types-capture-sat}, $\SH \sidmodels \fa$.
\end{proof}
%
\noindent
Moreover, recall that $\SLIDguarded$ formulas are quantifier-free (although quantifiers may appear in predicate definitions).
As demonstrated below, this limitation is crucial for upholding \cref{thm:types-capture-sat}.
%
\begin{example}
  Recall $\SidLs$ from \cref{ex:sids}. Moreover, let $\SHi{k}$,
  $k \in \N$, be a list of length $k$ from $x_1$ to $x_2$. It then
  holds for all $i,j\geq 2$ that $\sidtypeof{\S,\H_i} =
  \sidtypeof{\S,\H_j}$. However,
  \begin{align*}
    \SHi{2} \not\sidmodels \SHEX{\tuple{y_1,y_2}}
    \lseg(x_1,y_1)\sep\lseg(y_1,y_2)\sep\lseg(y_2,x_2),
  \end{align*}
  whereas
  \begin{align*}
  \SHi{j} \sidmodels \SHEX{\tuple{y_1,y_2}}
  \lseg(x_1,y_1)\sep\lseg(y_1,y_2)\sep\lseg(y_2,x_2)
  \end{align*}
  for all $j \geq 3$.
  Hence, the refinement theorem 
  does not hold if we admit quantifiers in $\SLIDguarded$ formulas.
\end{example}
%
\noindent
\subsubsection{Proving the refinement theorem}
We will prove \cref{thm:types-capture-sat} by structural induction on the syntax of $\SLIDguarded$ formulas.
For most base cases---those that involve the heap---we rely on the fact that a state satisfies all 
formulas in its type.
%
\begin{lemma}\label{lem:forms-in-type-hold}
  If $\phi \in \sidtypeof{\S,\H}$ for some state $\SH$, then $\SH \sidmodels \phi$.
\end{lemma}
\begin{proof}
  Since $\phi \in \sidtypeof{\S,\H}$, there exists a $\Sid$-forest
  $\frst$ with $\fheapof{\frst}=\H$ and $\sfproj{\S}{\frst}=\phi$.
  %
  By \cref{lem:sf-projection-sound}, we have
  $\SHpair{\S}{\fheapof{\frst}}\sidmodels \sfproj{\S}{\frst}$
  and thus also $\SH \sidmodels \phi$.
  %
\end{proof}
%
\noindent
Furthermore, we exploit that if a type $\typ$ can be computed from a \emph{guarded} state, then \emph{every} state with type $\typ$ is guarded as well.
%
\begin{lemma}\label{lem:same-type-both-guarded}
  If $\SH\in\Mpos{\Sid}$ and $\sidtypeof{\S,\H} = \sidtypeof{\S,\H'}$, then $\SHprime \in \Mpos{\Sid}$.
\end{lemma}
\begin{proof}
  By \cref{lem:guarded-iterated-star-predicates},
  %By \cref{def:positive-model}, 
  $\SHi{1} \sidmodels\pred_1(\vec{x_1})\sep\cdots\sep\pred_k(\vec{x_k})$ for
  some choice of predicate calls.
  %
  For
  $\psi\defn\IteratedStar_{1\leq i \leq k}(\emp \mw
  \pred_i(\vec{x_i}))$, it then holds that
  $\psi \in \sidtypeof{\S,\H_1}=\sidtypeof{\S,\H_2}$.
  %
  \Cref{lem:forms-in-type-hold} yields that $\SHi{2} \sidmodels \psi$
  holds.
  %
  Therefore,
  $\SHi{2} \sidmodels
  \pred_1(\vec{x_1})\sep\cdots\sep\pred_k(\vec{x_k})$, implying
  $\SHi{2}\in\Mpos{\Sid}$.
\end{proof}
%
\noindent
Finally, to deal with the separating conjunction, we need another auxiliary result.
In \cref{lem:types:homo:compose}, we showed how two types can be composed into a single one, i.e.,
\[ \sidtypeof{\S,\H_1}\Compose\sidtypeof{\S,\H_2}=\sidtypeof{\S,\H_1\stdunion\H_2}~. \]
To prove \cref{thm:types-capture-sat}, we need the reverse: 
Given a composed type, say $\sidtypeof{\S,\H}=\typ_1\Compose\typ_2$, 
we need to \emph{decompose} $\H$ into two heaps whose types (in conjunction with stack $\S$) are $\typ_1$ and $\typ_2$.
%
\begin{lemma}[Type decomposability]\label{lem:types:decompose}
  %
  Let $\SH\in\Mpos{\Sid}$ and assume that
  $\sidtypeof{\S,\H}=\typ_1\ACompose\typ_2$.
  %
  Then there exist $\H_1,\H_2$ such that
  %$\SHpair{\S}{\H_1},\SHpair{\S}{\H_2}\in\Mpos{\Sid}$,
  $\H=\H_1\stdunion\H_2$, $\typ_1=\sidtypeof{\S,\H_1}$, and
  $\typ_2=\sidtypeof{\S,\H_2}$.
\end{lemma}
%
Since proving type decomposability involves a bit more technical machinery, we refer the interested
reader to \cref{app:types:decompose} for a detailed proof.
%

With the above three lemmas at hand, we can now to prove the refinement theorem.
%
\begin{proof}[Proof (of \cref{thm:types-capture-sat})]
  If $\SHi{1}$ or $\SHi{2}$ is not a guarded state in $\Mpos{\Sid}$, 
  then $\sidtypeof{\S,\H_1}$ is undefined and neither model satisfies $\phi$ by
  \cref{lem:pos-formula-pos-model}.

  Let us thus assume $\SHi{1},\SHi{2}\in \Mpos{\Sid}$.
  %
  We proceed by induction on the structure of the $\SLIDguarded$ formula $\phi$. 
  We only show that if $\SHi{1} \sidmodels \phi$ then $\SHi{2} \sidmodels \phi$; 
  the converse direction is symmetric.
  %
  \begin{description}
  \item[Case $\phi=\emp$.] Assume that $\SHi{1} \sidmodels \phi$. By
    the semantics of $\emp$, we have $\H_1 = \emptyset$. 
    Let $\frst$ be the empty forest. Then
    $\frst \in \sidfrstsof{\H_1}$ and thus
    $\emp=\sfproj{\S}{\frst} \in \sidtypeof{\S,\H_1} =
    \sidtypeof{\S,\H_2}$. 
    Hence, by \cref{lem:forms-in-type-hold}, we have $\SHi{2} \sidmodels \emp$.
    %
  \item[Cases $\phi = \sleq{x}{y}$, $\phi=\slneq{x}{y}$.] Trivial,
      because the states $\SHi{1}$ and $\SHi{2}$ have the same stack.
    %
  \item[Case $\phi = \pto{x}{\tuple{y_1,\ldots,y_k}}$.] Assume that
      $\SHi{1} \sidmodels \phi$. 
      By assumption (see \cref{sec:using-types:assumptions}), $\Sid$ is \ptrclosed{}, i.e., 
    $\SHi{1} \sidmodels \ptrpred_{k}(x,y_1,\ldots,y_k)$.
    %
    We define a $\Sid$-forest $\frst = \set{\ftree}$, where $\ftree$ is 
    \begin{align*}
    \ftree = \{ \S(x) \mapsto \langle \emptyset,
        \ptrpred_{k}(\S(x),\S(y_1),\ldots,\S(y_k))\; \Rule
        \pto{\S(x)}{\tuple{\S(y_1),\ldots,\S(y_k)}} \rangle\}~.
    \end{align*}
    %
    Observe that $\frst \in \sidfrstsof{\H_1}$ and
    %
    \begin{align*}
\ptrpred_{k}(x,y_1,\ldots,y_k)=\sfproj{\S}{\frst} \in
    \sidtypeof{\S,\H_1} = \sidtypeof{\S,\H_2}.
    \end{align*}
    %
    Hence, by \cref{lem:forms-in-type-hold}, we have
    $\SHi{2} \sidmodels \ptrpred_{k}(x,y_1,\ldots,y_k)$.
    %
    By definition of the predicate $\ptrpred_k$, we conclude that
    $\SHi{2} \sidmodels \pto{x}{\tuple{y_1,\ldots,y_k}}$.
    %
  \item[Case $\phi = \pred(z_1,\ldots,z_k)$.] Assume that
    $\SHi{1} \sidmodels \phi$.
    %
    By \cref{lem:model-of-pred-to-tree}, there exists a $\Sid$-tree
    $\ftree$ with $\trootpred{\ftree}=\pred(\S(z_1),\ldots,\S(z_k))$,
    $\tallholepreds{\ftree}=\emptyset$, and
    $\fheapof{\set{\ftree}}=\H_1$.
    %
    Let
    \[
      \psi \defn
      \pinst{\pred(\S(z_1),\ldots,\S(z_k))}{\dom(\stkchc)}{\img(\stkchc)}
      = \sfproj{\S}{\set{\ftree}}
    .\]
    %
    Thus, $\psi \in \sidtypeof{\S,\H_1} = \sidtypeof{\S,\H_2}$
    and, by 
    \cref{lem:forms-in-type-hold}, $\SHi{2} \sidmodels \psi$.
    %
    Observe that while $\psi \neq \pred(\vec{z})$ is possible, we have
    by definition of $\stkchc$ that the parameters of the predicate
    call in $\psi$ evaluate to the same locations as the parameters
    $\vec{z}$.  Hence, $\SHi{2}\sidmodels\pred(z_1,\ldots,z_k)$.
    %
  \item[Case $\phi = \phi_1 \wedge \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$. We then have $\SHi{1} \sidmodels \phi_1$
    and $\SHi{1} \sidmodels \phi_2$. By I.H.,
    $\SHi{2} \sidmodels \phi_1$ and $\SHi{2} \sidmodels \phi_2$.
    Hence,
    $\SHi{2} \sidmodels \phi_1 \wedge \phi_2$.
    %
  \item[Case $\phi = \phi_1 \vee \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$. We then have 
    $\SHi{1} \sidmodels \phi_1$ or $\SHi{1} \sidmodels \phi_2$. Assume
    w.l.o.g.~that $\SHi{1} \sidmodels \phi_1$. By I.H., $\SHi{2} \sidmodels \phi_1$.
    Hence, $\SHi{2} \sidmodels \phi_1 \vee \phi_2$.
    %
  \item[Case $\phi = \phi_1 \wedge\neg \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$. We then have 
    $\SHi{1} \sidmodels \phi_1$ and $\SHi{2} \not\sidmodels
    \phi_2$. By I.H., $\SHi{2} \sidmodels \phi_1$
    $\SHi{2} \not\sidmodels \phi_2$. Hence,
    $\SHi{2} \sidmodels \phi_1 \wedge \neg \phi_2$.
    %
  \item[Case $\phi = \phi_1 \sep \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$.
    %
    By the semantics of $\sep$, there exist heaps $\Hoo$ and $\Hot$ such
    that $\SHpair{\S}{\H_{1,i}} \sidmodels \phi_i$ for
    $1 \leq i \leq 2$.
    %
    Let $\typ_i \defn \sidtypeof{\S,\H_{1,i}}$; we then apply
    \cref{lem:types:decompose} to $\SHi{2}$, $\typ_1$ and $\typ_2$ to
    obtain states $(\S,\Hto)$ and $(\S,\Htt)$ with $\H_2=\Hto\stdunion\Htt$,
    $\sidtypeof{\S,\Hto}=\typ_1$, and $\sidtypeof{\S,\Htt}=\typ_2$.
    Moreover, by \cref{lem:pos-formula-pos-model}, we know that 
    $\SHpair{\S}{\H_{1,i}} \in \Mpos{\Sid}$.
    Applying \Cref{lem:same-type-both-guarded} to $\Hoo$ and $\Hto$ then
    yields $\SHpair{\S}{\H_{2,i}} \in \Mpos{\Sid}$.

    We can thus apply the I.H. to both
    $\Hoo$, $\Hot$, $\phi_1$ and $\Hto$, $\Htt$, $\phi_2$
    to conclude that
    $\SHpair{\S}{\H_{2,1}} \sidmodels \phi_1$
    and $\SHpair{\S}{\H_{2,2}} \sidmodels \phi_2$.
    %
    Since $\Hto \stdunion \Htt = \H_2$, the semantics
    of $\sep$ then yields $\SHi{2} \sidmodels \phi$.
    %
  \item[Case $\phi = \phi_0 \wedge (\phi_1 \protect\sept \phi_2)$.]
    Assume that $\SHi{1} \sidmodels \phi$.
    %
    Then there exists a heap $\H_0$ with $\SHi{0} \sidmodels \phi_1$
    and $\SHpair{\S}{\H_1 \stdunion \H_0} \sidmodels \phi_2$.

    Since $\SHi{1}$ and $\SHi{2}$ have the same type, we have
    $\valloc{\S,\H_1}=\valloc{\S,\H_2}$.  We can therefore
    assume w.l.o.g.~that $\H_2 \stdunion \H_0$ is defined---if this
    is not the case, simply replace $\H_0$ with a heap $\H_0'$ such
    that $\SHi{0} \Iso \SHpair{\S}{\H_0'}$ and both
    $\H_1 \stdunion \H_0'$ and $\H_2 \stdunion \H_0'$ are defined.
    %
    Then, by \cref{lem:sid:iso-models-same-formulas}, we can conclude that $(\S, \H_1\stdunion
    \H_0')\sidmodels \phi$.

    By assumption, $\SHi{1}\in\Mpos{\Sid}$ and, by
    \cref{lem:pos-formula-pos-model}, $\SHi{0}\in\Mpos{\Sid}$. 
    Thus, $\SHpair{\S}{\H_1\stdunion\H_0}\in\Mpos{\Sid}$.
    %
    Our assumptions and \cref{lem:types:homo:compose} then yield
    %
    \begin{align*}
\sidtypeof{\S,\H_1\stdunion\H_0} ~=~& \sidtypeof{\S,\H_1} \Compose
    \sidtypeof{\S,\H_0}\\ ~=~& \sidtypeof{\S,\H_2} \Compose
    \sidtypeof{\S,\H_0}\\ ~=~& \sidtypeof{\S,\H_2\stdunion\H_0}.
    \end{align*}

    Next, we apply the I.H. for $\phi_0$ and $\H_1$ and
    $\H_2$ to conclude $\SHi{2} \sidmodels \phi_0$
    %
    Furthermore, we apply the I.H. for formula
    $\phi_2$ and states $\SHpair{\S}{\H_1\stdunion\H_0}$ and
    $\SHpair{\S}{\H_2\stdunion\H_0}$ to conclude 
    $\SHpair{\S}{\H_2\stdunion\H_0} \sidmodels \phi_2$.
    %
    Hence, by the semantics of $\sept$ and $\wedge$, we have
    $\SHi{2}\sidmodels \phi_0 \wedge (\phi_1 \sept \phi_2)$.
    %
  \item[Case $\phi = \phi_0 \wedge (\phi_1 \mw \phi_2)$.]
    %
    Analogous to the previous case for guarded septraction, except that we must consider
    \emph{arbitrary} models $\H_0$ with $\SHi{0} \sidmodels \phi_1$
    and $\SHpair{\S}{\H_1 \stdunion \H_0} \sidmodels
    \phi_2$. \Cref{lem:sid:iso-models-same-formulas,lem:types:homo:compose},
    and the I.H. can then be applied just like in the
    case for septraction.
    %
    \qedhere
  \end{description}
\end{proof}
%


==> PartA/Insights.tex <==
% \chapter{An Overview of the Results / Approach / Insights of this
% Thesis}\label{ch:insights}
\section{Overview}\label{ch:insights}
\cmtodo{ToDo: Overhaul}
\cmtodo{Up to the first subsection, this is a mostly a good discussion of related work; we could also move parts of it into the introduction.}
  %
  In many variants of separation logic, systems of recursive equations
  can be used to define custom data structures.
  %
  Among these, ``shape-only'' symbolic-heap separation logic with
  inductive definitions, a generalization of the original
  symbolic-heap
  fragment~\cite{berdine2004decidable,berdine2005symbolic}, has
  received a lot of
  attention~\cite{brotherston2011automated,enea2014compositional,iosif2014deciding,serban2018entailment,ta2018automated,tatsuta2015separation,tatsuta2019completeness,sighireanu2019slcomp}.
  %
  Entailment in this logic is undecidable in
  general~\cite{antonopoulos2014foundations}, but a large fragment,
  which I denote $\SLIDbtw$ in this thesis, was shown decidable via
  reduction to monadic second-order logic by Iosif et
  al.~\cite{iosif2013tree}.
  \cmtodo{Undecidability is also shown in \cite{iosif2014deciding}}
  %
  Unlike most other decidable separation logics, this fragment allows
  definitions of data structures ``beyond trees,'' i.e., of data
  structures that are neither lists or trees. For example,
  binary trees with linked leaves can be defined in $\SLIDbtw$.

  Iosif et al.~\cite{iosif2013tree} did not propose a practical
  decision procedure for $\SLIDbtw$; the authors remarked in the
  follow-up paper~\cite{iosif2014deciding} that ``the method
  from~\cite{iosif2013tree} causes a blowup of several exponentials in
  the size of the input problem and is unlikely to produce an
  effective decision procedure.''
  %
  To circumvent this blowup, I develop a direct, model-theoretic
  decision procedure for an extension of $\SLIDbtw$.
  %
  This decision procedure proved to have potential in
  practice~\cite{sighireanu2019slcomp}, but takes
  double-exponential time in the size of the input in the worst case.
  %
  In light of a recent $\TwoExpTime$-hardness
  proof~\cite{echenim2019lower}, we now know that this asymptotic
  behavior is unavoidable.
  %procedure is
  %asymptotically optimal.

Let us look at this contribution in more detail.

Initially, separation logic was used for manual proofs of
program
correctness~\cite{ishtiaq2001bi,yang2001local,reynolds2002separation}.
%
The (unsurprising) undecidability of first-order separation
logic and a few decidability results were established early
on~\cite{calcagno2001computability},
but it took several more years until Berdine et al.~first showed the
% potential o automated reasoning a useful separation-logic fragment
applicability of SL-based reasoning in practice with the development
of \tool{Smallfoot}~\cite{berdine2005smallfoot}.\index{Smallfoot@\tool{Smallfoot}}
%
\tool{Smallfoot} uses a fragment of separation-logic as symbolic
states in symbolic execution~\cite{berdine2005symbolic}. This fragment
is since known as the \emph{symbolic-heap fragment} of separation
logic (see also \cref{sec:sl-intro:ar}).

Many tools, including \tool{Smallfoot}, have hardcoded support for a
small number of data structures, typically variants of lists or binary trees~\cite{berdine2004decidable,cook2011tractable,piskac2013automating,piskac2014automating,iosif2013tree,iosif2014deciding,echenim2020bernays}.
%
There has, however, been significant
theoretical~\cite{antonopoulos2014foundations,iosif2013tree} and
practical~\cite{sighireanu2019slcomp} work on the symbolic-heap
fragment with user-defined inductive definitions.
%
In this fragment, the user of the logic can define their own custom
data structures by providing a set of recursive equations that I call
\emph{systems of inductive definitions} (SIDs) and define formally in
\cref{ch:seplog}.
%
The formulas in the equations are themselves symbolic heaps. The
semantics of the user-defined predicates is then given by the least
fixed point of the equation system.
%
For example, the equations
%
\[
  \begin{array}{lll}
\gls{lsSIDlseg}(x_1,x_2) &\Rule& \pto{x_1}{x_2}\\
        \lseg(x_1,x_2) &\Rule& \SHEX{y} \ppto{x_1}{y} \sep
        \lseg(y,x_2)
  \end{array}
\]
      %
define a binary predicate $\lseg$ whose models are all nonempty
singly-linked list segments.

If arbitrary symbolic heaps are allowed in SIDs, the entailment
problem of the symbolic-heap fragment with inductive definitions is
undecidable~\cite{antonopoulos2014foundations}.
%
To obtain a decidable logic, it is thus necessary to restrict the
inductive definitions; for example, restricting them to linear
structures~\cite{gu2016complete} or tree
structures~\cite{tatsuta2015separation,tatsuta2019completeness,iosif2014deciding}.

It is, however, also possible to go beyond trees.
%
% There is a close connection between certain classes of graph gramm \cite{jansen2017static}
%
% This is, perhaps, not very surprising
Iosif et al.~\cite{iosif2013tree} proposed to restrict SIDs in a way
that guarantees that all models of the user-defined predicates (when
viewed as graphs) have bounded treewidth. I denote this fragment of
SIDs by $\gls{IDbtw}$ in this thesis.
%
The restriction to $\IDbtw$ made it possible to solve the entailment
problem for symbolic heaps via a reduction to the satisfiability
problem monadic second-order logic (MSO)
%
\index{monadic second-order logic}
\index{MSO|see{monadic second-order logic}}
%
over graphs of bounded treewidth
(BTW)\index{bounded treewidth}, which is decidable as a
consequence of a classical result by
Rabin~\cite{rabin1969decidability}.

In $\IDbtw$ we can, for example, define a predicate for trees with
linked leaves\index{tree with linked leaves} (TLL), which can be used
to implement an efficient sorted-set data structure.
%
I define such a predicate and display a small TLL in \cref{fig:tll-example}.

\begin{figure}[t!]
  \begin{subfigure}[b]{0.6\textwidth}
      $\begin{array}{lll}
        \gls{tll}(x_1,x_2,x_3) &\Rule& \ppto{x_1}{\tuple{\nil,\nil,x_3}} \sep (\sleq{x_1}{x_2})
        \\
        %
    \tll(x_1,x_2,x_3)& \Rule& \SHEX{\tuple{l,r,m}} \ppto{x_1}{\tuple{l,r,\nil}}
      \\&&\phantom{\SHEX{\tuple{l,r,m}}}\sep \tll(l,x_2,m)\\&&\phantom{\SHEX{\tuple{l,r,m}}} \sep \tll(r,m,x_3)
      \end{array}$
      \caption{The definition of the $\tll$ predicate representing trees
    with linked leaves.}
      \label{fig:ex:sid:tll}
    \end{subfigure}\hfill
     %
    \begin{subfigure}[b]{0.3\textwidth}
      \scalebox{0.6}{\input{gfx/PartA/tll-example}}
      \caption{A model of $\tll(x_1,x_2,x_3)$.}
      \label{fig:ex:sid:heap}
    \end{subfigure}
    %
  \begin{subfigure}[b]{0.6\textwidth}
      $\begin{array}{lll}
        \gls{tll}(x_1,x_2,x_3) &\Rule& \ppto{x_1}{\tuple{\nil,\nil,x_3}} \sep (\sleq{x_1}{x_2})
        \\
        %
    \tll(x_1,x_2,x_3)& \Rule& \SHEX{\tuple{l,r,m}} \ppto{x_1}{\tuple{l,r,\nil}}
      \\&&\phantom{\SHEX{\tuple{l,r,m}}}\sep \tll(l,x_2,m)\\&&\phantom{\SHEX{\tuple{l,r,m}}} \sep \tll(r,m,x_3)
      \end{array}$
      \caption{The definition of the $\tll$ predicate representing trees
    with linked leaves.}
      \label{fig:ex:sid:tll}
    \end{subfigure}\hfill
    %
    \caption[Example: SID defining trees with linked leaves]{A system of inductive definition (SID) defining trees
      with linked leaves. This SID is in the fragment $\IDbtw$
      introduced in \cite{iosif2013tree}.}\label{fig:tll-example}
\end{figure}

The satisfiability problem of MSO over graphs of BTW is non-elementary,
but the reduction in \cite{iosif2013tree} has a bounded number of
quantifier alternations, leading to an elementary recursive decision
procedure
% ; the decision procedure
that is, however, still several times
exponential~\cite{iosif2014deciding}.

My primary goal in \cref{pt:btw} is to develop a more practical
decision procedure for separation logic with inductive definitions
from $\IDbtw$.
%
I present a direct model-theoretic decision procedure, as opposed to a
reduction to a different formalism.
%
This decision procedure runs in double-exponential time in the worst case.
%
Granted, this does not sound all that practical; fortunately, the performance in
practice is much better than the asymptotic complexity would
suggest~\cite{sighireanu2019slcomp}.
%
Moreover, there is no hope to obtain a decision procedure with better
asymptotic behavior: The entailment problem for $\IDbtw$ was recently
shown to be hard for $\TwoExpTime$~\cite{echenim2019lower}.

I also address the question of whether we can allow arbitrary
definitions from $\IDbtw$, but go beyond the symbolic-heap fragment. I
show that it is possible to allow classical conjunction and
disjunction, as well as \emph{guarded} variants of negation, magic
wand, and septraction, i.e., formulas of the form $\phi\wedge \neg
\psi$, $\phi \wedge (\psi_1\mw\psi_2)$ and $\phi \wedge
(\psi_1\sept\psi_2)$. I also show that allowing any of these three
operators without guards yields an undecidable logic.
%
This leaves us with an almost complete picture of the decidability
landscape for separation logics with $\IDbtw$ definitions.
  

\cmtodo{Perhaps the term Satisfiability Checking is confusing giving that the paper is about entailment checking?}
\subsection{Abstraction-Based Satisfiability
  Checking}\label{sec:insights:abstraction}
\index{abstraction!for satisfiability checking}

As discussed earlier in this chapter, both \cref{pt:ssl} and
\cref{pt:btw} are centered around a decision procedure for a variant
of SL.
%
Both of these decision procedures are based on a \emph{compositional
  abstraction}\index{compositional abstraction} that \emph{refines}
the satisfaction relation of the respective SL variant.
%
In this section, I briefly discuss this approach in a generic setting. % I've also included references to the corresponding results
% in \cref{tbl:comparison}

Let $\SLgeneric$ be a variant of separation logic.
\cmtodo{I would remove stacks and heaps here in favor of a more generic notion of memory $\mathfrak{m}$ as stack-heap pairs are not really defined yet.
Furthermore, I would prefer ``memory'' for a well-defined stack-heap pair over ``model'' as model is occasionally also used as a stack-heap pair that satisfies a formula (a model of...)}
%
We are looking for a finite abstract domain $\AD$ and an
abstraction function $\genabst\colon \SS\times\HH \to \AD$ with the
following key properties.
%
\begin{description}
\item[Refinement.]\index{refinement} If
  $\genabst(\S,\H_1)=\genabst(\S,\H_2)$, then $\SHi{1}$ and $\SHi{2}$
  satisfy the same $\SLgeneric$ formulas, so the equivalence relation
  induced by the abstraction function,
  \[
    \SHi{1} \equiv_\genabst \SHi{2} \text{ iff } \genabst(\S,\H_1)=\genabst(\S,\H_2),
  \]
  refines the satisfaction relation.
  %
 % \TODO{Really state this for fixed stack?}
\item[Compositionality.]\index{compositionality} There exists an
  operation $\Compose\colon \AD\times\AD \pfun \AD$ such that
  %
  $\genabst(\S, \H_1 \sqcup \H_2) = \genabst(\S,\H_1) \ACompose
  \genabst(\S,\H_2)$, where $\sqcup$ is the notion of disjoint union
  used to give the semantics to the separating conjunction. (This
  notion of disjoint union will differ between \cref{pt:ssl,pt:btw}.)
\end{description}

Refinement and compositionality make it possible to go from the
function $\genabst\colon \SS\times\HH \to \AD$ to a function
%
\begin{align*}
   \genabst_\SLgeneric\colon & \SLgeneric \to \AD,\\
  & \phi \mapsto \set{ \genabst(\S,\H) \mid \SH \models \phi },
\end{align*}
%
because
%
\begin{enumerate}
\item if $a \in \genabst_\SLgeneric(\phi_1) \cap
  \genabst_\SLgeneric(\phi_2)$ then $a \in
  \genabst_\SLgeneric(\phi_1\wedge \phi_2)$ (by refinement), and
\item if $a_1 \in \genabst_\SLgeneric(\phi_1)$ and $a_2 \in
\genabst_\SLgeneric(\phi_2)$ then $a_1 \Compose a_2 \in \genabst_\SLgeneric(\phi_1\sep\phi_2)$ (by
  compositionality).
\end{enumerate}
%
Provided we come up with a way to compute the abstraction of atomic
formulas, we can then use $\genabst_\SLgeneric$ for satisfiability checking:
$\genabst_\SLgeneric(\phi)\neq\emptyset$ iff $\phi$ is satisfiable.

\cmtodo{I like the overview so far. A few items are missing here though. In particular, the forget operation should also be motivated. Moreover, one should briefly mention more generally, that our abstraction should be compositional with respect to all the logical operators of our SL variant. It then makes sense that we pick $\sep$ as an example because every SL variant should support it.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> PartA/SLIntro.tex <==
\section{An Introduction to Separation Logic}\label{ch:sl-intro}

\cmtodo{I would put general notation in its own section}

\subsection{Notation}\label{sec:notation}

In this section, I establish the basic notational conventions that I
use both later in this chapter and in the main parts of this thesis,
\cref{pt:ssl,pt:btw}.

\paragraph*{Ordered sequences.}

Ordered sequences are denoted in boldface, e.g., $\vec{x}$.
The %size 
\cm{length} of the sequence $\vec{x}$ is $\size{\vec{x}}$.
%
To list the elements of a sequence, I write $\gls{--zz-seq}$.
%
Further, I often omit the brackets around single-element
sequences---i.e., write $x$ instead of $\tuple{x}$---to reduce
clutter.

The empty sequence is $\gls{-E-emptyseq}$ ann the concatenation of
$\vec{x}$ and $\vec{y}$ is $\vec{x}\gls{---concat}\vec{y}$.
%, and
%$\vec{x}\gls{--rel-subseq}\vec{y}$ expresses that $\vec{x}$ is a
%sub-sequence of $\vec{y}$.

As usual, $A^{*}$ denotes finite sequences over $A$, $A^{+}$ denotes
nonempty finite sequences over $A$.

Moreover, I frequently treat sequences as sets when convenient and
order does not matter. For example, $x \in \vec{x}$ states that the
sequence $\vec{x}$ contains the element $x$, $\vec{x}\cup\vec{y}$ is
the set that contains the elements of both sequences, etc.

\paragraph*{Functions.}
I write $f\colon A \gls{---pfun} B$ to denote a partial function from
$A$ to $B$; $\gls{dom-f}$ is the domain of (partial) function $f$ and
$\gls{img-f}$ is the image of (partial) function $f$.
%
The fact that partial function $f$ is undefined on $x$ is denoted
$f(x)=\gls{---bot}$.
%
As usual, $f \mathbin{\gls{---funcomp}} g$ is the composition of
functions $f$ and $g$ that maps $x$ to $f(g(x))$.

We will also need notation to compare partial functions:
\begin{enumerate}
\item For functions $f,g\colon A\pfun B$, $f\subseteq g$ holds if
  $\dom(f)\subseteq\dom(g)$ and $f(a)=g(a)$ for all $a \in \dom(f)$.
\item For functions $f,g\colon A\pfun 2^B$,
  $f \mathrel{\gls{--rel-subfun}} g$ holds if
  $\dom(f)\subseteq\dom(g)$ and $f(a)\subseteq g(a)$ for all
  $a \in \dom(f)$.
\end{enumerate}

I frequently use set notation to define and reason about partial
functions. For example,
$\set{x_1 \mapsto y_1, \ldots, x_k \mapsto y_k}$ is the partial
function that maps $x_i$ to $y_i$, $1 \leq i \leq k$, and is undefined
on all other values. Consequently, $\emptyset$ represents a function
that is undefined everywhere.
%
$f \cup g$ is the (not necessarily disjoint) union of partial
functions $f$ and $g$; it is only defined if $f(x)=g(x)$ for all
$x \in \dom(f)\cap\dom(g)$.
%
The size of a partial function $f$ is the size of its domain, i.e.,
$\size{f} \defn \size{\dom(f)}$.

Finally, the following conventions will simplify defining and using
functions.
%improve readability when
%defining and using function.
\begin{description}
\item[Lifting functions to sequences.] For $f\colon A \pfun B$ and
  $\vec{a}\in A^{*}$, then $f(\vec{a})$ for the point-wise
  application of $f$ to $\vec{a}$, i.e.,
  \[f(\tuple{a_1,\ldots,a_k})\defn\tuple{f(a_1),\ldots,f(a_k)}.\]
\item[Omitting brackets.] If $f\colon A^{*} \pfun B$, I sometimes
  write $f(a_1,\ldots,a_k)$ instead of $f(\tuple{a_1,\ldots,a_n})$ to
  improve readability.
\item[Lambda notation.] The expression $\gls{-L-lambda} x\ldotp f(x)$
  defines an anonymous (partial) function that maps $x$ to $f(x)$.
\end{description}
\cmtodo{Lambda notation seems to be used only at the end of this part of the thesis. I would introduce it ad hoc.}

% \paragraph*{Complexity.}
% \TODO{Introduce complexity notation $\bigO, \Theta$ and complexity classes $\PTime,\NP,\coNP,\PSpace,\ExpTime,\TwoExpTime$?} %

%\paragraph*{Other notation?}
%
%$\N$ are the natural numbers.
% logarithm

%\begin{infobox}{Additional information}
%  Throughout this thesis, you will from time to time encounter boxes
%  like this one.
%  %
%  I use these boxes to shed light on the larger context or provide
%  additional information that is connected to the content at
%  hand. Reading the boxes is not necessary for following the technical
%  development.
%\end{infobox}
\cmtodo{I would convert the info boxes to remarks where appropriate.}

\cmtodo{The preliminaries are more general than necessary (probably due to other parts of the thesis); we should write a more condensed form such that we can quickly move to the contributions; I can try to write a compact version of sections 3 and 4.}

\subsection{A Basic First-Order Separation
  Logic}\label{sec:sl-intro:formal}

Over the course of this thesis, I will study multiple variants of
separation logic. I will introduce the syntax and semantics of these variants as needed
in \cref{pt:ssl,pt:btw} of the thesis.

In this section, I formalize a simple first-order separation logic,
$\gls{SLbase}$. This gives me the chance to introduce the
\emph{stack--heap model} and formalize the separate connectives in a
simple setting.
%
Moreover, $\SLbase$ will serve as the basis for a discussion about
alternative semantics of the separating connectives in
\cref{ch:insights}.

\subsection{The Syntax of Separation Logic}\label{sec:sl-intro:syntax}
\index{syntax!of SLbase@of $\SLbase$}

\begin{figure}
  \centering
  $
  \begin{array}{lll}
  \phiAtom & ::= & \emp \mid \pto{x}{\tuple{y_1,\ldots,y_k}} \mid
                   \sleq{x}{y} \mid \slneq{x}{y} \\
                   %
  \phi & ::= & \phiAtom \mid \phi \sep \phi \mid \phi \mw \phi \mid
               \phi \wedge \phi \mid \phi \vee \phi \mid \neg \phi
               \mid \EXO{x}\phi \mid \FAO{x}\phi\\
    %
    % \phiSH & ::= & \EXO{\underbrace{x_1,\ldots,x_k}_{k \geq 0}} \underbrace{\phiAtom \sep \cdots
    %                \sep \phiAtom}_{\text{1 or more atoms}}
  \end{array}
  $
  \caption[Syntax of $\SLbase$]{The syntax of a
    first-order separation logic} %and its symbolic-heap fragment}
  \label{fig:sl:generic-syntax}
\end{figure}

In \cref{fig:sl:generic-syntax}, I define the syntax of the
first-order separation logic $\SLbase$.
% (formulas $\phi$) and its \emph{symbolic-heap
% fragment}~\index{symbolic-heap fragment} (formulas $\phiSH$).
%

% If you are familiar with separation logic, the choice of atomic
% formulas may seem rather limited to you; we will consider richer
% variants of SL later in the thesis.

% I've included several common atomic formulas $\phiAtom$, but the exact
% set of atomic formulas depends on the variant of separation logic, as
% does the availability of operators and quantifiers.

Informally, the meaning of the atomic formulas is as follows.
\begin{itemize}
\item The \emph{empty-heap predicate}\index{empty-heap predicate}
  $\gls{emp}$ denotes the empty heap.
  %
\item The \emph{points-to assertion}\index{points-to assertion}
  $x \mathbin{\gls{--pto}} \tuple{y_1,\ldots,y_k}$ expresses that the pointer
  variable $x$ points to a heap-allocated object that consists of $k$
  fields that store the values of the variables $y_1,\ldots,y_k$.
  %
\item \index{equality}\index{disequality}
  %
  (Dis-)equalities $x\mathbin{\gls{--rel-sleq}}y$ and
  $x\mathbin{\gls{--rel-slneq}}y$ express that the pointer variables
  $x$ and $y$ alias and that they don't alias, respectively.
  %
% \item The predicate $\ls(x,y)$ states that the heap contains a
%   singly-linked list segment from $x$ to $y$ of arbitrary length.
\end{itemize}
%
The predicates $\emp$ and $\pto{\cdot}{\cdot}$ are often called
\emph{spatial} atoms because they describe the spatial layout of the
heap, whereas (dis-)equalities are often called \emph{pure}
atoms~\cite{ishtiaq2001bi}\index{pure}\index{spatial}.

The atomic formulas defined in \cref{fig:sl:generic-syntax} give rise
to a rather minimalistic separation logic. Most separation logics
provide additional atomic formulas.
%
Later in this thesis, I will consider an SL variant with built-in
atoms representing lists and trees as well as atoms for reasoning
about the data stored inside the heap (\cref{pt:ssl}). I will also
consider an SL variant with a mechanism for user-defined predicates
(\cref{pt:btw}).

In $\SLbase$, formulas are built using classical propositional
connectives $\wedge,\vee,\neg$, quantifiers $\exists,\forall$, as well
as a set of \emph{separating connectives}\index{separating
  connective}, the aforementioned separating conjunction
$\gls{--sl-sep}$ and its right adjoint, the \emph{separating
  implication}\index{separating implication} $\gls{--slwand-mw}$. Because
of the appearance of the separating implication, most people use the
moniker \emph{magic wand}\index{magic wand} instead. As usual, we can
derive additional operators such as classical implication
$\phi\Rightarrow\psi \defn \neg \phi \vee \psi$ and \emph{septraction}
$\phi \gls{--slwand-sept} \psi \defn \neg (\phi \mw \neg
\psi)$~\cite{brochenin2012almighty,thakur2014satisfiability}.\index{septraction}

Let us contrast the meaning of the classical and separating
connectives.
%
While $\phi \wedge \psi$ means that the program state satisfies both
$\phi$ and $\psi$ simultaneously, $\phi \sep \psi$ denotes that the
program state can be split into two disjoint parts which separately
satisfy $\phi$ and $\psi$. In particular, there can be no aliasing
between the two disjoint parts of the program state, which implies the
soundness of the frame rule introduced in
\cref{sec:sl-intro:motivation}.
%
Similarly, while $\phi \Rightarrow \psi$ means that every program
state that satisfies $\phi$ also satisfies $\psi$, $\phi \mw \psi$
means that the \emph{extension} of the program state with any program
state that satisfies $\phi$ yields a program state that satisfies
$\psi$.

The magic wand is particularly useful for weakest-precondition
reasoning\index{weakest-precondition calculus}, for example to express
memory allocation~\cite{ishtiaq2001bi,reynolds2002separation}.
%
In much of the separation-logic literature as well as in the bulk of
the tools, the magic wand is not considered or only partially
supported, however, because its inclusion in a separation logic
quickly leads to
undecidability~\cite{appel2014program,blom2015witnessing,schwerhoff2015lightweight}.
\cmtodo{I want to mention both Iris and QSL here :)}

% Unfortunately, the magic wand is notoriously hard to automate and
% thus often not considered
%
% Unfortunately, including the magic wand in a separation logic quickly
% leads to undecidability.
% %
% Most tools do in, fact, not only disallow the magic wand, but remove
% every operator except for the separating conjunction~\cite{TODO}.
% %
% The resulting logic is known as the \emph{symbolic-heap
%   fragment}\index{symbolic-heap fragment} of separation
% logic~\cite{berdine2005symbolic} and defined as formulas of the form
% $\phiSH$ in \cref{fig:sl:generic-syntax}.

\subsection{The Semantics of Separation
  Logic}\label{sec:sl-intro:semantics}
\index{stack--heap pair}

\paragraph*{The stack--heap model.} In this thesis, I use
\emph{stack--heap pairs} as models of SL
formulas. While clearly not the only possible model of separation
logics for reasoning about unbounded data structures, it has been the
most-widely used model ever since the first papers on SL were
written~\cite{ishtiaq2001bi,reynolds2002separation}.
%
A stack--heap pair is a pair of partial functions $\SH$. The
\emph{stack}\index{stack} $\gls{s}$ is a partial function from
(program and logical) variables to some set(s) of values.
%
The set(s) of values may be identical to or subsume the set of
addressable \emph{memory locations}.
%
The \emph{heap}\index{heap} $\gls{h}$ is a partial function from
memory locations to ordered sequences of values.

Let us formalize these definitions.
%
Throughout this thesis, $\gls{Var}$ denotes a countable infinite set
of variables with $\gls{nil} \in \Var$. Here, $\nil$ can be seen as an
auxiliary constant that we can use to refer to the null
pointer\index{null pointer} in separation-logic formulas.
%
% \TODO{Originally defined order on Var here, but it's annoying to have
%   that so early in the thesis.}

We also need a countably infinite set of addressable memory locations
$\gls{Loc}$ and a set of values $\gls{Val}$ with
$\Loc \subseteq \Val$.
%
Note that interpreting $\Loc$ by an infinite set is a deliberate
abstraction from the (finite, e.g. 64 bit) address space of a real
program.
%
In a ``shape-only'' separation logic whose formulas constrain only the
shape, not the content of the heap, we can simply set $\Val \defn
\Loc$. This will be the case in \cref{pt:btw}.
%
If we want to combine reasoning about shape and content, we also need
to model the data stored in the heap, so $\Val$ will subsume both the
locations and a data domain. This will be the case in \cref{pt:ssl}.

A \emph{stack}\index{stack} is a finite partial function
$\S\colon \Var \pfun \Val$.
%
I implicitly assume $\nil \in \dom(\S)$ for every stack, but unless
$\nil$ is relevant for an example at hand, I often do not explicitly
include $\nil$ when defining stacks.
%
A \emph{heap}\index{heap} is a finite partial function $\H \colon \Loc
\pfun \Val^{+}$ that maps locations to ordered sequences of values.
%
By mapping to a sequence rather than a single location, the heap maps
every allocated memory location to the entire structure allocated at
this location. This is a fairly standard (but far from
ubiquitous~\cite{reynolds2002separation,calcagno2006beyond})
abstraction from actual memory layout; it simplifies the model and
does not lose precision as long as we are not interested in pointer
arithmetic\index{pointer arithmetic} or other word-level operations.
%
I write $\gls{Stacks}$ for the set of all stacks and $\gls{Heaps}$ for
the set of all heaps.

\cmtodo{The term model is also used as ``model of a formula'', e.g. in the very first figure and throughout the rest of the thesis. Can we agree to use a more generic term here? We could call this a program state (already used in Sec. 3.3) or ``memory''.}
A \emph{model}\index{model} is a stack--heap pair $\SH$ with
$\S(\nil)\notin\dom(\H)$, reflecting that the null pointer cannot be
allocated.

\paragraph*{Semantics.}
I define a semantics for our basic first-order separation logic
$\SLbase$ in \cref{fig:sl:generic-semantics}.

\begin{figure}[tb!]
  \centering
  $
  \begin{array}{lll}
    \SH \models \emp & \text{iff} & \H = \emptyset\\
    %
    \SH \models \sleq{x}{y} & \text{iff} & \S(x)=\S(y) \text{ and
                                           }\H=\emptyset\\
                                           %
    \SH \models \slneq{x}{y} & \text{iff} & \S(x)\neq\S(y) \text{ and
                                           }\H=\emptyset\\
    %
    % \SH \models \pto{x}{\tuple{y_1,\ldots,y_k}} & \text{iff} & \H =
    %                                                            \set{\S(x)
    %                                                            \mapsto
    %                                                            \tuple{\S(y_1),\ldots,\S(y_k)}}
    % \\
    \SH \models \pto{x}{\vec{y}} & \text{iff} & \H =
                                                               \set{\S(x)
                                                               \mapsto
                                                              \S(\vec{y})}
    \\
                                      %
    \SH \models \phi \sep \psi & \text{iff} & \text{ex.~} \H_1,\H_2
                                              \text{~s.t.~}
                                              \H_1\cap\H_2=\emptyset,
                                              \H=\H_1\cup\H_2,\\&&
                                              \SHi{1}\models\phi,
                                              \text{ and }
                                              \SHi{2}\models \psi\\
                                                                   %
    \SH \models \phi \mw \psi & \text{iff} & \text{for all } \H_0,
                                              \text{ if }
                                              \H_0\cap\H=\emptyset
                                             \text{ and }
                                              \SHi{0} \models \phi\\&&
                                              \text{then }
                                              \SHpair{\S}{\H_0\cup\H}\models \psi\\
    %
    \SH \models \phi \wedge \psi & \text{iff}  & \SH \models \phi
                                                 \text{ and } \SH
                                                 \models \psi \\
                                      %
    \SH \models \phi \vee \psi & \text{iff}  & \SH \models \phi
                                                 \text{ or } \SH
                                                 \models \psi \\
                                      %
    \SH \models \neg\phi & \text{iff} & \SH \nvDash \phi \\
    %
    \SH \models \EXO{x}\phi & \text{iff} & \text{ex. } \ell\in\Loc
                                           \text{ s.t.~} \SHpair{\S
                                           \cup \set{x \mapsto
                                           \ell}}{\H} \models \phi\\
    %
    \SH \models \FAO{x}\phi & \text{iff} & \text{for all } \ell\in\Loc,
                                           \SHpair{\S
                                           \cup \set{x \mapsto
                                           \ell}}{\H} \models \phi\\
  \end{array}
$
  \caption[Semantics of $\SLbase$]{A semantics of
    first-order separation logic.\index{semantics!of SLbase@of $\SLbase$}}
  \label{fig:sl:generic-semantics}
\end{figure}

The empty-heap predicate $\emp$ holds iff the heap is empty;
equalities and disequalities between variables hold iff the stack maps
the variables to identical and different values, respectively.
%
For (dis-)equalities, I additionally require that the heap is
empty. This is nonstandard, but not
unprecedented~\cite{piskac2013automating}, and will simplify some of
the development later in this thesis.

\cmtodo{The term precise originated in the PhD thesis of Yang}
A points-to assertion $\pto{x}{\tuple{y_1,\ldots,y_k}}$ holds in a
singleton heap that allocates only the location $\S(x)$ and stores the
values $\S(y_1),\ldots,\S(y_k)$ in this location. This is often called
a \emph{precise}~\cite{calcagno2007local} semantics, because the heap
contains precisely the object described by the points-to assertion,
nothing else.%---in contrast to an \emph{intuitionistic} semantics,

The separating connectives are formalized in terms of disjoint unions
of heap functions: in the standard semantics presented here,
$\SH \models \phi \sep \psi$ if and only if there exist
domain-disjoint functions $\H_1$, $\H_2$ such that their point-wise
union is $\H$ and such that $\SHi{1}\models\phi$ and
$\SHi{2}\models\psi$. I will argue in \cref{ch:insights} and
\cref{pt:ssl} that there are other reasonable semantics for $\sep$
that may simplify automated reasoning about the logic.

While the separating conjunction is about splitting the heap, the
magic wand is about extending the heap: $\SH \models \phi \mw \psi$
if all ways to extend $\H$ with a disjoint model of $\phi$ yields a
model of $\psi$.

The semantics of the Boolean operators and the quantifiers is
standard; for simplicity I only allow quantifying over locations, not
over arbitrary values. This is necessary because variables in
$\SLbase$ (as well as the other logics in this thesis) are not
sorted---their interpretation is not constrained to either $\Loc$ or
$\Val\setminus\Loc$---and it rarely makes sense for a single variable
to range both over memory locations and over the domain of data values
stored in the heap.

% The semantics \cref{fig:sl:generic-semantics} is merely a starting
% point for this thesis. I will later consider additional atomic
% formulas, as well as different semantics for the separating
% connectives.

\begin{example}
  \begin{enumerate}
  \item $\ppto{x}{y} \sep \ppto{y}{\nil}$ states that the heap consists
    of exactly two objects, one pointed to by $x$, the other pointed
    to by $y$; that the object pointed to by $x$ contains a pointer to
    the object pointed to by $y$; and that the object pointed to by
    $y$ contains a null pointer.
    %
    Put less precisely but more concisely, $x$ points to $y$, $y$
    points to $\nil$, and $x$ and $y$ are separate objects in the
    heap.
    %
    The precise semantics of points-to assertions guarantees that
    there are no other objects in the heap.
    %
  \item $\ppto{x}{y}\wedge\ppto{z}{y}$ states that (1) the heap consists
    of a single object $x$ that points to $y$ and that simultaneously
    (2) the heap consists of a single object $z$ that points to $y$.
    %
    This formula is only satisfiable in stacks $\S$ with
    $\S(x)=\S(z)$.
    %
  \item $\ppto{x}{y} \mw \ppto{z}{y}$ states that after adding a pointer
    from $x$ to $y$ to the heap, we obtain a heap that contains a
    single pointer from $z$ to $y$.
    %
    This formula is only satisfiable in the empty heap and in stacks
    $\S$ with $\S(x)=\S(z)$.
    %
  \item
    $\FAO{x} \ppto{x}{\nil} \mw ((\neg \emp) \sep (\neg \emp))$
    states that the heap contains at least one pointer: No matter
    which variable we allocate additionally, the resulting heap can be
    split into two nonempty parts, so the original heap must itself
    have been nonempty.
    %
    We could, of course, state this property more succinctly as $\neg \emp$.
    %
  \end{enumerate}
\end{example}

\subsection{Automated Reasoning about Separation
  Logic}\label{sec:sl-intro:ar}\index{automated reasoning}
%
While program verification and --analysis are the motivation for
studying separation logic, they are not the focus of this
thesis. Instead, I mainly focus on \emph{automated reasoning} about
separation-logic formulas.
%
Roughly speaking, such automated reasoning forms the backend of an
automated verifier or static analyzer based on SL: the verifier or
analyzer generates \emph{queries}, i.e., SL formulas, which we would
like to answer automatically.
%
This leads to the following two decision problems.
\begin{itemize}
\item The \emph{satisfiability problem}\index{satisfiability problem}:
  given an SL formula $\phi$, is there a model $\SH$ that satisfies
  $\phi$?
\item The \emph{entailment problem}\index{entailment problem}: given
  two formulas $\phi$, $\psi$, is it the case that all models that
  satisfy $\phi$ also satisfy $\psi$?
\end{itemize}

We already saw in \cref{sec:sl-intro:motivation} that the entailment
problem is central to Hoare-style deductive verification: the rule of
consequence involves two instances of the entailment problem.  This is
in contrast to most other Hoare-logic rules, which can be applied
purely syntactically.
%
Given this central role of \emph{entailment checking} in deductive
verification, it is not surprising that the entailment problem has
received the bulk of the attention in the corner of the separation-logic
literature that is concerned with automated deduction~\cite{berdine2004decidable,brotherston2011automated,enea2014compositional,enea2017spen,iosif2013tree,iosif2014deciding,navarro2013separation,serban2018entailment,sighireanu2019slcomp,ta2018automated,tatsuta2015separation,tatsuta2019completeness}.

For the first-order separation logic $\SLbase$ defined in this
section, satisfiability and entailment are, of course, undecidable.
After all, the logic is an extension of first-order logic, which is
already undecidable.

Many fragments of separation logic with decidable entailment problems
have been proposed and
implemented~\cite{berdine2004decidable,iosif2013tree,iosif2014deciding,piskac2013automating,piskac2014automating,serban2018entailment,tatsuta2015separation,tatsuta2019completeness};
usually, these fragments restrict or disallow quantifiers, the magic
wand, and negation. I attempt a more-or-less thorough overview of the
``decidability landscape'' in \cref{ch:related-work}.

\begin{infobox}{The symbolic-heap fragment}
  Much effort has been put into automated reasoning about the
  \emph{symbolic-heap fragment}\index{symbolic-heap fragment}. This
  fragment is suitable as an abstract domain in program
  analyses~\cite{berdine2005symbolic} and expressive enough to write
  interesting specifications. At the same time, reasoning about
  symbolic heaps is
  tractable~\cite{cook2011tractable} or at least decidable, even when
  considering quite general data structures~\cite{iosif2013tree}; as
  such, this fragment has also been the main focus of the
  \emph{Competition of Solvers for Separation Logic}~\cite{sighireanu2019slcomp}.
  \index{SL-COMP}\index{separation logic competition}

  A symbolic heap is a formula of the form
  %
  \[
\EXO{\underbrace{x_1,\ldots,x_k}_{k \geq 0}} \underbrace{\phiAtom \sep \cdots
                    \sep \phiAtom}_{\text{1 or more atoms}}.
  \]
  %
  Since negation is not allowed in symbolic heaps, the entailment
  problem for symbolic heaps is genuinely different from the
  satisfiability problem---it is impossible to solve an entailment
  $\phi \models \psi$ by checking the unsatisfiability of
  $\phi \wedge \neg \psi$, because the latter formula is not a
  symbolic heap.
\end{infobox}


This thesis can be seen as a search for the right trade-off
between expressiveness and tractability---to find a separation logic
in which we can express and prove interesting properties, and for
which automation of the entailment problem is also feasible.
%
Obviously, there is not the one right trade-off; depending on your
goals and target applications, quite different trade-offs may be
appropriate.
%
For example, if you need a lightning fast bug finder, you may go for a
logic that is not very expressive and try to solve queries in this
logic with a set of fast but incomplete
heuristics~\cite{calcagno2011compositional}.
%
Conversely, if you're interested in building a deductive-verification
tool for code annotated with contracts and loop invariants, you may
prefer a more expressive logic that allows you to prove more complex
properties of the
program~\cite{chin2012automated,qiu2013natural,piskac2014grasshopper}.

% I like designing decision procedures, as it forces you to understand a
% reasoning problem deeply, including all corner cases.
% %
% Such a deep understanding
% Decidability, of course, is not a prerequisite for
% automation. Incomplete heuristics may be good enough in practice.
% %
% Once again, this depends on your specific goals.
 % \TODO{Say here or somewhere in the
 %  thesis: While undecidability isn't a showstopper, decidability /
 %  decision procedures are still useful: What's possible? Understand
 %  the problem deeply. Something to fall back to when heuristics
 %  fail. Etc.}

\subsection[Reasoning about Stack--Heap Models]{Reasoning about Stack--Heap Models: Locations, Isomorphism, Aliasing}\label{sec:sl-intro:other}
\cmtodo{I would like to introduce most of these notions where needed or at least at the end of the preliminaries in a clearly labeled subsection.}

Several concepts appear again and again throughout
\cref{pt:ssl,pt:btw}: we need to distinguish between several types of
locations; we need to reason about \emph{isomorphism}; and we need to
keep track of \emph{aliasing}.
%
I formalize these terms below.
%
This section is meant as a reference section; you can skim it on a
first reading. All notation introduced below also appear in the
\emph{List of Symbols} at the beginning of this document.

\paragraph*{Locations.} We will frequently have to reason about the
locations in a heap. Let $\S\in\SS$ be a stack and let $\H \in \HH$
be a heap.
%
A location $\ell$ is \emph{labeled}\index{labeled location} iff
$\ell\in\img(\S)$.
%
We let
$\gls{locs-h} \defn \dom(\H) \cup ((\bigcup\img(\H))\cap\sbothloc)$.
%
A location $\ell \in \Loc$ is an \emph{allocated
  location}\index{allocated location} in $\H$ if $\ell \in \dom(\H)$
and a \emph{referenced location}\index{referenced location} if
$\ell \in \img(\H)$.
  %
  Similarly, a variable $x$ is allocated or referenced if $\S(x)$ is
  allocated or referenced, respectively.

  A location $\loc$ is \emph{dangling}\index{dangling locations} if
  $\loc \in \locs{\H}\setminus\dom(\H)$ and a variable $x$ is dangling
  if $\S(x)$ is dangling. We collect all dangling locations of a heap
  $\H$ in $\gls{danglinglocs}$.

  We define $\gls{alloced} \defn \set{x \mid \S(x)\in\dom(\H)}$ and
  $\gls{refed} \defn \set{x \mid \S(x)\in\img(\H)}$, i.e., the sets of
  \emph{allocated variables}\index{allocated variables} and
  \emph{referenced variables}\index{referenced variables} of the model
  $\SH$.

\paragraph*{Isomorphism.}

Two models are isomorphic if one can be transformed into
the other by renaming locations.

\begin{definition}[Isomorphic
  models]\label{def:slbase:iso}\index{isomorphism!of models}
  Let $\SH,\SHpair{\S'}{\H'}$ be models. $\SH$ and $\SHpair{\S'}{\H'}$
  are \emph{isomorphic}, $\SH \gls{--eq-Iso} \SHpair{\S'}{\H'}$, if there exists
  a bijection
  \[\renfun\colon \Val \to \Val\] such that
\begin{enumerate}
\item for all $v \in \Val \setminus \Loc$, $\renfun(v)=v$,
  \item for all $x$, $\S'(x) = \renfun(\S(x))$, and
  \item
    $\H' = \{ \renfun(\ell) \mapsto \renfun(\H(\ell)) \mid \ell \in
    \dom(\H)\}$.
  \end{enumerate}
  We call $\renfun$ a \emph{witness} of the
  isomorphism.\index{witness!of isomorphism}
\end{definition}

By demanding in \cref{def:slbase:iso} that the bijection $\renfun$ is
the identity on $\Val\setminus\Loc$, we capture that the two heaps
must agree on the data stored inside the allocated heap locations.

Neither the logic $\SLbase$, nor the logics $\SSLpdata$ and $\SLIDea$
studied in \cref{pt:ssl,pt:btw} can distinguish between isomorphic
models.

\paragraph*{Aliasing.}%\label{sec:prelim:aliasing}

In general, the stack may map multiple variables to the same location,
i.e., variables may be aliases.

We sometimes need to pick a variable from sets of aliases.
%
To make this choice consistently, I assume a linear order on $\Var$
and denote by $\gls{max-v}(\vec{v})$ the maximal variable among a
finite set of variables $\vec{v}$ according to this order.

For example, we need the \emph{\stkchoicefun{}}\index{stack-choice function}
of stack $\S$, a partial function that maps every location
$\ell\in\img(\S)$ to a variable $x$ with $\S(x)=\ell$.

\begin{definition}[Stack inverse and \stkchoicefun{}]\label{def:sid:stack-inverse}
  Let $\S$ be a stack.
  \begin{enumerate}
  \item The function $\gls{s-1} \defn \set{ l \mapsto \set{x \mid \S(x)=l}}$
    is the \emph{stack inverse}\index{stack inverse}
    %
  \item
    The function $\gls{s-1-max} \defn \set{ l \mapsto
      \max(\stkinv(l))}$ is the \emph{\stkchoicefun{}} of $\S$.
    % \[\gls{s-1} \defn \set{ l \mapsto \max\set{x \mid \S(x) = l} \mid
    %     l \in \img(\S) }\] is the \emph{\stkchoicefun{}} of $\S$.
  \end{enumerate}

\end{definition}

Stack aliasing induces an equivalence relation, the
\emph{stack-aliasing constraint}\index{stack-aliasing constraint} of
$\S$ given by
%
\[\gls{aliasing} \defn \set{(x,y) \mid x,y\in\dom(\S) \text{ and }
    \S(x)=\S(y)}.\]
%
The equivalence class in $\eqclasses{\S}$ of variable $x$ is
\[\gls{--zz-eqclass} \defn \set{y \mid \S(y)=\S(x)}.\]
  % \item
  Just like with other functions, I sometimes apply
  $\eqclassAMS{\S}{\cdot}$ to sequences in a point-wise manner, i.e.,
  write $\eqclassAMS{\S}{\tuple{y_1,\ldots,y_k}}$ as shorthand for
  $\tuple{\eqclassAMS{\S}{y_1},\ldots,\eqclassAMS{\S}{y_k}}$.
%
  The set of all equivalence classes of $\S$ is
  \[\gls{classes-s} \defn \set{\eqclassAMS{\S}{x} \mid x \in
      \dom(\S)}.\]

  Finally, the following auxiliary notation will simplify reasoning
  about stack aliasing.
%
\begin{itemize}
  %
\item I frequently denote a fixed stack-aliasing constraint by
  $\gls{-S-scls}$.
\item The \emph{domain} of stack-aliasing constraint $\scls$ are
  all variables on which $\scls$ is defined, i.e.,
  $\gls{dom--scls} \defn \set{x \mid (x,x)\in\scls}$.
\item The \emph{restriction} of stack-aliasing constraint
    $\scls$ to the variables $\vec{y}$ is
    $\gls{-S-scls-restr} \defn \scls \cap (\vec{y} \times
    \vec{y})$.
% \item $\EqClassesKW$ is the set of all stack-aliasing
%     constraints.
  \item
    $\gls{ACx} \defn \set{ \eqclasses{\S} \mid \dom(\S) =
      \vec{x}}$ is the set of all stack-aliasing constraints over
    variables $\vec{x}$.
    \cmtodo{is there an $\S \in Stacks$ missing?}
\end{itemize}
%
Observe that $\EqClasses{\vec{x}}$ is finite if $\vec{x}$ is
finite---Its size is given by the $\size{\vec{x}}$-th Bell number.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> PartC/DecidingBTW-SatCapture.tex <==
Our goal in this section is to show that models with the same type
satisfy the same $\SLIDguarded$ formulas that do not contain location
terms.
%
This is perhaps surprising, as types only contain formulas from the
DUSH fragment, which is largely orthogonal to $\SLIDguarded$. For
example, $\SLIDguarded$ formulas allow guarded negation and guarded
septraction, but neither quantifiers nor unguarded magic wands,
whereas DUSHs allow limited use of guarded quantifiers and unguarded
magic wands, but neither Boolean structure nor septraction.
%

\cmtodo{I would shorten and present only the proof of the refinement theorem in detail, i.e., keep only lemmas 8.7 - 8.9 and move all remaining proofs and lemmas to the appendix.}

\paragraph*{Models with the same types satisfy the same guarded
  formulas.}

\Cref{lem:types:decompose} allows us to show the refinement theorem,
\cref{thm:types-capture-sat}, which states that guarded models with
identical types satisfy the same guarded formulas.

We need two additional properties of types to prove the refinement theorem.
%First, observe that a model satisfies all the formulas in its type.
%
%\cmtodo{CMFIXME: only used in the proof of the refinement theorem}
%\begin{lemma}\label{lem:forms-in-type-hold}
%  If $\phi \in \sidtypeof{\S,\H}$ then $\SH \sidmodels \phi$.
%\end{lemma}
%\begin{proof}
%  Since $\phi \in \sidtypeof{\S,\H}$, there exists a $\Sid$-forest
%  $\frst$ with $\fheapof{\frst}=\H$ and $\sfproj{\S}{\frst}=\H$.
%  %
%  By \cref{lem:sf-projection-sound},
%  $\SHpair{\S}{\fheapof{\frst}}\sidmodels \sfproj{\S}{\frst}$.
%  %
%  Substituting the previous identities, we obtain
%  $\SH \sidmodels \phi$.
%\end{proof}

Second, if two models have the same type, then the first model is
guarded iff the second model is guarded.

\cmtodo{CMFIXME: only used in the proof of the refinement theorem}
\begin{lemma}\label{lem:same-type-both-guarded}
  Let $\S\in\SS$, $\H_1,\H_2\in\HH$ and assume that (1)
  $\SHi{1}\in\Mpos{\Sid}$ and (2)
  $\sidtypeof{\S,\H_1}=\sidtypeof{\S,\H_2}$.
  %
  Then $\SHi{2}\in\Mpos{\Sid}$.
\end{lemma}
\begin{proof}
  By \cref{def:positive-model}, $\SHi{1} \sidmodels
  \pred_1(\vec{x_1})\sep\cdots\sep\pred_k(\vec{x_k})$ for
  some choice of predicate calls.
  %
  For
  $\psi\defn\IteratedStar_{1\leq i \leq k}(\emp \mw
  \pred_i(\vec{x_i}))$, it then holds that
  $\psi \in \sidtypeof{\S,\H_1}=\sidtypeof{\S,\H_2}$.
  %
  \Cref{lem:forms-in-type-hold} yields that $\SHi{2} \sidmodels \psi$
  holds.
  %
  Therefore,
  $\SHi{2} \sidmodels
  \pred_1(\vec{x_1})\sep\cdots\sep\pred_k(\vec{x_k})$, implying
  $\SHi{2}\in\Mpos{\Sid}$.
\end{proof}


\cmtodo{CMFIXME: central theorem!; not used in this form outside of the section}
\begin{theorem}[Refinement
  theorem]\label{thm:types-capture-sat}\index{refinement theorem!of
    Phi-types@of $\Sid$-types} Let $\S$ be a stack and $\H_1,\H_2$ be
  heaps. Let $\phi \in \SLIDguarded$ with $\locs{\phi}=\emptyset$ and
  let $\Sid\in\IDbtw$ be \ptrclosed{} w.r.t.~$\phi$.
  %
  Moreover, assume $\sidtypeof{\S,\H_1} = \sidtypeof{\S,\H_2}$.
  %
  Then $\SHi{1} \sidmodels \phi$ iff $\SHi{2} \sidmodels \phi$.
\end{theorem}
\begin{proof}
  If $\SHi{1},\SHi{2}\notin \Mpos{\Sid}$, then $\sidtypeof{\S,\H_1}$
  is undefined and neither model satisfies $\phi$ by
  \cref{lem:pos-formula-pos-model}.

  Assume $\SHi{1},\SHi{2}\in \Mpos{\Sid}$
  %
  We proceed by induction on the structure of $\phi$. We only show
  that if $\SHi{1} \sidmodels \phi$ then $\SHi{2} \sidmodels \phi$, as
  the proof of the other direction is completely analogous.
  %
  \begin{description}
  \item[Case $\phi=\emp$.] Assume that $\SHi{1} \sidmodels \phi$. By
    the semantics of $\emp$, $\H_1 = \emptyset$. Let
    $\frst = \emptyset$ be the empty forest. Then
    $\frst \in \sidfrstsof{\H_1}$ and thus
    $\emp=\sfproj{\S}{\frst} \in \sidtypeof{\S,\H_1} =
    \sidtypeof{\S,\H_2}$. Thus $\SHi{2} \sidmodels \emp$ by
    \cref{lem:forms-in-type-hold}.
    %
  \item[Cases $\phi = \sleq{x}{y}$, $\phi=\slneq{x}{y}$.] Trivial,
    because the models have the same stack.
    %
  \item[Case $\phi = \pto{x}{\tuple{y_1,\ldots,y_k}}$.] Assume that
    $\SHi{1} \sidmodels \phi$. By assumption, $\Sid$ is \ptrclosed{},
    so
    $\SHi{1} \sidmodels \ptrpred_{k}(x,y_1,\ldots,y_k)$.
    %
    Let
    \begin{align*}
    \ftree = \{ \S(x) \mapsto \langle \emptyset,&
        \ptrpred_{k}(\S(x),\S(y_1),\ldots,\S(y_k))\\&\; \Rule
        \pto{\S(x)}{\tuple{\S(y_1),\ldots,\S(y_k)}} \rangle\}
    \end{align*}
be a tree and
    $\frst = \set{\ftree}$.
    %
    Observe that $\frst \in \sidfrstsof{\H_1}$ and
    %
    \begin{align*}
\ptrpred_{k}(x,y_1,\ldots,y_k)=\sfproj{\S}{\frst} &\in
    \sidtypeof{\S,\H_1}\\& = \sidtypeof{\S,\H_2}.
    \end{align*}
    %
    Thus
    $\SHi{2} \sidmodels \ptrpred_{k}(x,y_1,\ldots,y_k)$ by
    \cref{lem:forms-in-type-hold}.
    %
    By definition of $\ptrpred_k$, we conclude that
    $\SHi{2} \sidmodels \pto{x}{\tuple{y_1,\ldots,y_k}}$.
    %
  \item[Case $\phi = \pred(z_1,\ldots,z_k)$.] Assume that
    $\SHi{1} \sidmodels \phi$.
    %
    By \cref{lem:model-of-pred-to-tree}, there exists a $\Sid$-tree
    $\ftree$ with $\trootpred{\ftree}=\pred(\S(z_1),\ldots,\S(z_k))$,
    $\tallholepreds{\ftree}=\emptyset$, and
    $\fheapof{\set{\ftree}}=\H_1$.
    %
    Let
    \[\psi \defn
      \pinst{\pred(\S(z_1),\ldots,\S(z_k))}{\dom(\stkchc)}{\img(\stkchc)}.\]
    %
    Note that $\psi = \sfproj{\S}{\set{\ftree}}$ by definition of
    stack--forest projection and thus
    $\psi \in \sidtypeof{\S,\H_1} = \sidtypeof{\S,\H_2}$. By
    \cref{lem:forms-in-type-hold}, $\SHi{2} \sidmodels \psi$.
    %
    Observe that while $\psi \neq \pred(\vec{z})$ is possible, we have
    by definition of $\stkchc$ that the parameters of the predicate
    call in $\psi$ evaluate to the same locations as the parameters
    $\vec{z}$.  Thus, $\SHi{2}\sidmodels\pred(z_1,\ldots,z_k)$.
    %
  \item[Case $\phi = \phi_1 \wedge \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$. We then have that $\SHi{1} \sidmodels \phi_1$
    and $\SHi{1} \sidmodels \phi_2$. By the induction hypotheses,
    $\SHi{2} \sidmodels \phi_1$ and $\SHi{2} \sidmodels \phi_2$ and thus
    $\SHi{2} \sidmodels \phi_1 \wedge \phi_2$.
    %
  \item[Case $\phi = \phi_1 \vee \phi_2$.] and assume that
    $\SHi{1} \sidmodels \phi$. We then have that
    $\SHi{1} \sidmodels \phi_1$ or $\SHi{1} \sidmodels \phi_2$. Assume
    w.l.o.g.~that $\SHi{1} \sidmodels \phi_1$. By induction, $\SHi{2} \sidmodels \phi_1$ and thus
    $\SHi{2} \sidmodels \phi_1 \vee \phi_2$.
    %
  \item[Case $\phi = \phi_1 \wedge\neg \phi_2$.] Assume that
    $\SHi{1} \sidmodels \phi$. We then have that
    $\SHi{1} \sidmodels \phi_1$ and $\SHi{2} \not\sidmodels
    \phi_2$. By the induction hypotheses, $\SHi{2} \sidmodels \phi_1$
    $\SHi{2} \not\sidmodels \phi_2$ and thus
    $\SHi{2} \sidmodels \phi_1 \wedge \neg \phi_2$.
    %
  \item[Case $\phi = \phi_1 \sep \phi_2$.] and assume that
    $\SHi{1} \sidmodels \phi$.
    %
    By the semantics of $\sep$, there exist $\Hoo$ and $\Hot$ such
    that $\SHpair{\S}{\H_{1,i}} \sidmodels \phi_i$ for
    $1 \leq i \leq 2$.
    %
    Let $\typ_i \defn \sidtypeof{\S,\H_{1,i}}$ and apply
    \cref{lem:types:decompose} to $\SHi{2}$, $\typ_1$ and $\typ_2$ to
    obtain models $\Hto$ and $\Htt$ with $\H_2=\Hto\stdunion\Htt$,
    $\sidtypeof{\S,\Hto}=\typ_1$, and $\sidtypeof{\S,\Htt}=\typ_2$.

    Note that $\SHpair{\S}{\H_{1,i}} \in \Mpos{\Sid}$ by
    \cref{lem:pos-formula-pos-model}. \Cref{lem:same-type-both-guarded},
    applied once to $\Hoo$ and $\Hto$, once to $\Hot$ and $\Htt$, then
    yields that also $\SHpair{\S}{\H_{2,i}} \in \Mpos{\Sid}$.

    We can therefore apply the induction hypothesis for both $\Hoo$,
    $\Hot$, $\phi_1$ and $\Hto$, $\Htt$, $\phi_2$ to obtain that for
    $1 \leq i \leq 2$, $\SHpair{\S}{\H_{2,i}} \sidmodels \phi_i$.
    %
    As $\Hto \stdunion \Htt = \H_2$, it follows by the semantics
    of $\sep$ that $\SHi{2} \sidmodels \phi$.
    %
  \item[Case $\phi = \phi_0 \wedge (\phi_1 \protect\sept \phi_2)$.]
    Assume that $\SHi{1} \sidmodels \phi$.
    %
    Then there exists a heap $\H_0$ with $\SHi{0} \sidmodels \phi_1$
    and $\SHpair{\S}{\H_1 \stdunion \H_0} \sidmodels \phi_2$.

    Since $\SHi{1}$ and $\SHi{2}$ have the same type,
    $\valloc{\S,\H_1}=\valloc{\S,\H_2}$ holds.  We can therefore
    assume w.l.o.g.~that $\H_2 \stdunion \H_0$ is defined---if this
    is not the case, simply replace $\H_0$ with a heap $\H_0'$ such
    that $\SHi{0} \Iso \SHpair{\S}{\H_0'}$ and both
    $\H_1 \stdunion \H_0'$ and $\H_2 \stdunion \H_0'$ are defined.
    %
    By \cref{lem:sid:iso-models-same-formulas}, $\H_1\stdunion
    \H_0'\sidmodels \phi$.

    By assumption $\SHi{1}\in\Mpos{\Sid}$ and by
    \cref{lem:pos-formula-pos-model}, $\SHi{0}\in\Mpos{\Sid}$. Thus, $\SHpair{\S}{\H_1\stdunion\H_0}\in\Mpos{\Sid}$.
    %
    Our assumptions and \cref{lem:types:homo:compose} thus yield
    %
    \begin{align*}
\sidtypeof{\S,\H_1\stdunion\H_0} =& \sidtypeof{\S,\H_1} \Compose
    \sidtypeof{\S,\H_0}\\ =& \sidtypeof{\S,\H_2} \Compose
    \sidtypeof{\S,\H_0}\\ =& \sidtypeof{\S,\H_2\stdunion\H_0}.
    \end{align*}

    We apply the induction hypothesis for $\phi_0$ and $\H_1$ and
    $\H_2$ to obtain $\SHi{2} \sidmodels \phi_0$
    %
    Furthermore, we apply the induction hypotheses for formula
    $\phi_2$ and models $\SHpair{\S}{\H_1\stdunion\H_0}$ and
    $\SHpair{\S}{\H_2\stdunion\H_0}$ to obtain
    $\SHpair{\S}{\H_2\stdunion\H_0} \sidmodels \phi_2$.
    %
    By the semantics of $\sept$ and $\wedge$, we get
    $\SHi{2}\sidmodels \phi_0 \wedge (\phi_1 \sept \phi_2)$.
    %
  \item[Case $\phi = \phi_0 \wedge (\phi_1 \mw \phi_2)$.]x
    %
    Analogous to
    the case for guarded septraction, except that we must consider
    \emph{arbitrary} models $\H_0$ with $\SHi{0} \sidmodels \phi_1$
    and $\SHpair{\S}{\H_1 \stdunion \H_0} \sidmodels
    \phi_2$. \Cref{lem:sid:iso-models-same-formulas,lem:types:homo:compose},
    and the induction hypotheses can then be applied just like in the
    case for septraction.
    %
    \qedhere
  \end{description}
\end{proof}

Note that it is crucial to consider only guarded quantifier-free formulas in
\cref{thm:types-capture-sat}.

\cmtodo{CMFIXME keep}
\begin{example}
  Recall $\SidLs$ from \cref{ex:sids}. Moreover, let $\SHi{k}$,
  $k \in \N$, be a list of length $k$ from $x_1$ to $x_2$. It then
  holds for all $i,j\geq 2$ that $\sidtypeof{\S,\H_i} =
  \sidtypeof{\S,\H_j}$. However,
  \begin{align*}
    \SHi{2} \not\sidmodels \SHEX{\tuple{y_1,y_2}}
    \lseg(x_1,y_1)\sep\lseg(y_1,y_2)\sep\lseg(y_2,x_2),
  \end{align*}
  whereas
  \begin{align*}
  \SHi{j} \sidmodels \SHEX{\tuple{y_1,y_2}}
  \lseg(x_1,y_1)\sep\lseg(y_1,y_2)\sep\lseg(y_2,x_2)
  \end{align*}
  for all $j \geq 3$.
\end{example}

%\Cref{thm:types-capture-sat} immediately implies that if the type of a
%guarded model $\SH$ is among the types of $\phi$, then $\SH$ is a
%model of $\phi$.
%%
%\cmtodo{CMFIXME: central for correctness! THIS IS NEEDED LATER IN THIS FORM!!!}
%\begin{corollary}\label{cor:phi-typ-satisfies-phi}
%  Let $\phi \in \SLIDguarded$ and let $\SH \in \Mpos{\Sid}$ be a guarded
%  model such that $\sidtypeof{\S,\H} \in \phitypes{\S}{\phi}$. Then
%  $\SH \sidmodels \phi$.
%\end{corollary}
%\begin{proof}
%  Because $\sidtypeof{\S,\H} \in \phitypes{\S}{\phi}$, there exists,
%  by definition of $\phitypes{\S}{\phi}$, a heap $\H'$ such that
%  $\SHprime \sidmodels \phi$ and
%  $\sidtypeof{\S,\H'} = \sidtypeof{\S,\H}$. Because
%  $\SH \in \Mpos{\Sid}$ by assumption, \cref{thm:types-capture-sat}
%  then implies that $\SH \sidmodels \phi$.
%\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> PartC/DummyGls.tex <==
\chapter*{Dummy Chapter to Avoid Undefined References}
\label{ch:ssl}

\TODO{Some dummy definitions to have no undefined references.}

\begin{definition}[Abstraction of $\SSL$
  formulas]
  \label{def:sl:abstraction}
\end{definition}

\TODO{Make sure all relevant glossary entries are defined by using
  some defined earlier.}

\gls{ls}, \gls{tree}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> PartC/Equivalences.tex <==
\chapter{Reasoning about Systems of Inductive Definitions: A Broader Perspective}\label{ch:equivalences}

\TODO{List of used notation}
\begin{itemize}
\item $\SLID$
\item $\idfun$\index{id@$\idfun$} for identity
\item lambda notation
\item Write $\modelsofsid{\Sid}$\index{models@$\modelsofsidKW$} for
  the set of all models $\SH$ such that there exists a predicate call
  $\pred(\vec{x})$ such that $\SH \sidmodels \pred(\vec{x})$.
\item $\S'$ is the $\renfun$-instantiation of $\S$, written
  $\S'=\renfuninst{\renfun}{\S}$\index{inst@$\renfuninstKW$}, if\dots
\item Notation $\S \setminus \vec{x}$ for the stack obtained by
  removing $\vec{x}$ from the domain.
\end{itemize}
\TODO{End list of used notation}

My main focus in this part of the thesis has been on the satisfiability and
entailment problems for a certain sub-class of systems of inductive
definitions, $\IDbtw$.

To solve these problems, we developed (1) a compositional abstraction that
refined the satisfiability relation and (2)
a fixed-point algorithm for computing the abstractions of the models
of inductive predicates.

Can we generalize this approach from satisfiability and entailment to
other properties of symbolic heaps?
%
In this final technical chapter of the thesis, I will show that we can.
%
This chapter is loosely based on our paper~\cite{jansen2017unified},
but I will forego the introduction of \emph{heap automata}\index{heap automaton} and \emph{robustness properties}\index{robustness property}.

\TODO{Continue here.}

I would instead advise thinking about \emph{compositional} properties
of symbolic heaps (and, by extension, systems of inductive
definitions).

Recall that a systems of inductive definitions are built from
points-to assertions, (dis)equalities, and predicate calls
$\pred(\vec{x})$ using separating conjunctions $\sep$ and existential
quantifiers $\exists$.

Write $\MM$ for the set of all stack--heap models.

A set $\Prop \subseteq \MM$ is a \emph{property}\index{property}.

A set $\MM_0\subseteq \MM$ is a \emph{class}\index{class!of models} of models iff it is
closed under isomorphism.

\begin{definition}[Strong incompatibility]
  Two heaps $\H_1,\H_2$ are \emph{strongly incompatible} w.r.t.~$\S$,
  written $\StrongSIncomp{\H_1}{\H_2}$, if for all $\H_2'$ with
  $\SHi{2}\Iso\SHpair{\S}{\H_2'}$, it holds that
  $\H_1 \stdunion \H_2' = \bot$. Equivalently, $\H_1$ and $\H_2$ are
  strongly incompatible w.r.t.~$\S$ if there exists a variable
  $x \in \dom(\S)$ such that $\S(x) \in \dom(\H_1)\cap\dom(\H_2)$.
\end{definition}


\begin{definition}[Compositional abstraction]\label{def:comp-abst}\index{compositional abstraction}
  Let $\MM_0$ be a class of models.
  %
  A tuple
  %
  \[\Abst = \AbstTuple{\AbstSupp}\]
  %
  is a \emph{compositional abstraction} of $\MM_0$ iff all of the
  following conditions hold.
  \begin{enumerate}
  \item $\AbstFunKW\colon\MM_0 \to \AbstSupp$ such that
    $\AbstFun{\AbstSupp}{\S,\H}$ is computable if $\size{\H}\leq 1$.
    %
  \item The functions
    $\AbstComp_\Abst\colon \AbstSupp\times\AbstSupp\pfun\AbstSupp$,
    $\AbstInstKW_\Abst\colon 2^\Var \times 2^\Var \times
    \AbstSupp\pfun\AbstSupp$, and
    $\AbstForgetKW_\Abst\colon (\Var\pfun\Var) \times
    \AbstSupp\pfun\AbstSupp$ are computable.
    %
  \item\label{case:comp-abst:undef} For all $\S$, $\H_1$, $\H_2$ with
    $\SHi{1},\SHi{2}\in\MM_0$, it holds that if
    $\StrongSIncomp{\H_1}{\H_2}$ then
    $\AbstFun{\AbstSupp}{\S,\H_1} \AbstComp_{\AbstSupp}
    \AbstFun{\AbstSupp}{\S,\H_2} = \bot$.\todo{It's enough to have an
      implication and not an iff here, right? Otherwise we don't get
      an iff in \cref{lem:prod-abst-is-abst}, but do we even need that?}
    %
  \item For all $\S$, $\H_1$, $\H_2$, if $\SHi{1},\SHi{2}\in\MM_0$ and
    $\H_1\stdunion\H_2\neq\bot$ then
    $\AbstFun{\AbstSupp}{\S, \H_1 \stdunion \H_2} =
    \AbstFun{\AbstSupp}{\S,\H_1} \AbstComp_\AbstSupp
    \AbstFun{\AbstSupp}{\S,\H_2}$.
  %
\item For all $\S,\S'$, $\H$, and $\renfun\colon\dom(\S)\to\dom(\S')$,
  if $\S'=\renfuninst{\renfun}{\S}$ then
%
  $\AbstInst{\AbstSupp}{\renfun}{\AbstFun{\AbstSupp}{\S,\H}}=\AbstFun{\AbstSupp}{\S',\H}$.
%
\item For all $\S,\S'$, $\H$ and $\vec{y}\subseteq\Var$
  %
  \TODO{Do we need a condition such as $\S(\vec{y})\subseteq\dom(\H)$
    or $\S(\vec{y})\subseteq\locs{\H}$? (This condition always holds
    in the entailment abstraction.)}
  %such that $y \in \dom(\S)$,
  %$\S(y)\in\dom(\H)$,\todo{This may be too strong in general? Can
  %  easily use $\S(y)\in\locs{\H}$. Is that sufficiently general?}
  %  and
  %
  such that $\S' = \S \setminus \vec{y}$, it holds that
  $\AbstFun{\S',\H} =
  \AbstForget{\AbstSupp}{\vec{y}}{\AbstFun{\AbstSupp}{\S,\H}}$.
\end{enumerate}
If $\Abst$ satisfies all requirements
except~\ref*{case:comp-abst:undef}, we call $\Abst$ \emph{weakly
  compositional}\index{weakly
  compositional}\index{compositional!weakly}.
%
  We call $\AbstSupp$ the \emph{support}\index{support!of
    compositional abstraction} of $\Abst$. The
  \emph{size}\index{size!of compositional abstraction},
  $\size{\Abst}$, is given by $\size{\AbstSupp}$.
\end{definition}

Note that we fix the stack in the composition operation.

\begin{example}
  \begin{enumerate}
  \item \emph{Trivial abstraction.} We can obtain a compositional (but
    not very interesting) abstraction by abstracting every model with
    itself.  Formally, for
    \begin{itemize}
    \item composition
      $\AbstComp_\MM \defn \lambda \SHi{1} \lambda \SHi{2}\ldotp
      \SHpair{\S}{\H_1\stdunion\H_2}$,
    \item $\AbstInstKW_\MM \defn \lambda\renfun\lambda\SH\ldotp
      \SHpair{\renfuninst{\renfun}{\S}}{\H}$, and
    \item $\AbstForgetKW_\MM \defn \lambda \vec{x}\lambda \SH \ldotp
      \SHpair{\S \setminus \vec{x}}{\H}$,
    \end{itemize}
    %
    it holds that
    $\Abst_{trivial} \defn \tuple{\MM, \idfun, \AbstComp_\MM,
      \AbstInstKW_\MM, \AbstForgetKW,\MM}$ is a compositional
    abstraction.
  \item \emph{Nonemptiness abstraction.} We can obtain a \emph{weakly}
    compositional abstraction as follows.
    \begin{align*}
      \Abst_{nonempty} \defn \langle & \set{0,1},\\
      %
      & \lambda \SH\ldotp \min(\size{\H}, 1), \\
      %
      & \lambda
        \rangle
    \end{align*}
    \TODO{To be continued.}
  \item Allocation abstraction.
  \item Tracking abstraction
  \item Reachability abstraction.
  \end{enumerate}
\end{example}

\begin{definition}[Product abstraction]
  For $1 \leq i \leq 2$, let \[\Abst_i \defn \AbstTuple{\AbstSupp_i}\] be
  (weakly) compositional abstractions.
  %
  The \emph{product abstraction}\index{product abstraction}
  $\Abst_1\CompProd\Abst_2$ is given by
  \begin{align*}
    \langle & \AbstSupp_1 \times \AbstSupp_2,\\
    %
    & \lambda \SH \ldotp \tuple{\AbstFun{\AbstSupp_1}{\S,\H}, \AbstFun{\AbstSupp_2}{\S,\H}}, \\
    %
    &\lambda \tuple{\abstcls_{1,1},\abstcls_{2,1}} \lambda
    \tuple{\abstcls_{1,2},\abstcls_{2,2}}\ldotp \tuple{ \abstcls_{1,1}
    \AbstComp_{\AbstSupp_1} \abstcls_{1,2}, \abstcls_{2,1}
              \AbstComp_{\AbstSupp_1} \abstcls_{2,2} }, \\
              %
    & \lambda \renfun \lambda \tuple{\abstcls_1,\abstcls_2} \ldotp
      \tuple{ \AbstInst{\AbstSupp_1}{\renfun}{\abstcls_2},
      \AbstInst{\AbstSupp_1}{\renfun}{\abstcls_2} }, \\
    %
    & \lambda \vec{y} \lambda \tuple{\abstcls_1,\abstcls_2} \ldotp
      \tuple{
      \AbstForget{\AbstSupp_1}{\vec{y}}{\abstcls_1},
      \AbstForget{\AbstSupp_2}{\vec{y}}{\abstcls_2}
      }
    %
     \rangle
  \end{align*}
  Here, I assume that a tuple with an undefined component is itself
  undefined, i.e.
  $\tuple{\bot,\abstcls}=\tuple{\abstcls,\bot}=\tuple{\bot,\bot}=\bot$.
\end{definition}

\begin{lemma}\label{lem:prod-abst-is-abst}
  A product of two or more weakly compositional abstractions
  $\mathcal{B} \defn \Abst_1\CompProd\cdots\CompProd\Abst_k$ is
  compositional if at least one $\Abst_i$ is a compositional
  abstraction.
\end{lemma}
\begin{proof}
  Let
  $\mathbf{B} := \AbstSupp_1 \CompProd \cdots \CompProd \AbstSupp_k$.
  $\AbstFun{\mathbf{B}}{\S,\H_1} \AbstComp_{\mathbf{B}}
  \AbstFun{\mathbf{B}}{\S,\H_2}$ is undefined iff there exists an $i$
  such that
  $\AbstFun{\AbstSupp_i}{\S,\H_1} \AbstComp_{\mathbf{B}}
  \AbstFun{\AbstSupp_i}{\S,\H_2}$ is undefined. If $\Abst_i$ is
  compositional, this holds at least for all $\H_1,\H_2$ with
  $\StrongSIncomp{\H_1}{\H_2}$, guaranteeing that $\mathcal{B}$ is
  compositional.
\end{proof}

\begin{lemma}
  If $\Abst$ is a compositional abstraction,
  $\AbstFun{\AbstSupp}{\S,\H}$ is computable for all $\SH$.
\end{lemma}
\begin{proof}
  By introducing sufficiently many existentials, every model can be
  decomposed into points-to assertions (and (dis)equalities).
\end{proof}

\begin{definition}
  Let $\MM_0$ be a class of models and $\Prop\subseteq\MM$ a
  property. $\Prop$ is \emph{finitely compositional}\index{finitely
    compositional}\index{compositional!finitely} on $\MM_0$ iff there
  exists a compositional abstraction $\Abst=\AbstTuple{\AbstSupp}$,
  $\size{\AbstSupp} \leq \infty$, such that
  \begin{enumerate}
  \item for all models $\SHi{1},\SHi{2}\in\MM_0$, if
    $\AbstFun{\AbstSupp}{\S,\H_1}=\AbstFun{\AbstSupp}{\S,\H_2}$ then ($\SHi{1} \in \Prop$
    iff $\SHi{2}\in\Prop$)
  \item
  every $\abstcls \in \AbstSupp$,
  \end{enumerate}
  We say that $\Abst$ is a \emph{witness}\index{Witness} of the finite
  compositionality of $\Prop$.
\end{definition}

\begin{theorem}[Filter theorem]
If $\modelsofsid{\Sid} \subseteq \MM_0$ and $\Prop$ is finitely
compositional on $\MM_0$, we can compute a refined/filtered SID.
\end{theorem}

\begin{theorem}

\end{theorem}

We called the above theorem \emph{refinement theorem} instead of
filter theorem in \cite{jansen2017unified}. Here, we use a different
name to avoid confusion with \cref{thm:types-capture-sat}.\todo{And a
  similar theorem about SSL?}

\begin{corollary}[\cite{brotherston2014decision}]
  The satisfiability problem for $\SLID$ is decidable.
\end{corollary}


Given the undecidability of the entailment problem for symbolic
heaps~\cite{antonopoulos2014foundations}, I cannot choose something
like ``entails $\pred(\vec{x})$'' as a property in general.

\begin{infobox}{Filtering SIDs vs.~filtering inside the composition operation}
  Design space: Filter out undesirable stuff first / normalize SID via
  compositional abstraction, or use compositional product.
  %
  For example, allocation refinement or (dis)equality ALL-SAT
  refinement prior to further analysis!
\end{infobox}

\begin{infobox}{Differences to the robustness properties of~\cite{jansen2017unified}}
  Differences between this formalization and the robustness
  properties: Here I take a semantic approach, whereas robustness
  properties where syntactic. (Properties of reduced symbolic heaps
  rather than of models.)
  %
  So, for example, the unsatisfiability refinement in
  \cite{jansen2017unified} does not work in this context.
\end{infobox}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> PartC/SLID.tex <==
\section{Separation Logic with Inductive Definitions}\label{ch:seplog}
%\index{separation logic!with inductive definitions}
%\index{SLID|see{separation logic!with inductive definitions}}
\index{separation logic with inductive definitions}

In this part of the thesis, I study \emph{separation logic with
  inductive definitions} (SLID).
%
In contrast to \cref{pt:ssl}, we no longer assume that predicates for
data structures, such as $\ls$ and $\tree$, are built into the logic.
%
Instead, the user of SLID can define custom predicates by providing a
set of recursive equations called a \emph{system of inductive
  definitions} (SID).
%
Our main focus will be on (an extension of) the decidable fragment
$\SLIDbtw$~\cite{iosif2013tree}, which I introduced informally in
\cref{ch:insights} and will formalize later in the present chapter.

\paragraph*{Outline.} In this chapter, I introduce the syntax and
semantics of SLID and define the \emph{guarded fragment} $\SLIDguarded$, the
extension of $\SLIDbtw$ that is my main object of study.
%
The following three chapters center around an abstraction for
$\SLIDguarded$ formulas, \emph{$\Sid$-types}. Specifically,
\cref{ch:towards} contains an informal motivation of the abstraction,
\cref{ch:forests} introduces \emph{$\Sid$-forests} and their
\emph{projections} onto formulas, and \cref{ch:types} uses such forest
projections to define the $\Sid$-type abstraction.
%
A decision procedure for $\SLIDguarded$ based on the $\Sid$-type
abstraction follows in \cref{ch:deciding-btw}.
%
In \cref{ch:undec}, I conclude this part of the thesis by proving that
all logics that all extensions of $\SLIDguarded$ that lift one of the
\emph{guardedness} restrictions are undecidable.

\cmtodo{Only briefly remark that there is a difference}
\paragraph*{How \cref{pt:ssl} relates to
  \cite{jansen2017unified,katelaan2018harrsh,katelaan2019effective,pagel2020complete,pagel2020beyond}.}
\index{heap automaton}\index{robustness property}

We began studying abstraction-based entailment checking for SLID, in
the guise of \emph{compositional heap automata} and \emph{robustness
  properties}, in \cite{jansen2017unified}. In that paper, we provided
anecdotal evidence that our approach might lend itself to deciding
entailment in large fragments of SLID.
%
In \cite{katelaan2019effective}, we proposed the \emph{$\Sid$-profile}
abstraction, including an implementation in our \tool{Harrsh}
tool~\cite{katelaan2018harrsh}, claiming that this approach yields a
$\TwoExpTime$ decision procedure for $\SLIDbtw$.

Unfortunately, we later discovered that the approach of
\cite{katelaan2019effective} is incomplete, which led to the
development of the \emph{$\Sid$-type} abstraction introduced in
\cite{pagel2020complete}. \cref{ch:forests,ch:types,ch:deciding-btw}
are based on this article.
%
Our recent article~\cite{pagel2020beyond} contains a more accessible
introduction to the $\Sid$-type abstraction, which has informed both
\cref{ch:towards} and the presentation of
\cref{ch:forests,ch:types,ch:deciding-btw}. Further,
\cite{pagel2020beyond} contains an abridged version of the
undecidability proofs in \cref{ch:undec}.

To sum up, this part of the thesis has grown out of joint work with
Christina Jansen, Christoph Matheja, Thomas Noll and Florian
Zuleger~\cite{jansen2017unified,katelaan2018harrsh,katelaan2019effective,pagel2020complete,pagel2020beyond}.
%
Sections that are due in large part to one of my contributors contain
an explicit attribution.

\subsection{Syntax of Separation Logic with Inductive
  Definitions}\label{sec:sid:syntax}\index{syntax!of SLID@of $\SLID$}

We assume a set \gls{Preds} of \emph{predicate
  identifiers}\index{predicate identifier}. Each predicate
$\pred\in \PredsKW$ is equipped with an arity\index{arity}
$\gls{arity-pred} \in \mathbb{N}$, representing the number of
parameters to be passed to the predicate.

The grammar in \cref{fig:sid:syntax} defines three variants of
separation logic with inductive definitions:
\begin{itemize}
\item \emph{Guarded} quantifier-free separation logic,
  %
  \index{guarded separation logic}
  \index{separation logic!guarded}
  %
  formulas of the
  form $\phiGuarded$, collected in the set \gls{SLIDguarded}.
%
\item Quantifier-free separation logic,
  %
  \index{separation logic!quantifier-free}
  %
  formulas of the form $\phiQf$, collected in
  \gls{SLIDqf}.
%
\item \emph{Existentially-quantified symbolic heaps},
  \gls{SHe}.\index{symbolic heap}
%
\end{itemize}
%
\begin{figure}[t!]
  \centering
  \input{figtbl/PartC/syntax-slid.tex}
  \caption[Syntax of SL with inductive definitions]{The syntax of the
    separation-logic fragments studied in this part of the thesis:
    Guarded formulas $\phiGuarded$, collected in $\AllSLIDguarded$;
    quantifier-free formulas $\phiQf$, collected in $\AllSLIDqf$; and
    existentially-quantified symbolic heaps, $\phiSH$, collected in
    $\SymHeap$.}\label{fig:sid:syntax}
\end{figure}

In \cref{fig:sid:syntax}, $\pred \in \PredsKW$ is a predicate
identifier and $\size{\vec{u}}=\arity{\pred}$.

The first line of \cref{fig:sid:syntax} defines the atomic formulas,
$\tau$, common to all three SL variants. As with the first-order
separation logic $\SLbase$ from \cref{ch:sl-intro}, $\gls{emp}$ is the
\emph{empty heap}, $x \mathbin{\gls{--pto}}\vec{y}$ asserts that $x$
\emph{points to} the locations captured by $\vec{y}$,
$x\mathbin{\gls{--rel-sleq}}y$ asserts the equality between variables
$x$ and $y$, and $x\mathbin{\gls{--rel-slneq}}y$ asserts the
disequality of $x$ and $y$.\index{equality}\index{disequality}
  %
Guarded formulas, $\phiGuarded$, are built from atomic formulas using
the separating conjunction $\sep$, conjunction $\wedge$, disjunction
$\vee$, \emph{guarded negation}
\index{guarded negation!in SLID@in $\SLID$}\index{negation!guarded}
$\phiGuarded \wedge \neg \phiGuarded$, \emph{guarded
  septraction}\index{septraction}\index{guarded septraction}
$\phiGuarded \wedge (\phiGuarded \gls{--slwand-sept} \phiGuarded)$, and
\emph{guarded magic wands}\index{guarded magic wand}
$\phiGuarded \wedge (\phiGuarded \gls{--slwand-mw} \phiGuarded)$.

In (not necessarily guarded) quantifier-free formulas, $\phiQf$,
negation and magic wands may occur unguarded. Moreover, we omit the
septraction operator in $\phiQf$, as it is definable as
$\fa \sept \fb \defn \neg (\fa \mw \neg \fb)$.

Finally, $\phiSH$ formulas are existentially-quantified symbolic
heaps, consisting of points-to assertions, predicate calls, and a
\emph{pure constraint}\index{pure constraint}, i.e., a conjunction of
(dis-)equalities.
%
In the literature, the pure constraint, $\gls{-P-Pi}$, is usually
defined with the classical conjunction
$\wedge$~\cite{berdine2004decidable}.
%
Just like in \cref{pt:intro,pt:ssl} of the thesis, we instead use the
separating conjunction $\sep$ to express the pure constraint, because
our semantics of (dis-)equalities, defined in
\cref{sec:sid:semantics}, forces the heap to be empty in models of
(dis-)equalities.
\cmtodo{Perhaps briefly mention that conjunction or sep. conjunction with pure formulas is equivalent (Reynolds)}

As in \cref{pt:ssl},
$\gls{--sl-sep-iterated}\set{\psi_1,\ldots,\psi_k}$ is the formula
$\psi_1 \sep \cdots \sep \psi_k$.

\cmtodo{ls(y,z) has not been defined or explained yet}
\begin{example}[Syntax of SLID]
  Assume the predicate $\lseg(x_1,x_2)$ is interpreted by the set of
  all nonempty list segments from $x_1$ to $x_2$.
  \begin{enumerate}
  \item The symbolic heap $\SHEX{y} \lseg(x,y) \sep \lseg(z,y) \sep
    \lseg(y,\nil) \in \SymHeap$ states that the heap consists of two overlaid
    null-terminated lists, one with head $x$, the other with head $z$.
    %
  \item The guarded formula
    $\lseg(x,y) \wedge \neg \pto{x}{y} \in \SLIDguarded$ states that
    the heap consists of a list of length at least two.
    %
  \item The guarded formula
    $\lseg(x,y) \wedge (\ls(y,z) \sept \ls(x,x)) \in \SLIDguarded$
    states that the heap consists of a list segment from $x$ to $y$
    that can be extended to a cyclic list by adding a (nonempty) list
    from $y$ to $z$.
    %
    This formula is only satisfied by models in which $\sleq{x}{z}$
    holds.
    %
  \item The unguarded formula $\ppto{x}{\nil} \mw \slneq{x}{x} \in \SLIDqf$ states
    that in all models obtained by extending the current model with a
    pointer from $x$ to $\nil$, $x$ is different from $x$.
    %
    As it is impossible that $x$ is different from $x$, the formula is
    only satisfied by models in which there is \emph{no} way to extend
    the heap by the pointer from $x$ to $\nil$, i.e., by models in
    which $x$ is allocated.
  \end{enumerate}
\end{example}

\begin{infobox}{An atom representing $true$?\index{true!in SLID}}
  It is quite common to include an atomic formula that holds in every
  model, often denoted $true$ or
  \gls{t}~\cite{reynolds2002separation}, even in symbolic-heap
  fragments~\cite{calcagno2011compositional}.
  %
  We do \emph{not} include a spatial atom $true$ in any of
  the logics; while $true$ can of course be defined in $\AllSLIDqf$,
  it is \emph{not} definable in $\AllSLIDguarded$ because of the
  aforementioned semantics of (dis-)equalities.
  %
  This is crucial: If $true$ were definable, $\AllSLIDqf$ and
  $\AllSLIDguarded$ would be equivalent, because we could simply use
  $true$ for all guards.
\end{infobox}

\paragraph*{Locations in formulas.}\index{location!in formulas}
I make the nonstandard choice to allow locations as terms in
formulas.
%
While I make this choice purely for technical convenience, it is in
fact quite natural when considering languages such as \tool{C} that
allow accessing concrete memory addresses.
%
Given a formula $\fa$, we denote by $\gls{locs-phi}$ the set of all
locations that occur in $\fa$.
\cmtodo{At this point one might ask how this is compatible with considering models up to isomorphism. This is clarified later on, but it may still be confusing. Furthermore, I think the question why we use locations needs a bit more motivation. In the end we move from the ``standard'' derivation trees to ones with locations and then later say that we abstract locations by variables again...}

\paragraph{Inductive definitions.}\index{inductive definition}
%
Predicates are defined by a \emph{system of inductive
  definitions}\index{system of inductive definitions}
(SID). An SID is a finite set \gls{-V-Phi} of \emph{rules}
%
\index{rule!of SID}
%
of the form $\pred(\vec{x}) \Rule \fa$, where $\pred \in \PredsKW$ is
a predicate symbol, $\vec{x}$ are the
\emph{parameters}\index{parameter!of a predicate} of $\pred$, and---as
is
standard~\cite{iosif2013tree,antonopoulos2014foundations}---$\fa \in
\SymHeap$ is an existentially-quantified symbolic heap as defined in
\cref{fig:sid:syntax}.
%
We assume that all rules of the same predicate $\pred$ have the same
parameters.
%, and that these parameters are
%$\tuple{x_1,\ldots,x_{\arity{\pred}}}$.
We collect these \emph{free variables}
%
\index{free variables!of predicate}
%
of $\pred$ in the set $\gls{fvars-pred}$.
%
We collect all predicates that occur in SID $\Sid$ in the
set \gls{PredsPhi}.
%
The size of an SID $\Sid$, $\size{\Sid}$, is the sum of the sizes of
the formulas in its rules.\index{size! of SID}
%
We give a few examples of SIDs; the formal semantics of SIDs will be
defined in \cref{sec:sid:semantics}.
%
\begin{example}[SID]\label{ex:sids}
  \begin{enumerate}
      \item Let $\SidLs$ be the following SID.\index{list segment!user-defined}
    \[
      \begin{array}{lll}
        \lseg(x_1,x_2) &\Rule& \pto{x_1}{x_2}\\
        \lseg(x_1,x_2) &\Rule& \SHEX{y} \pto{x_1}{y} \sep
        \lseg(y,x_2)\\
        \ls(x_1) &\Rule& \pto{x_1}{\nil} \\
        \ls(x_1) &\Rule& \SHEX{y} \ppto{x_1}{y} \sep \ls(y)\\
      \end{array}
    \]
    %
    The predicates \gls{lsSIDlseg} and \gls{lsSID} correspond to the
    built-in $\ls$ predicate of the logic $\SSL$ from \cref{pt:ssl}
    with one and zero holes, respectively, except that they do
    \emph{not} allow empty lists.
    %
    The formulas $\lseg(x_1,\nil)$ and $\ls(x_1)$ are
    equivalent w.r.t. $\SidLs$.
    %
  \item Let $\SidOddEven$ be the following SID.
    \[
      \begin{array}{lll}
        \gls{odd}(x_1,x_2) &\Rule& \pto{x_1}{x_2}\\
        \odd(x_1,x_2) &\Rule& \SHEX{y} \ppto{x_1}{y} \sep
                              \even(y,x_2)\\
                      %
        \gls{even}(x_1,x_2) &\Rule& \SHEX{y} \ppto{x_1}{y} \sep
                               \odd(y,x_2)
      \end{array}
    \]
    $\SidOddEven$ defines all lists of odd and even length,
    respectively.
    %
  \item Let $\SidTree$ be the following SID.
    %
    \index{binary tree!SID defining}
    %
        \[
          \begin{array}{lll}
            \gls{tree}(x_1) &\Rule& \pto{x_1}{\tuple{\nil,\nil}}\\
            \tree(x_1) &\Rule& \SHEX{\tuple{l,r}} \ppto{x_1}{\tuple{l,r}} \sep \tree(l) \sep
                               \tree(r)
          \end{array}
        \]
        %
        $\SidTree$ defines the set of null-terminated binary trees,
        equivalent to trees without holes in $\SSL$.
  \end{enumerate}
\end{example}

\paragraph*{Instantiating variables.}\index{variable instantiation}
%
Let $\fa$ be a formula and let $\vec{y},\vec{z} \in
{(\Var\cup\Loc)^{*}}$ be sequences of the same length, $\vec{y}$
repetition free.
%
We denote by $\gls{-V-pinst}$ the instantiation of
$\vec{y}=\tuple{y_1,\ldots,y_k}$ by $\vec{z}=\tuple{z_1,\ldots,z_k}$
in $\fa$. Formally,
%
\[
  \begin{array}{lll}
    \pinst{y_i}{\vec{y}}{\vec{z}}& \defn & z_i, \quad 1\leq i \leq k
    \\
    %
    \pinst{a}{\vec{y}}{\vec{z}}& \defn & a, \quad \text{iff } a \notin \vec{y}\\
                               %
  \pinst{\tuple{a_1,\ldots,a_k}}{\vec{y}}{\vec{z}} & \defn &
                                                     \tuple{\pinst{a_1}{\vec{y}}{\vec{z}},\ldots,\pinst{a_k}{\vec{y}}{\vec{z}}}
    \\
    %
    \pinst{\emp}{\vec{y}}{\vec{z}} & \defn & \emp\\
    %
    \pinst{\pto{a}{\vec{b}}}{\vec{y}}{\vec{z}} & \defn &
                                         \pto{\pinst{a}{\vec{y}}{\vec{z}}}{\pinst{\vec{b}}{\vec{y}}{\vec{z}}}
    \\
    %
    \pinst{\pred(\vec{x})}{\vec{y}}{\vec{z}} &\defn&
                                             \pred(\pinst{\vec{x}}{\vec{y}}{\vec{z}})
    \\
    %
    \pinst{\neg \phi}{\vec{y}}{\vec{z}} &\defn & \neg (\pinst{\phi}{\vec{y}}{\vec{z}})\\
    %
    \pinst{\phi \times \psi}{\vec{y}}{\vec{z}} & \defn &
                                                 \pinst{\phi}{\vec{y}}{\vec{z}}
                                                 \times
                                                 \pinst{\psi}{\vec{y}}{\vec{z}},
                                                 \text{ where } \times
                                                 \in
                                                 \set{\wedge,\vee,\sep,\mw,\sept}\\
                                                 %
    \pinst{\SHEX{e} \phi}{\vec{y}}{\vec{z}}  & \defn &
                                               \SHEX{\pinst{e}{\vec{y}}{\vec{z}}} \pinst{\phi}{\vec{y}}{\vec{z}}
  \end{array}
\]
%
For example, for $\vec{y}=\tuple{x}$ and $\vec{z}=\tuple{w}$, we have
$\pinst{\ppto{x}{v}}{\vec{y}}{\vec{z}} = \pto{w}{v}$;
%
and $\pinst{\SHEX{x} \ls(z,x)}{\vec{y}}{\vec{z}} = \SHEX{w} \ls(z,w)$.

Finally, assuming we have an order on the free variables of a formula
(as we do with predicate calls, for example) we abbreviate
$\gls{-V-phiapp} \defn \pinst{\phi}{\fvs{\phi}}{\vec{z}}$.
\cmtodo{This arbitrary ordering makes me a bit nervous. Can we please properly define this once in the notation section? In particular, for substitution, we have to be careful that there is no overlapping when choosing some arbitrary ordering.}

\subsection{Semantics of Separation Logic with Inductive
  Definitions}\label{sec:sid:semantics}\index{semantics!of SLID@of $\SLID$}

As usual, we define the semantics in terms of stack--heap pairs, $\SH$
(cf.~\cref{ch:sl-intro}).
%
In this part of thesis, we only consider variants of SLID
\emph{without} data constraints. We thus define $\Val \defn \Loc$ for
this part of the thesis.
%
Given this assumption, we have $\S\colon \Var\pfun\Loc$ and
$\H\colon\Loc\pfun\Loc^{+}$, i.e., all values stored in the stack and
the heap are locations.
%
\Cref{fig:sid:semantics} defines the semantics of separation logic
formulas $\fa$ w.r.t.~a fixed SID $\Sid$.
%
To simplify the technical development in later chapters, we deviate
from the standard presentation of the semantics (see
e.g.~\cite{reynolds2002separation}) by syntactically replacing
variables by their corresponding heap locations. This is possible
because we allow locations as terms in formulas.
%
When writing $\pinst{\phi}{\dom(\S)}{\img(\S)}$, I assume that an
arbitrary but consistent order is imposed on the domain and image of
the stack, i.e., every variable $x \in \dom(\S)$ is replaced by
$\S(x)$.

As in \cref{pt:intro,pt:ssl}, the semantics of equalities and
disequalities require that the heap is empty. This ensures that $true$
is not definable in guarded formulas (e.g., as $\sleq{x}{x}$).
%
Apart from this choice, our semantics is equivalent to the standard
semantics of separation logic with inductive
definitions~\cite{iosif2013tree,antonopoulos2014foundations} on
formulas that do not contain location terms.
%
\begin{figure}[tb!]
  \centering
  \input{figtbl/PartC/slid-semantics}
  \caption[Semantics of SL with inductive
  definitions]{Semantics of separation logic with inductive
    definitions.}\label{fig:sid:semantics}
\end{figure}

Just like in \cref{pt:intro,pt:ssl}, we use a
\emph{precise}~\cite{calcagno2007local} semantics of the points-to
assertion: $\SH \sidmodels \pto{x}{\vec{y}}$ holds only in
single-pointer heaps.\index{precise}

\cmtodo{Below is an example why model is ambiguous...}
A heap is a model of a predicate call $\pred(\vec{v})$ iff it is a
model of a rule $\pred(\vec{x}) \Rule \psi$, in which the parameters
$\vec{x}$ have been replaced by the actual arguments, $\vec{v}$. Note
that this semantics of predicates corresponds to the least fixed-point
semantics as formalized e.g.~in \cite{brotherston2014decision}.

In this part of the thesis, we use the standard, ``weak'' semantics of
the separating conjunction: $\H \sidmodels \fa_1 \sep \fa_2$ iff $\H$
can be split into disjoint heaps that are models of $\fa_1$ and
$\fa_2$; and $\H \sidmodels \fa_1 \mw \fa_2$ iff extending $\H$ with a
model of $\fa_1$ always yields a model of $\fa_2$, provided the
extension is defined.
%
The semantics of the (classical) Boolean connectives and the
existential $\exists$ are standard. In particular, $\exists$
corresponds to stack extension, even though this is not explicit in
our semantics.

\begin{lemma}\label{lem:existential-variable-stack-extension}
  Let $\fa \in \SymHeap$ and $e\in\Var$. Then
  $\SH \sidmodels \SHEX{e}\fa$ if and only if there exists a location
  $v\in\Loc$ such that
  $\SHpair{\S \cup \set{e\mapsto v}}{\H} \sidmodels \fa$.
\end{lemma}
\cmtodo{Appendix}
\begin{proof}\ProofBeginsWithDisplayMath{}
  \begin{align*}
    & \SH \sidmodels \SHEX{e} \fa \\
    \text{iff } & \H \sidmodels \pinstS{(\SHEX{e}\phi)} \\
    %
    \text{iff } & \H \sidmodels \SHEX{e}(\pinstS{\phi}) \\
    %
    \text{iff } &\text{ ex.~$v\in\Loc$~s.t.~} \H \sidmodels
                  \pinst{\pinstS{\phi}}{e}{v}\\
    %
    \text{iff } &\text{ ex.~$v\in\Loc$~s.t.~} \H \sidmodels
                  \pinst{\phi}{\dom(\S) \concat \tuple{e}}{\img(\S)
                  \concat \tuple{v}}\\
    %
    \text{iff } &\text{ ex.~$v\in\Loc$~s.t.~} \\&\;\H \sidmodels
                  \pinst{\phi}{\dom(\S \cup \set{e \mapsto
                  v})}{\img(\S \cup \set{e \mapsto v})}\\
                %
    \text{iff } &\text{ ex.~$v\in\Loc$~s.t.~} \SHpair{\S
                  \cup \set{e \mapsto v}}{\H}\sidmodels\phi \qedhere
  \end{align*}
\end{proof}

\paragraph*{Satisfiability and entailment.}
%
As the semantics of an SLID formula depends on the given SID, the
satisfiability and entailment problems are parameterized by an SID.
%
Let $\fa,\fb$ be SLID formulas. We say that $\fa$ is
\emph{satisfiable}\index{satisfiability problem!of SLID} w.r.t.~SID $\Sid$ if there exists a model $\SH$
such that $\SH \sidmodels \fa$.
%
We say that $\fa$ \emph{entails}
%
\index{entailment problem!of SLID@of $\SLID$}
%
$\fb$ w.r.t.~$\Sid$, denoted $\fa
\sidmodels \fb$, iff for all models $\SH$, $\SH\sidmodels\fa$ implies
$\SH\sidmodels\fb$.

\cmtodo{Put everything about isomorphisms in one place}
\paragraph{Isomorphism.}
Formulas without location terms cannot distinguish between isomorphic
models. I restate the definition of isomorphism, simplifying it
(compared to \cref{def:slbase:iso}) based on the identity $\Val=\Loc$
that holds in this part of the thesis.

\begin{definition}[Isomorphic stack--heap pairs]\index{isomorphism!in
    SLID@in $\SLID$}
  Two stack--heap pairs $\SH$ and $\SHpair{\S'}{\H'}$ are
  \emph{isomorphic}, written $\SH \Iso \SHpair{\S'}{\H'}$, if there
  exists a bijection
  $\renfun\colon (\locs{\H} \cup \img(\S)) \to (\locs{\H'} \cup
  \img(\S'))$ such that (1) for all $x$, $\S'(x) = \renfun(\S(x))$ and
  (2)
  $\H' = \{ \renfun(l) \mapsto \renfun(\H(l)) \mid l \in \dom(\H)\}$.
\end{definition}

\begin{lemma}\label{lem:sid:iso-models-same-formulas}
  Let $\fa$ be an SLID formula with $\locs{\fa}=\emptyset$. Let $\SH$
  and $\SHpprime$ be models with $\SH \Iso \SHpprime$. Then
  $\SH \sidmodels \fa$ iff $\SHpprime \sidmodels \fa$.
\end{lemma}
\cmtodo{Appendix}
\begin{proof}[Proof sketch.]
  Let $\renfun$ be the bijection that witnesses the isomorphism
  between $\SH$ and $\SHpprime$. Then:
  %
  \begin{align*}
    & \SH \sidmodels \fa \\
    %
  \text{iff~}  & \H \sidmodels \pinstS{\fa} \\
    %
  \text{iff~}  & \H' \sidmodels
      \pinst{\pinstS{\fa}}{\dom(\renfun)}{\img(\renfun)} \tag*{\tagA}
    \\
    %
  \text{iff~}  & \H' \sidmodels \pinstSomeS{\fa}{\S'} \tag*{(because
                $\locs{\fa}=\emptyset$)} \\
              %
    \text{iff~} & \SHpprime \sidmodels \fa.
  \end{align*}
  %
  If we wanted to be fully formal, we would have to prove the step
  marked \tagA{} by a structural induction on $\fa$.
  %
  %\TODO{Prove this and mention why it is important that $\locs{\fa}=\emptyset$.}
  %\LeftToTheReader{}
\end{proof}

% \subsection{Inductive Definitions with Models of Bounded
% Treewidth}\label{sec:btw}
\subsection{SIDs with Models of Bounded Treewidth}\label{sec:btw}

As discussed in \cref{sec:insights:btw}, the entailment problem even
of the symbolic-heap fragment of SLID is undecidable in
general~\cite{antonopoulos2014foundations}.
%
To obtain a decidable logic, we restrict SIDs to the fragment
\gls{IDbtw} that was introduced by Iosif et
al.~in~\cite{iosif2013tree}.
%
$\IDbtw$ imposes restrictions on SIDs that guarantee that all models
of the predicates of the SID are of \emph{bounded
  treewidth}.\footnote{More precisely, when viewed as graphs, all
  models of the SIDs in $\IDbtw$ have bounded treewidth. For a
  definition of treewidth, see e.g.~\cite{diestel2016graph}.}
\index{treewidth}
\index{bounded treewidth}
\index{BTW|see{bounded
    treewidth}}
\index{separation logic!of bounded treewidth}

  \begin{infobox}{The relationship between $\IDbtw$ and monadic
      second-order logic over graphs of bounded
      treewidth.
      \index{monadic second-order logic}}
      \index{graphs of bounded treewidth}
    %
    The subscript $\mathsf{btw}$ is slightly misleading, as
    $\IDbtw$ does \emph{not} have the same expressive power as MSO
    over connected graphs of bounded treewidth. At the very least, one
    would need to generalize the progress property to allow ``backward
    edges'' in rules.
    %
    It is an open problem whether such an extension of $\IDbtw$ would
    capture MSO over connected graphs of bounded treewidth.
    %
  \end{infobox}


In $\IDbtw$, all SIDs have to satisfy \emph{progress},
\emph{connectivity}, and \emph{establishment}.
%
To formalize these assumptions, we introduce a couple of auxiliary
definitions for symbolic heaps $\phi$: the \emph{local allocation of
  $\phi$}, $\gls{lalloc-phi}$\index{local
  allocation}; and the \emph{local references of
  $\phi$}\index{local references},
$\gls{lref-phi}$.
%
In the following
definition, $\lfunKW \in \set{\lallocKW,\lrefKW}$.
%
\[
  \begin{array}{ll}
    \lallocKW(\pto{x}{\vec{y}}) \defn \set{x} &
                                                \lrefKW(\pto{x}{\vec{y}}) \defn \vec{y} \\
    %
    \multicolumn{2}{l}{\lfunKW(\emp) \defn \emptyset}\\
    %
    \multicolumn{2}{l}{\lfunKW(\pred(\vec{y})) \defn \emptyset}\\
    %
    \multicolumn{2}{l}{\lfunKW(\phi_1 \sep \phi_2) \defn \lfunKW(\phi_1) \cup
    \lfunKW(\phi_2)}\\
    %
    \multicolumn{2}{l}{\lfunKW(\SHEX{e}\phi) \defn \lfunKW(\phi)}\\
    %
    % \multicolumn{2}{l}{\lusedKW(\phi) \defn
    % \lallocKW(\phi)\cup\lrefKW(\phi)}\\
    %
  \end{array}
\]
\cmtodo{Have we quietly eliminated pure formulas or why are they not considered in inductive definitions?}
%
\begin{description}
\item[Progress.] 
  A predicate $\pred$ satisfies
  \emph{progress}\index{progress} iff every rule of $\pred$ contains
  exactly one points-to assertion and there is a variable
  $x\in\fvs{\pred}$ such that for all rules
  $(\pred(\vec{x}) \Rule \phi) \in \Sid$, $\lalloc{\phi} =
  \set{x}$. In this case, we define
  $\lalloc{\pred(\vec{y})} \defn \set{ \pinst{x}{\vec{x}}{\vec{y}}}$
  and call $x$ the \emph{root of the predicate}.
  \cmtodo{Overwriting the above definition is a bit confusing}
%
  \index{root!of predicate}
%
  Moreover, if the $i$-th parameter of $\pred$ is the root of $\pred$,
  then $\gls{predroot}(\pred(z_1,\ldots,z_k)) \defn z_i$.

  \item[Connectivity.] A predicate $\pred$ satisfies
  \emph{connectivity}\index{connectivity} iff for all rules of
  $\pred$, all variables that are allocated in the recursive calls of
  the rule are referenced in the rule.
%
  Formally, for all rules $(\pred \Rule \phi) \in \Sid$ and for all
  predicate calls $\pred'(\vec{y})\in\phi$, it holds that
%
  $\lalloc{\phiapp{\pred'}{\vec{y}}}
    \subseteq \lref{\phi}$.
  % \[ \lalloc{\phiapp{\pred'}{\vec{y}}}
  %   \subseteq \lref{\phi}.\]

  \item[Establishment.] A predicate $\pred$ is
  \emph{established}\index{establishment} iff all existentially
  quantified variables across all rules of $\pred$ are eventually
  allocated.
%
  Formally, for all rules $(\pred \Rule \SHEX{\vec{y}}\phi)\in\Sid$
  and for all models $\SH$, if $\SH \sidmodels \phi$ then
  $\S(\vec{y}) \subseteq \dom(\H)$.
  \cmtodo{The definition of establishment is non-standard as it does not account for unallocated free variables, e.g. $p(x,y) = \exists z . x \mapsto z \sep y = z$ would be fine. Radu's definition states that all existentially quantified variables are either allocated or ultimately equal to a free variable.The second possibility is not allowed here. One should comment on this.}
\end{description}


We collect in $\IDbtw$ all SIDs that satisfy \emph{progress},
\emph{connectivity}, and \emph{establishment}.
%
Unless stated otherwise, we assume $\Sid\in\IDbtw$ for all SIDs $\Sid$ in this \TypeOfDoc{}.
%
\begin{example}[SID Assumptions]\label{ex:btw:assumptions}
  All SIDs in \cref{ex:sids} satisfy progress, connectivity, and
  establishment and are thus elements of $\IDbtw$.
\end{example}
%

Throughout this \TypeOfDoc{}, I assume w.l.o.g.~that non-recursive
rules do not contain existential quantifiers, because in $\IDbtw$,
such existentials can always be eliminated: all
existentially-quantified variables in a non-recursive rule must be
provably equal to the root of the predicate---and thus to a parameter
of the predicate---to satisfy establishment.
%
Consequently, we can replace all occurrences of
existentially-quantified variables in non-recursive rules with the
corresponding root variable.

\paragraph*{Restricting SLID to SIDs from
  $\IDbtw$.}
%
I write \gls{SLIDguardedbtw} and \gls{SLIDqfbtw} for the restriction
of the logics $\AllSLIDguarded$ and $\AllSLIDqf$ in which only SIDs
from $\IDbtw$ may be used to interpret predicate calls.

\paragraph*{Adding predicates for points-to assertions to SIDs.} To
avoid dedicated reasoning about points-to assertions, we sometimes
(specifically, in \cref{sec:sid:dangling,ch:deciding-btw}) exploit that we can add
predicates that simulate points-to assertions to any SID. I call the
resulting SIDs \emph{\ptrclosed{}}.

\begin{definition}[Pointer-closed
  SID]\label{def:ptrclosed}\index{pointer-closed}
  An SID $\Sid$ is \emph{\ptrclosed{}} w.r.t.~$\phi$ iff it contains
  for all points-to assertions of arity $k$ that occur in $\phi$ a
  predicate \gls{ptrpred_k} defined by the rule
  $\ptrpred_k(\vec{x}) \Rule \pto{x_1}{\tuple{x_2,\ldots,x_{k+1}}}$.
\end{definition}

\subsection{Guarded Models and Dangling Pointers}\label{sec:sid:dangling}

\paragraph*{Guarded models.} Much of the development in the remainder
of this thesis exploits that guarded formulas interpreted over SIDs
from $\IDbtw$, i.e., formulas in $\SLIDguarded$, only have
\emph{guarded} models in the following sense.

\cmtodo{The term guarded models seems to be perfectly fine here :)}

\begin{definition}\label{def:positive-model}\index{guarded model}
  Let $\SH$ be a model. We call $\SH$ \emph{guarded} w.r.t.~SID
  $\Sid$ if there exist predicate calls
  $\pred_1(\vec{x_1}),\ldots,\pred_k(\vec{x_k})$, $k \geq 0$, such
  that
  $\SH \sidmodels \pred_1(\vec{x_1})\sep\cdots\sep\pred_k(\vec{x_k})$.

  We denote by $\ModelsgSid$ the set of all guarded states w.r.t. to SID $\Sid$.
\end{definition}

We write
$\gls{ModelsgSid} \defn \set{ \SH \mid \SH \text{ is guarded w.r.t.~}
  \Sid }$ for the set of all guarded models w.r.t.~SID $\Sid$.

The use of the adjective \emph{guarded} is justified by the following lemma.

\begin{lemma}\label{lem:pos-formula-pos-model}
  %
  Let $\Sid\in\IDbtw$ be a \ptrclosed{} SID.
  %
  Let $\phi \in \SLIDguarded$ and let $\SH$ be a model with $\SH
  \sidmodels \phi$.
  %
  Then $\SH \in \Mpos{\Sid}$.
\end{lemma}
\begin{proof}
\cmtodo{Move to appendix; again, the assumption that we consider no pure constraits seems to be missing somewhere}
  By induction on $\phi$.
  \begin{description}
  \item[Case $\phi=\emp$.] Trivial, $\SH$ satisfies the separating
    conjunction of $k=0$ predicate calls.
    %
  \item[Case $\phi=\pto{x}{\vec{y}}$.] Because $\Sid$ is \ptrclosed{},
    there exists a predicate that $\SH$ satisfies.
    %
  \item[Case $\phi=\pred(\vec{x})$.] Trivial.
    %
  \item[Case $\phi= \phi_1\sep\phi_2$.] Split $\H$ into $\H_1\stdunion\H_2$
    such that $\SHi{1}\sidmodels\phi_1$ and $\SHi{2}\sidmodels\phi_2$,
    which is possible by the semantics of $\sep$.
    %
    By the induction hypotheses, there exist %$predicate calls
    $\pred_{1,1}(\vec{x_1}),\ldots,\pred_{1,m}(\vec{x_m})$ and
    $\pred_{2,1}(\vec{y_1}),\ldots,\pred_{2,n}(\vec{y_n})$ with
    %
    \begin{align*}
      & \SHi{1}\sidmodels\IteratedStar_{1\leq i \leq
      m}\pred_{1,i}(\vec{x_i}) \text{ and}\\
    & \SHi{2}\sidmodels\IteratedStar_{1\leq j \leq
      m}\pred_{2,j}(\vec{y_j}).
    \end{align*}
    %
    As $\H=\H_1\stdunion\H_2$, we obtain
    \[\SH \sidmodels \IteratedStar_{1\leq i \leq
        m}\pred_{1,i}(\vec{x_i}) \sep \IteratedStar_{1\leq j \leq
        m}\pred_{2,j}(\vec{y_j}).\] Thus, $\SH$ is guarded.
  \item[Case $\phi = \phi_1\wedge\phi_2$.]
    %, where $\phi_2$ is either a
    %guarded formula or of the form $\neg \psi$, $\psi_1\sept\psi_2$,
    %or $\psi_1\mw\psi_2$.
    %In all these cases, $\SH \sidmodels \phi_1$,
    In this case, in particular $\SH \sidmodels \phi_1$, so the claim
    follows immediately from the induction hypothesis for $\phi_1$.
    %
  \item[Case $\phi = \phi_1 \vee \phi_2$.] Assume w.l.o.g.~that
    $\SH \sidmodels \phi_1$. The claim follows immediately from the
    induction hypothesis for $\phi_1$. \qedhere
  \end{description}
\end{proof}

\paragraph*{Dangling pointers in $\SLIDbtw$.}
\index{dangling pointers!in SLIDbtw@in $\SLIDbtw$}

If a predicate $\pred$ satisfies establishment, and $\SH \sidmodels
\pred(\vec{y})$, then only the locations $\S(\vec{y})$ can be dangling
in $\SH$.

% In models of predicate calls of predicates that satisfy establishment,
% only the parameters of predicates can be dangling pointers.
%
Recall from \cref{sec:sl-intro:other} that we denote the dangling
locations of the heap $\H$ by
$\danglinglocs{\H} \defn \set{l \in \bigcup\img(\H) \mid l \notin
  \dom(\H)}$.

\begin{lemma}\label{lem:btw:pred-non-dangling-locs}
  Let $\Sid\in\IDbtw$. If $\H \sidmodels \pred(\vec{l})$ then
  $\danglinglocs{\H} \subseteq \vec{l}$.
\end{lemma}
\begin{proof}
  A simple consequence of establishment.
\end{proof}

\begin{lemma}\label{lem:btw:pred-non-dangling}
  Let $\Sid\in\IDbtw$. If $\SH \sidmodels \pred(\vec{z})$ then
  $\danglinglocs{\H} \subseteq \S(\vec{z})$.
\end{lemma}
\begin{proof}
  Follows from the semantics and
  \cref{lem:btw:pred-non-dangling-locs}.
\end{proof}

This
property extends to arbitrary $\SLIDguarded$ formulas over $\IDbtw$ SIDs and
hence to guarded models.

\begin{lemma}\label{lem:btw:pos-non-dangling}
  Let $\Sid\in\IDbtw$ and $\SH \in \Mpos{\Sid}$. Then $\danglinglocs{\H} \subseteq \img(\S)$.
\end{lemma}
\begin{proof}
  By \cref{lem:pos-formula-pos-model}, there exist predicate calls
  $\pred_1(\vec{x_1}),\ldots,\pred_k(\vec{x_k})$ such that $\SH
  \sidmodels \IteratedStar_{1\leq i \leq k}\pred_i(\vec{x_i})$.
  %
  By the semantics of $\sep$, there thus exist $\H_1,\ldots\H_k$ with
  $\H = \H_1 \stdunion \cdots \H_k$ and
  $\SHi{i}\sidmodels\pred_i(\vec{x_i})$.
  %
  \cmtodo{It seems we sometimes write $\H \cup \H'$ and sometimes $\H \stdunion \H'$; the latter is not really defined?}
  %
  \Cref{lem:btw:pred-non-dangling} yields $\danglinglocs{\H_i}
  \subseteq \S(\vec{x_i})$ for all $1 \leq i \leq k$.
  %
  It follows that
  %
  \begin{align*}
\danglinglocs{\H}& =\danglinglocs{\H_1}\cup\cdots\danglinglocs{\H_k}\\&\subseteq\S(\vec{x_1})\cup\cdots\cup\S(\vec{x_k})\subseteq \img(\S),
  \end{align*}
  where the last inequality holds because
  $\vec{x_i} \subseteq \dom(\S)$ for all $i$.
\end{proof}

\begin{corollary}\label{cor:btw:star-model-to-oursunion}
  Let $\phi_1,\phi_2 \in \SLIDguarded$ be guarded formulas and let
  $\Sid\in\IDbtw$. Let $\SH \sidmodels \phi_1\sep\phi_2$.
  %
  Then there exist heaps $\H_1,\H_2$ such that
  $\SHi{1},\SHi{2}\in\Mpos{\Sid}$, $\H = \H_1\stdunion\H_2$,
  $\SHi{1} \sidmodels \phi_1$ and $\SHi{2} \sidmodels \phi_2$.
\end{corollary}
\begin{proof}
  By the semantics of $\sep$, there exist $\H_1$, $\H_2$ with $\H =
  \H_1 \stdunion \H_2$, $\SHi{1}\sidmodels\phi_1$ and $\SHi{2}\sidmodels\phi_2$.
  %
  By \cref{lem:pos-formula-pos-model}, $\SHi{1},\SHi{2}\in\Mpos{\Sid}$.
\end{proof}

We will exploit this property of $\SLIDguarded$ in the decision
procedure we develop later in the \TypeOfDoc.

\begin{infobox}{The importance of guardedness for limiting dangling
  pointers}\index{guardedness}
  For all models to be guarded (\Cref{lem:pos-formula-pos-model}), it
  is crucial that all occurrences of negation, magic wand, and
  septraction in $\SLIDguarded$ are guarded.
%
For negation and the magic wand, this is straightforward, as they can
be used to define \emph{true} (e.g.~by $\emp\vee(\neg \emp)$ and
$(\ppto{x}{\nil}\sep\ppto{x}{\nil})\mw\emp$), and \emph{true} is
satisfied by all models, including non-guarded models.

For septraction, consider the following SID.
\[
  \begin{array}{lll}
    \gls{tll}(r,h,t)& \Rule & \pto{h}{t} \sep \sleq{r}{h} \\
    %
    \tll(r,h,t)& \Rule & \SHEX{\tuple{s_1,s_2,m}} \pbpto{r}{s_1,s_2} \sep
                 \tll(s_1,l,m) \sep \tll(s_2,m,r) \\
                 %
    \lseg(h, t)& \Rule & \pto{h}{t} \\
    %
    \lseg(h, t)& \Rule & \SHEX{n} \ppto{h}{n} \sep \lseg(n, t)
  \end{array}
\]
%
The $\tll$ predicate encodes a binary tree with root $r$ and leftmost
leaf $h$ overlaid with a singly-linked list segment from $h$ to $t$ whose nodes
are the leaves of the tree.
%
Now assume that $\SH \sidmodels \lseg(h,t) \sept \tll(r,h,t)$.  Then
there exists a heap $\H_1$ with $\SHi{1} \sidmodels \lseg(h,t)$ and
$\SHpair{\S}{\H\stdunion\H_1} \sidmodels \tll(r,h,t)$.
%
It is easy to see that $\danglinglocs{\H} = \dom(\H_1)$, contradicting
\Cref{lem:btw:pos-non-dangling}, which in turn implies that
$\lseg(h,t) \sept \tll(r,h,t)$ has non-guarded models.
\end{infobox}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Thesis"
%%% End:


==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}


==> figtbl/PartC/derived-rules.tex <==
    \begin{tabular}{cc}
    \textbf{Derived Rule} & \textbf{Proof} \\[18pt]
    %%%%
    % \AxiomC{}
    % \RightLabel{\RuleId}
    % \UnaryInfC{$\phi \deriveqf \phi$}
    % \DisplayProof{}
      \RuleId
    &
    %
      \footnotesize
      \AxiomC{}
      \RightLabel{(emp)}
      \UnaryInfC{$\phi \deriveqf \phi \sep \emp$}
      \AxiomC{}
      \RightLabel{(emp)}
      \UnaryInfC{$\phi \deriveqf \phi \sep \emp$}
      \RightLabel{(trans)}
      \BinaryInfC{$\phi \deriveqf \phi$}
      \DisplayProof{} \\[18pt]
      %%%%
    % \AxiomC{}
    % \RightLabel{\RuleMp}
    % \UnaryInfC{$(\phi_1 \mw \phi_2) \sep \phi_1 \deriveqf \phi_2$}
    %   \DisplayProof{}
      \RuleMp
                          &
                          %
                            \footnotesize
                    \AxiomC{}
                    \RightLabel{(id)}
                    \UnaryInfC{$\phi_1 \mw \phi_2 \deriveqf \phi_1\mw\phi_2$}
\RightLabel{(adj)}
                    \UnaryInfC{$(\phi_1 \mw \phi_2) \sep \phi_1 \deriveqf \phi_2$}
                    \DisplayProof{}
    \\[18pt]
    %%%%%%
% \AxiomC{}
%     \RightLabel{\RuleGMp}
%     \UnaryInfC{$((\phi_1\sep\psi) \mw \phi_2) \sep \phi_1 \deriveqf (\psi \mw \phi_2)$}
%     \DisplayProof{}
      \RuleGMp
                          &
                          %
                            \footnotesize
                      \AxiomC{}
                      \RightLabel{\RuleId}
                      \UnaryInfC{$\phi_2 \deriveqf \phi_2$}
                      \RightLabel{\RuleMp}
                      \UnaryInfC{$((\phi_1\sep\psi) \mw \phi_2) \sep (\phi_1 \sep \psi) \deriveqf \phi_2$}
    \RightLabel{\RuleAssoc}
    \UnaryInfC{$((\phi_1\sep\psi) \mw \phi_2) \sep \phi_1 \sep \psi \deriveqf \phi_2$}
    \RightLabel{\RuleAdj}
    \UnaryInfC{$((\phi_1\sep\psi) \mw \phi_2) \sep \phi_1 \deriveqf (\psi \mw \phi_2)$}
    \DisplayProof{}
    \\[36pt]
    %%%%%%
    % \AxiomC{}
%     \RightLabel{\RuleMwTrans}
%     \UnaryInfC{$(\phi \mw \psi) \sep (\psi \mw \zeta) \deriveqf \phi \mw \zeta$}
%     \DisplayProof{}
      \RuleMwTrans
                          &
                            \footnotesize
% Left subtree
\AxiomC{}
\RightLabel{\RuleId}
\UnaryInfC{$\psi \deriveqf \psi$}
\RightLabel{\RuleMp}
\UnaryInfC{$\phi \sep (\phi \mw \psi) \deriveqf \psi$}
\RightLabel{\RuleMono}
\UnaryInfC{$\phi \sep (\phi \mw \psi) \sep (\psi \mw \zeta) \deriveqf \psi \sep (\psi \mw \zeta)$}
% Right subtree
\AxiomC{}
\RightLabel{\RuleId}
\UnaryInfC{$\zeta \deriveqf \zeta$}
\RightLabel{\RuleMp}
\UnaryInfC{$\psi \sep (\psi \mw \zeta) \deriveqf \zeta$}
% Transitivity and below
\RightLabel{\RuleTrans}
\BinaryInfC{$\phi \sep (\phi \mw \psi) \sep (\psi \mw \zeta) \deriveqf \zeta$}
\RightLabel{\RuleAdj}
\UnaryInfC{$(\phi \mw \psi) \sep (\psi \mw \zeta) \deriveqf \phi \mw \zeta$}
\DisplayProof{}
\end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/deriveqf-full.tex <==
\begin{tabular}{cc}
    %
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
    \RightLabel{\RuleMono}
    \UnaryInfC{$\phi_1 \sep \psi \deriveqf \phi_2 \sep \psi$}
    \DisplayProof{} &
    %
    \AxiomC{$\bowtie \in \set{\deriveqf,\triangleleft}$}
    \RightLabel{\RuleEmp}
\UnaryInfC{$\phi_1 \sep \emp \bowtie \phi_1$}
    \DisplayProof{} \\[14pt]
    %%%
    %%%
    %%%
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
   \RightLabel{\RuleAnti}
   \UnaryInfC{$\phi_2 \mw \psi \deriveqf \phi_1 \mw \psi$}
                      \DisplayProof{}
                      %
    &
    \AxiomC{$\bowtie \in \set{\deriveqf,\triangleleft}$}
    \RightLabel{\RuleAssoc}
    \UnaryInfC{$\phi_1 \sep (\phi_2 \sep \phi_3) \bowtie (\phi_1 \sep \phi_2) \sep \phi_3$}
      \DisplayProof{}
    \\[14pt]
    %
    \AxiomC{}
    \RightLabel{\RuleComm}
    \UnaryInfC{$\phi_1 \sep \phi_2 \deriveqf \phi_2 \sep \phi_1$}
      \DisplayProof{}
    &
    %
        \AxiomC{$\phi_1 \deriveqf \phi_3$}
                      \AxiomC{$\phi_3 \deriveqf \phi_2$}
                      \RightLabel{\RuleTrans}
                      \BinaryInfC{$\phi_1 \deriveqf \phi_2$}
  \DisplayProof{} \\[14pt]
  %%%
  \multicolumn{2}{c}{
                    \AxiomC{}
                    \RightLabel{\RuleMwMw}
                    \UnaryInfC{$(\pred(\vec{z}) \sep \fa) \mw \pred'(\vec{y}) \sep (\fb \mw
                    \pred(\vec{z})) \deriveqf (\fa \sep \fb) \mw \pred'(\vec{y})$}
  \DisplayProof{}}
  \\[14pt]
  \end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/deriveqf-mp-rules.tex <==
% Proof system with the generalized modus ponens rule instead of the
% adjointness rule
\begin{tabular}{cc}
    %
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
    \RightLabel{\RuleMono}
    \UnaryInfC{$\phi_1 \sep \psi \deriveqf \phi_2 \sep \psi$}
    \DisplayProof{} &
    %
                      \AxiomC{$\bowtie \in \set{\deriveqf,\rderiveqf}$}
    \RightLabel{\RuleEmp}
\UnaryInfC{$\phi_1 \sep \emp \bowtie \phi_1$}
    \DisplayProof{}
     \\[14pt]
    %
%
    \AxiomC{$\bowtie \in \set{\deriveqf,\rderiveqf}$}
    \RightLabel{\RuleAssoc}
    \UnaryInfC{$\phi_1 \sep (\phi_2 \sep \phi_3) \bowtie (\phi_1 \sep \phi_2) \sep \phi_3$}
    \DisplayProof{}
    &
    %
    \AxiomC{}
    \RightLabel{\RuleComm}
    \UnaryInfC{$\phi_1 \sep \phi_2 \deriveqf \phi_2 \sep \phi_1$}
      \DisplayProof{}
    \\[14pt]
    %%%
  \AxiomC{$\phi_1 \deriveqf \phi_2$}
   \RightLabel{\RuleAnti}
   \UnaryInfC{$\phi_2 \mw \psi \deriveqf \phi_1 \mw \psi$}
  \DisplayProof{} &
  %
        \AxiomC{$\phi_1 \deriveqf \phi_3$}
                      \AxiomC{$\phi_3 \deriveqf \phi_2$}
                      \RightLabel{\RuleTrans}
                    \BinaryInfC{$\phi_1 \deriveqf \phi_2$}
  \DisplayProof{} \\[14pt]
  %
  \multicolumn{2}{c}{
                    \AxiomC{}
                    \RightLabel{\RuleMp}
                    \UnaryInfC{$(\pred(\vec{z}) \sep \fa) \mw \pred'(\vec{y}) \sep (\fb \mw
                    \pred(\vec{z})) \deriveqf (\fa \sep \fb) \mw \pred'(\vec{y})$}
  \DisplayProof{}
  }
  \end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/deriveqf-rules.tex <==
  \begin{tabular}{cc}
    %
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
    %\AxiomC{$\oplus \in \set{\sep,\mw}$}
    \RightLabel{\RuleMono}
    \UnaryInfC{$\phi_1 \sep \psi \deriveqf \phi_2 \sep \psi$}
    \DisplayProof{} &
    %
    \AxiomC{$\phi_1 \sep \phi_2 \deriveqf \phi_3$}
    \RightLabel{\RuleAdj}
    \doubleLine
    \UnaryInfC{$\phi_1 \deriveqf \phi_2 \mw \phi_3$}
    \DisplayProof{} \\[14pt]
    %
    \AxiomC{$\bowtie \in \set{\deriveqf,\rderiveqf}$}
    \RightLabel{\RuleEmp}
\UnaryInfC{$\phi_1 \sep \emp \bowtie \phi_1$}
    \DisplayProof{} &
    %%%
    %%%
    %%%
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
   \RightLabel{\RuleAnti}
   \UnaryInfC{$\phi_2 \mw \psi \deriveqf \phi_1 \mw \psi$}
    \DisplayProof{} \\[14pt]
%               \multicolumn{2}{l}{
    \AxiomC{$\bowtie \in \set{\deriveqf,\rderiveqf}$}
    \RightLabel{\RuleAssoc}
    \UnaryInfC{$\phi_1 \sep (\phi_2 \sep \phi_3) \bowtie (\phi_1 \sep \phi_2) \sep \phi_3$}
    \DisplayProof{}%}
    &
    %
    \AxiomC{}
    \RightLabel{\RuleComm}
    \UnaryInfC{$\phi_1 \sep \phi_2 \deriveqf \phi_2 \sep \phi_1$}
      \DisplayProof{}
    \\[14pt]
    %%%
    %%%
    %%%
        \AxiomC{$\phi_1 \deriveqf \phi_3$}
                      \AxiomC{$\phi_3 \deriveqf \phi_2$}
                      \RightLabel{\RuleTrans}
                      \BinaryInfC{$\phi_1 \deriveqf \phi_2$}
    \DisplayProof{} &
    %
    % \AxiomC{$\phi_1 \deriveqf \phi_2$}
    % \RightLabel{\RuleAIntro}
    % \UnaryInfC{$\FA{\vec{y}}\phi_1 \deriveqf \FA{\vec{y}}\phi_2$}
    % \DisplayProof{}
    % &
    % %
    % \AxiomC{$\phi_1 \deriveqf \phi_2$}
    % \RightLabel{\RuleEIntro}
    % \UnaryInfC{$\EX{\vec{y}}\phi_1 \deriveqf \EX{\vec{y}}\phi_2$}
    % \DisplayProof{}
    % \\[12pt]
    %%%
    %%%
    %%%
    % \AxiomC{}
    % \RightLabel{\RuleAInst}
    % \UnaryInfC{$\forall x. \phi \deriveqf \phi\subst{x}{y}$}
    % \DisplayProof{} &
    % %
    % \AxiomC{$x \notin \fvs{\phi}$}
    % \AxiomC{$Q \in \set{\forall, \exists}$}
    % \RightLabel{\RuleDistB}
    % \BinaryInfC{$\phi \sep (Qx. \psi) \deriveqf Qx. \phi \sep \psi$}
    % \DisplayProof{} &
    %

    %
% \AxiomC{$Q \in \set{\forall,\exists}$}
%     \AxiomC{$\vec{z} \cap \fvs{\phi} = \emptyset$}
%                       \RightLabel{\RuleRen}
%                       \BinaryInfC{$Q \vec{y}\ldotp\phi \deriveqf Q
%                                         \vec{z}\ldotp \phi[\vec{y}/\vec{z}]$}
%                                         \DisplayProof{}
%     \\
    %
    %
    % \AxiomC{$x \notin \fvs{\phi}$}
    % \RightLabel{\RuleDistA}
    % \UnaryInfC{$\phi \mw (\forall x. \psi) \deriveqf \forall x. \phi \mw \psi$}
    % \DisplayProof{} &
    %
    %%%

  \end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/deriveqf-simplified.tex <==
% Proof system with the generalized modus ponens rule instead of the
% adjointness rule
\begin{tabular}{ccc}
  %
  \multicolumn{3}{c}{
                    \AxiomC{}
                    \RightLabel{\RuleMwMw}
                    \UnaryInfC{$(\pred(\vec{z}) \sep \fa) \mw \pred'(\vec{y}) \sep (\fb \mw
                    \pred(\vec{z})) \deriveqf (\fa \sep \fb) \mw \pred'(\vec{y})$}
  \DisplayProof{}}
  \\[14pt]
  %
      \AxiomC{$\phi_1 \rewreq \phi_2$}
    \RightLabel{\RuleEq}
    \UnaryInfC{$\phi_1 \deriveqf \phi_2$}
  \DisplayProof{}
  &
    %
    \AxiomC{$\phi_1 \deriveqf \phi_2$}
    %\AxiomC{$\oplus \in \set{\sep,\mw}$}
    \RightLabel{\RuleMono}
    \UnaryInfC{$\phi_1 \sep \psi \deriveqf \phi_2 \sep \psi$}
    \DisplayProof{} &
                      %
  \AxiomC{$\phi_1 \deriveqf \phi_3$}
                      \AxiomC{$\phi_3 \deriveqf \phi_2$}
                      \RightLabel{\RuleTrans}
                    \BinaryInfC{$\phi_1 \deriveqf \phi_2$}
  \DisplayProof{} \\[14pt]
  %
  \end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/slid-semantics.tex <==
$\begin{array}{lll}
    \SH \gls{--models-sidmodels} \phi & \text{iff} &
    \H \sidmodels \pinst{\phi}{\dom(\S)}{\img(\S)} \\
\H \sidmodels\emp
& \text{iff} & \dom(\H)=\emptyset
  \\
\H \sidmodels \sleq{\ell_1}{\ell_2} & \text{iff} & \dom(\H)=\emptyset
                                                   \text{ and } \ell_1 = \ell_2 \\
\H \sidmodels \slneq{\ell_1}{\ell_2} & \text{iff} & \dom(\H)=\emptyset
                                                    \text{ and }\ell_1 \neq \ell_2 \\
%
\H \sidmodels \pto{v}{w}
& \text{iff} &
\H = \{ v \mapsto w \}
    \\
%
\H \sidmodels \pred(\vec{v})
  & \text{iff} &
\H \sidmodels \pinst{\phi}{\vec{x}}{\vec{v}} \text{ for
                 some rule } (\pred(\vec{x}) \Rule \psi)\in\Sid
    \\
%
\H \sidmodels \phi_1 \sep \phi_2
& \text{iff} &
\text{ex.}~\H_1,\H_2 ~\text{s.t.}~
\H = \H_1 \stdunion \H_2 \text{ and } \H_1 \sidmodels \phi_1
                                \\&& \text{and } \H_2 \sidmodels \phi_2
\\
%
\H \sidmodels \phi_1 \mw \phi_2
& \text{iff} &
\text{for all}~\H_1,\H_2 ~\text{s.t.}~
\H_2 = \H_1 \stdunion \H  \\
&&\text{it holds that if}~ \H_1 \sidmodels \phi_1
                                  ~\text{then}~ \H_2 \sidmodels \phi_2 \\
  %
  \H \sidmodels \phi_1 \wedge \phi_2
& \text{iff} & \H \sidmodels \phi_1 \text{ and } \H \sidmodels \phi_2\\
  %
  \H \sidmodels \phi_1 \vee \phi_2
& \text{iff} & \H \sidmodels \phi_1 \text{ or } \H \sidmodels
                 \phi_2\\
                 %
  \H \sidmodels \neg \phi_1
& \text{iff} & \H \not\sidmodels \phi_1\\
%
\H \sidmodels \exists e\ldotp \phi
& \text{iff} &
    \text{exists } v \in \Loc \text{~s.t.~} \H \sidmodels \pinst{\phi}{e}{v}\\
    %
% \H \sidmodels \forall a\ldotp \phi
% & \text{iff} &
%     \text{for all } v \in \Loc\ldotp \H \sidmodels \pinst{\phi}{a}{v} }{\phi}\\
%
  \end{array}$
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/syntax-sl-btw.tex <==
\[
  \begin{array}{lll}
    && u,v,u_i,v_i',\ldots \in \Var \cup \Loc,\\
    && \vec{u},\vec{v},\vec{w_i},\ldots\in\Var\cup\Loc^{*},
    \vec{e},\vec{a_i}\in\Var^{*}\\
    %
    \atomic & ::= & \emp \mid \pto{u}{\vec{v}} \mid \pred(\vec{u}) \mid
                    \sleq{u}{v} \mid \slneq{u}{v} \\
    %
    \phiGuarded & ::= & \atomic \mid \phiGuarded \sep \phiGuarded \mid \phiGuarded
                    \wedge \phiGuarded \mid \phiGuarded \vee \phiGuarded
    \\&&\phantom{\atomic}\mid \phiGuarded \wedge \neg \phiGuarded \mid \phiGuarded
    \wedge (\phiGuarded \sept \phiGuarded) \mid \phiGuarded
    \wedge (\phiGuarded \mw \phiGuarded)\\
    %
    \phiQf & ::= & \atomic \mid \phiQf \sep \phiQf \mid \phiQf \mw \phiQf \mid \phiQf \wedge \phiQf \mid \phiQf \vee \phiQf \mid
                 \neg \phiQf\\
                 %
    %
    \phi & ::= &\EEX{\vec{e}} (\FFA{\vec{a_1}} \phiQf) \sep \cdots
                 \sep (\FFA{\vec{a_k}} \phiQf) \\
                 %
    \phiSH & ::= & \SHEX{\vec{e}} \ppto{u_1}{\veci{v}{1}} \sep \cdots
                   \sep
    %\phiSH & ::= & \EEX{\vec{e}} \ppto{x_1}{\veci{y}{1}} \sep \cdots \sep
  \ppto{u_k}{\veci{v}{k}} \sep \pred_1(\veci{w}{1}) \sep
  \cdots \sep
             \pred_l(\veci{w}{l}) \sep \Pure, \\
             && \text{ where } \Pure ::= \sleq{u_1}{v_1} \sep \cdots \sep \sleq{u_m}{v_m} \sep
\slneq{u_1'}{v_1'} \sep \cdots \sep \slneq{u_n'}{v_n'}
  \end{array}
\]
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> figtbl/PartC/syntax-slid.tex <==
\[
  \begin{array}{lll}
    && u,v,u_i,v_i',\ldots \in \Var \cup \Loc,\\
    && \vec{u},\vec{v},\vec{w_i},\ldots\in\Var\cup\Loc^{*},
    \vec{e},\vec{a_i}\in\Var^{*}\\
    %
    \atomic & ::= & \emp \mid \pto{u}{\vec{v}} \mid \pred(\vec{u}) \mid
                    \sleq{u}{v} \mid \slneq{u}{v} \\
    %
    \phiGuarded & ::= & \atomic \mid \phiGuarded \sep \phiGuarded \mid \phiGuarded
                    \wedge \phiGuarded \mid \phiGuarded \vee \phiGuarded
    \\&&\phantom{\atomic}\mid \phiGuarded \wedge \neg \phiGuarded \mid \phiGuarded
    \wedge (\phiGuarded \sept \phiGuarded) \mid \phiGuarded
    \wedge (\phiGuarded \mw \phiGuarded)\\
    %
    \phiQf & ::= & \atomic \mid \phiQf \sep \phiQf \mid \phiQf \mw \phiQf \mid \phiQf \wedge \phiQf \mid \phiQf \vee \phiQf \mid
                 \neg \phiQf\\
                 %
    %
    % \phi & ::= &\EEX{\vec{e}} (\FFA{\vec{a_1}} \phiQf) \sep \cdots
    %              \sep (\FFA{\vec{a_k}} \phiQf) \\
                 %
    \phiSH & ::= & \SHEX{\vec{e}} \ppto{u_1}{\veci{v}{1}} \sep \cdots
                   \sep
    %\phiSH & ::= & \EEX{\vec{e}} \ppto{x_1}{\veci{y}{1}} \sep \cdots \sep
                    \ppto{u_k}{\veci{v}{k}} \\&&
                    %
                                                 \phantom{\SHEX{\vec{e}} \ppto{u_1}{\veci{v}{1}}}
                                                 \sep \pred_1(\veci{w}{1}) \sep
  \cdots \sep
             \pred_l(\veci{w}{l}) \sep \Pure, \\
             && \text{with } \Pure = \sleq{u_1}{v_1} \sep \cdots \sep \sleq{u_m}{v_m} \sep
\slneq{u_1'}{v_1'} \sep \cdots \sep \slneq{u_n'}{v_n'}
  \end{array}
\]
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> gfx/PartC/induced-models.tex <==
\newcommand{\FullInducedModel}{
  \begin{tikzpicture}
    \node[external] (x1) {$l_1\colon x_1$};
    \node[internal,above right=of x1] (y) {$l_4$};
    \node[external,right=of y] (x2) {$l_2\colon x_2$};
    \node[external,right=of x1] (x3) {$l_3\colon x_3$};
    \draw (x1) edge[->] node[above] {$\sel{1}$} (y);
    \draw (x1) edge[->] node[above] {$\sel{2}$} (x3);
    \draw (x3) edge[->] (x2);
    \draw (y) edge[->,bend left] (x2);
    \draw (x2) edge[->,bend left] (y);
  \end{tikzpicture}
}
%
\newcommand{\FirstInducedModel}{
  \begin{tikzpicture}
    \node[external] (x1) {$l_1 \colon x_1$};
    \node[internal,above right=of x1] (y) {$l_4$};
    \node[external,right=of y] (x2) {$l_2 \colon x_2$};
    \node[external,right=of x1] (x3) {$l_3 \colon x_3$};
    \draw (x1) edge[->] node[above] {$\sel{1}$} (y);
    \draw (x1) edge[->] node[above] {$\sel{2}$} (x3);
    \draw (y) edge[->,bend left] (x2);
    \draw (x2) edge[->,bend left] (y);
  \end{tikzpicture}
}
%
\newcommand{\SecondInducedModel}{
  \begin{tikzpicture}
    \node (x1) {};
    \node[above right=of x1] (y) {};
    \node[external,right=of y] (x2) {$l_2 \colon x_2$};
    \node[external,right=of x1] (x3) {$l_3 \colon x_3$};
    \draw (x3) edge[->] (x2);
  \end{tikzpicture}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Thesis"
%%% End:


==> gfx/PartC/undecidability-gadgets.tex <==
\newcommand{\oneedge}[4]{\draw (#1) edge[->]
  node[xshift=#3mm,yshift=#4mm] {$1$} (#2)}
\newcommand{\twoedge}[4]{\draw (#1) edge[->]
  node[xshift=#3mm,yshift=#4mm] {$2$} (#2)}

\newcommand{\xeqyGadget}{
\begin{tikzpicture}
  \node[internal] (1) {};
  \node[below=5mm of 1] (2) {$\bot$};
  \node[external,above left=8mm of 1] (x) {$x$};
  \node[external,above right=8mm of 1] (y) {$y$};
  \node[left=5mm of x] (xnil) {$\bot$};
  \node[right=5mm of y] (ynil) {$\bot$};
  \oneedge{x}{1}{1}{1};
  \oneedge{y}{1}{-1}{1};
  \twoedge{x}{xnil}{0}{2};
  \twoedge{y}{ynil}{0}{2};
  \draw (1) edge[->,bend left] node[right] {$2$} (2);
  \draw (1) edge[->,bend right] node[left] {$1$} (2);

  \begin{scope}[on background layer]
    \node[fill=gray!10,fit=(xnil)(ynil)(x)(y)(2)] {};
  \end{scope}

\end{tikzpicture}
}

\newcommand{\xneqyGadget}{
\begin{tikzpicture}
  \node[internal] (1) {};
  \node[below=5mm of 1] (2) {$\bot$};
  \node[internal,right=7mm of 1] (3) {};
  \node[below=5mm of 3] (4) {$\bot$};
  \node[external,above=8mm of 1] (x) {$x$};
  \node[external,above=8mm of 3] (y) {$y$};
  \node[left=5mm of x] (xnil) {$\bot$};
  \node[right=5mm of y] (ynil) {$\bot$};
  \oneedge{x}{1}{1}{1};
  \oneedge{y}{3}{-1}{1};
  \twoedge{x}{xnil}{0}{2};
  \twoedge{y}{ynil}{0}{2};
  \draw (1) edge[->,bend left] node[right] {$2$} (2);
  \draw (1) edge[->,bend right] node[left] {$1$} (2);
  \draw (3) edge[->,bend left] node[right] {$2$} (4);
  \draw (3) edge[->,bend right] node[left] {$1$} (4);

  \begin{scope}[on background layer]
    \node[fill=gray!10,fit=(xnil)(ynil)(x)(y)(2)(4)] {};
  \end{scope}
\end{tikzpicture}
}

\newcommand{\BxyeqGadget}{
  \begin{tikzpicture}
  \node[external] (z) {$\relv{x}{y}$};
  \node[internal,below=of z] (1) {};
  \node[below=5mm of 1] (2) {$\bot$};
  \node[external,left=8mm of 1] (x) {$x$};
  \node[external,right=8mm of 1] (y) {$y$};
  \node[below=5mm of x] (xnil) {$\bot$};
  \node[below=5mm of y] (ynil) {$\bot$};
  \oneedge{x}{1}{0}{2};
  \oneedge{y}{1}{0}{2};
  \twoedge{x}{xnil}{-2}{0};
  \twoedge{y}{ynil}{-2}{0};
  \draw (z) edge[->,bend left] node[right] {$2$} (1);
  \draw (z) edge[->,bend right] node[left] {$1$} (1);
  \draw (1) edge[->,bend left] node[right] {$2$} (2);
  \draw (1) edge[->,bend right] node[left] {$1$} (2);

  \begin{scope}[on background layer]
    \node[fill=gray!10,fit=(z)(xnil)(ynil)(x)(y)(2)] {};
  \end{scope}

\end{tikzpicture}
}

\newcommand{\BxyneqGadget}{
  \begin{tikzpicture}
  \node[external] (z) {$\relv{x}{y}$};
  \node[internal,below left=8mm of z] (1) {};
  \node[below=5mm of 1] (2) {$\bot$};
  \node[internal,below right=8mm of z] (3) {};
  \node[below=5mm of 3] (4) {$\bot$};
  \node[external,left=8mm of 1] (x) {$x$};
  \node[external,right=8mm of 3] (y) {$y$};
  \node[below=5mm of x] (xnil) {$\bot$};
  \node[below=5mm of y] (ynil) {$\bot$};
  \oneedge{x}{1}{0}{2};
  \oneedge{y}{3}{0}{2};
  \twoedge{x}{xnil}{-2}{0};
  \twoedge{y}{ynil}{-2}{0};
  \oneedge{z}{1}{-1}{1};
  \oneedge{z}{3}{1}{1};
  \draw (1) edge[->,bend left] node[right] {$2$} (2);
  \draw (1) edge[->,bend right] node[left] {$1$} (2);
  \draw (3) edge[->,bend left] node[right] {$2$} (4);
  \draw (3) edge[->,bend right] node[left] {$1$} (4);

  \begin{scope}[on background layer]
    \node[fill=gray!10,fit=(z)(xnil)(ynil)(x)(y)(2)] {};
  \end{scope}

\end{tikzpicture}
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../Journal"
%%% End:


==> math-macros.tex <==
\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\make@circled}[2]{%
  \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
  \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother

% overset with custom vertical spacing
\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-2\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General math macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\tuple}[1]{\ensuremath{\left\langle#1\right\rangle}}
\newcommand{\size}[1]{\ensuremath{\left|#1\right|}} % size, length, etc

\newcommand{\pfun}{\rightharpoonup}

% Sets of numbers
\newcommand{\N}{\mathbb{N}}

% O notation
\newcommand{\bigO}{\mathcal{O}}

\newcommand{\complexity}[1]{\textsc{#1}}
\newcommand{\NP}{\complexity{NP}}
\newcommand{\PSpace}{\complexity{PSpace}}
\newcommand{\PTime}{\complexity{PTime}}
\newcommand{\coNP}{\complexity{coNP}}
\newcommand{\ExpTime}{\complexity{ExpTime}}
\newcommand{\NExpTime}{\complexity{NExpTime}}
\newcommand{\TwoExpTime}{\complexity{2ExpTime}}
\newcommand{\TwoNExpTime}{\complexity{2NExpTime}}

\newcommand{\Iso}{\cong}
\newcommand{\entails}{\models}

\newcommand{\seqidx}[2]{#1[#2]}
\newcommand{\phiapp}[2]{#1(#2)}

% General math operators
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\img}{img}

\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\veci}[2]{\vec{#1}_{#2}}
\newcommand{\emptyseq}{\tuple{}}
%\newcommand{\emptyseq}{\varepsilon}
\newcommand{\concat}{\cdot}
\newcommand{\subfun}{\sqsubseteq}

\newcommand{\idfun}{\mathsf{id}}

\newcommand{\pfuncomp}{\circledcirc}

% definitions
%\newcommand{\defn}{\ensuremath{\stackrel{\textup{\tiny def}}{=}}}
\newcommand{\defn}{\triangleq}

% \newcommand{\xDownarrow}[1]{%
%   {\left\Downarrow\vbox to #1{}\right.\kern-\nulldelimiterspace}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General logic macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Quantifying over mathematical objects. (Not for use in SL formulas,
% where we use \EEX and \SHEX instead.)
\newcommand{\EXO}[1]{\exists #1\ldotp}
\newcommand{\FAO}[1]{\forall #1\ldotp}

% Substitution functions
\newcommand{\funapp}[2]{ #1\!\left[ #2 \right]}
\newcommand{\renfun}{\sigma}
%\newcommand{\instfun}[2]{\renfun_{#1\mapsto#2}}
\newcommand{\funcomp}{\circ}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Common SL macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Var}{\mathbf{Var}}
\newcommand{\Loc}{\mathbf{Loc}}
\newcommand{\Val}{\mathbf{Val}}

% \newcommand{\graphofKW}{\mathsf{graph}}
% \newcommand{\graphof}[1]{\mathsf{graph}(#1)}
\newcommand{\ugraphofKW}{\mathsf{graph}}
\newcommand{\ugraphof}[1]{\mathsf{graph}(#1)}
\newcommand{\igraphofKW}{\mathsf{igraph}}
\newcommand{\igraphof}[1]{\mathsf{igraph}(#1)}
% \newcommand{\lgraphofKW}{\mathsf{lgraph}}
% \newcommand{\lgraphof}[1]{\mathsf{lgraph}(#1)}
\newcommand{\DG}{\mathcal{G}}
\newcommand{\VDG}{V_\mathcal{G}}
\newcommand{\EDG}{E_\mathcal{G}}
%\newcommand{\LG}{\mathcal{\G}}
\newcommand{\lfun}{\nu}
%\newcommand{\nodesKW}{\mathsf{nodes}}
%\newcommand{\nodes}[1]{\nodesKW(#1)}

\newcommand{\step}[2]{#1 \rightarrow #2}
\newcommand{\nstep}[2]{#1 \not\rightarrow #2}
\newcommand{\istep}[3]{#2 \overset{#1}{\rightarrow} #3}
\newcommand{\stepstarArr}{\overset{*}{\rightarrow}}
\newcommand{\stepstarPlus}{\overset{+}{\rightarrow}}
\newcommand{\stepviaArr}[1]{\xrightarrow{#1 *}}
\newcommand{\stepstar}[2]{#1 \overset{*}{\rightarrow} #2}
\newcommand{\stepplus}[2]{#1 \overset{+}{\rightarrow} #2}
\newcommand{\stepregex}[3]{#2 \xrightarrow{#1} #3}
%\newcommand{\stepvia}[3]{\stepregex{#1 \N^{*}}{#2}{#3}}
\newcommand{\stepvia}[3]{\stepregex{#1 *}{#2}{#3}}
\newcommand{\stepG}[2]{#1 \rightarrow_\DG #2}
\newcommand{\nstepG}[2]{#1 \not\rightarrow_\DG #2}
\newcommand{\istepG}[3]{#2 \overset{#1}{\rightarrow}_\DG #3}
\newcommand{\stepstarG}[2]{#1 \overset{*}{\rightarrow}_\DG #2}
\newcommand{\stepplusG}[2]{#1 \overset{+}{\rightarrow}_\DG #2}
\newcommand{\stepregexG}[3]{#2 \xrightarrow{#1}_\DG #3}
% \newcommand{\stepviaG}[3]{\stepregex{#1 \N^{*}}{#2}{#3}}
\newcommand{\stepviaG}[3]{\stepregexG{#1 *}{#2}{#3}}
\newcommand{\stepH}[2]{#1 \rightarrow_\H #2}
\newcommand{\nstepH}[2]{#1 \not\rightarrow_\H #2}
\newcommand{\istepH}[3]{#2 \overset{#1}{\rightarrow}_\H #3}
\newcommand{\stepstarH}[2]{#1 \overset{*}{\rightarrow}_\H #2}
\newcommand{\stepplusH}[2]{#1 \overset{+}{\rightarrow}_\H #2}
\newcommand{\stepregexH}[3]{#2 \xrightarrow{#1}_\H #3}
\newcommand{\stepviaH}[3]{\stepregexH{#1 *}{#2}{#3}}
\newcommand{\nstepviaH}[3]{#2 \centernot{\xrightarrow{#1}}_\H #3}

\newcommand{\stepM}[2]{#1 \rightarrow_{\Msmt} #2}
\newcommand{\nstepM}[2]{#1 \not\rightarrow_{\Msmt} #2}
\newcommand{\istepM}[3]{#2 \overset{#1}{\rightarrow}_{\Msmt} #3}
\newcommand{\stepstarM}[2]{#1 \overset{*}{\rightarrow}_{\Msmt} #2}
\newcommand{\stepplusM}[2]{#1 \overset{+}{\rightarrow}_{\Msmt} #2}
\newcommand{\stepregexM}[3]{#2 \xrightarrow{#1}_{\Msmt} #3}
\newcommand{\stepviaM}[3]{\stepregexM{#1 *}{#2}{#3}}

\newcommand{\stkchoicefun}{stack-choice function}
\newcommand{\stkinv}{\S^{-1}}
\newcommand{\stkchc}{\S^{-1}_{\max}}

% Predicates
\newcommand{\ls}{\PredName{ls}}
\newcommand{\tree}{\PredName{tree}}
\newcommand{\topTree}{\PredName{treePtr}}
\newcommand{\restPred}{\PredName{rest}}
\newcommand{\topCyclic}{\PredName{cyclic}}
\newcommand{\fork}{\PredName{fork}}


\newcommand{\tll}{\PredName{tll}}
\newcommand{\tllHole}{\PredName{tllHole}}
\newcommand{\tllHoleHelper}{\PredName{helper}}
\newcommand{\tllListFour}{\PredName{list4}}
\newcommand{\tllListThree}{\PredName{list3}}
\newcommand{\tllListTwo}{\PredName{list2}}
\newcommand{\treerp}{\PredName{treeRP}}

%%%%%%%%%%%%%%%%%%%%
% Generic abstraction
%%%%%%%%%%%%%%%%%%%%

\newcommand{\AD}{\mathbb{A}}
\newcommand{\genabst}{\mathsf{abst}}

%%%%%%%%%%%%%%%%%%%%
% SL Fragments
%%%%%%%%%%%%%%%%%%%%

\newcommand{\SLgeneric}{\mathbf{SL}}

\newcommand{\SLbase}{\mathbf{SL}_{\mathbf{base}}}

% Part B
\newcommand{\SSL}{\mathbf{SSL}}
\newcommand{\WSL}{\mathbf{WSL}}
\newcommand{\WSLp}{\mathbf{WSL}^{+}}
%\newcommand{\BothSL}{\mathbf{WSL}\cup\mathbf{SSL}}
\newcommand{\SSLp}{\mathbf{SSL}^{+}}
\newcommand{\SSLdata}{\SSL_{\mathsf{data}}}
\newcommand{\SSLpdata}{\SSLdata^{+}}

% Part C
%\newcommand{\SLID}{\mathbf{SLID}}
\newcommand{\SLID}{\SLgeneric}
\newcommand{\GSLID}{\mathbf{GSL}}
\newcommand{\SLIDbtw}{\SLID_{\mathsf{btw}}}
\newcommand{\IDbtw}{\mathbf{ID}_{\mathsf{btw}}}

\newcommand{\AllSLIDguarded}{\GSLID^{\mathsf{g}}}
\newcommand{\AllSLIDqf}{\SLID^{\mathsf{qf}}}
\newcommand{\AllSLIDea}{\SLID^{\protect\eexistsSMALL\protect\fforallSMALL}}
\newcommand{\AllSLIDa}{\SLID^{\protect\fforallSMALL}}

\newcommand{\SLIDguarded}{\GSLID}
%\newcommand{\SLIDguarded}{\GSLID_{\mathsf{btw}}}
\newcommand{\SLIDqf}{\SLIDbtw^{\mathsf{qf}}}
%\newcommand{\SLIDea}{\SLIDbtw^{\exists\forall}}
%\newcommand{\SLIDa}{\SLIDbtw^{\forall}}
\newcommand{\SLIDea}{\SLIDbtw^{\protect\eexistsSMALL\protect\fforallSMALL}}
\newcommand{\SLIDa}{\SLIDbtw^{\protect\fforallSMALL}}
%\newcommand{\SLkw}{\mathbf{SL}}
% \newcommand{\SLop}[1]{\SLkw(#1)}
\newcommand{\SLop}[1]{\SLIDbtw(#1)}

\newcommand{\SymHeap}{\mathbf{SH}^{\exists}}
\newcommand{\Pure}{\Pi}

%%%%%%%%%%%%%%%%%%%%
% SL Syntax
%%%%%%%%%%%%%%%%%%%%

\newcommand{\fa}{\phi}
\newcommand{\fb}{\psi}
\newcommand{\fc}{\zeta}

\newcommand{\atomic}{\tau}

\newcommand{\nil}{0}
%\newcommand{\nil}{\mathsf{nil}}

\newcommand{\sleqSymbol}{\approx}
\newcommand{\sleq}[2]{#1 \approx #2}
\newcommand{\slneqSymbol}{\not\approx}
\newcommand{\slneq}[2]{#1 \not\approx #2}
\newcommand{\ptoArrow}{\mapsto}
\newcommand{\pto}[2]{#1 \ptoArrow #2}
\newcommand{\ppto}[2]{(#1 \ptoArrow #2)}
\newcommand{\bpto}[2]{#1 \ptoArrow \tuple{#2}}
\newcommand{\pbpto}[2]{(#1 \ptoArrow \tuple{#2})}
\newcommand{\ptosth}[1]{#1 \ptoArrow \_}
\newcommand{\emp}{\mathbf{emp}}

\newcommand{\sep}{\mathbin{\star}}
\newcommand{\mw}{\mathbin{-\!\!\star}}
% \newcommand{\sept}{{-\!\!\!\ostar}}
\newcommand{\sept}{\mathbin{\raisebox{-0.3pt}{$-$}\!\!\!\ostar}}
\newcommand{\septalt}{{-\!\!\circ}}
\newcommand{\wsep}{\mathbin{\star^{\mathbf{w}}}}

\newcommand{\gmw}{{-\!\!\bullet}}
\newcommand{\gsept}{{-\!\!\bullet}}

% \newcommand{\IteratedStar}{\mathop{\scalebox{1.5}{\raisebox{-0.2ex}{$\ast$}}}}%
\newcommand{\IteratedStar}{\bigstar}%

% Derived formulas
\newcommand{\true}{\mathsf{t}}
\newcommand{\false}{\mathsf{f}}
\newcommand{\ipto}[2]{#1 \hookrightarrow #2}
\newcommand{\isalloced}[1]{\mathsf{alloc}(#1)}

% Accessing vars
\newcommand{\allvsKW}{\mathsf{vars}}
\newcommand{\fvsKW}{\mathsf{fvars}}
%\newcommand{\bvsKW}{\mathsf{bvars}}
%\newcommand{\exvsKW}{\mathsf{bvars}_\exists}
%\newcommand{\favsKW}{\mathsf{bvars}_\forall}
\newcommand{\allvs}[1]{\allvsKW(#1)}
\newcommand{\fvs}[1]{\fvsKW(#1)}
%\newcommand{\bvs}[1]{\bvsKW(#1)}
%\newcommand{\exvs}[1]{\exvsKW(#1)}
%\newcommand{\favs}[1]{\favsKW(#1)}
\newcommand{\vallocKW}{\mathsf{alloced}}
\newcommand{\vrefedKW}{\mathsf{refed}}
\newcommand{\valloc}[1]{\vallocKW(#1)}
\newcommand{\vrefed}[1]{\vrefedKW(#1)}

% Other
\newcommand{\PredName}[1]{\mathsf{#1}}
\newcommand{\Q}[1]{\mathsf{#1}}

%%%%%%%%%%%%%%%%%%%%
% SL Semantics
%%%%%%%%%%%%%%%%%%%%

\newcommand{\stdunion}{\uplus}

% Stack-heap models

\renewcommand{\S}{\mathfrak{s}}
\renewcommand{\H}{\mathfrak{h}}
\newcommand{\barH}{\bar{\H}}
\newcommand{\SH}{\tuple{\S,\H}}
\newcommand{\SHpair}[2]{\tuple{#1,#2}}
\newcommand{\SHprime}{\tuple{\S,\H'}}
\newcommand{\SHpprime}{\tuple{\S',\H'}}
\newcommand{\SiHi}[1]{\tuple{\S_{#1},\H_{#1}}}
\newcommand{\SHi}[1]{\tuple{\S,\H_{#1}}}

% Sets of stacks and heaps
\renewcommand{\SS}{\mathbf{Stacks}}
\newcommand{\SSover}[1]{\mathbf{Stacks}^{#1}}
\newcommand{\HH}{\mathbf{Heaps}}
%\newcommand{\Mpos}[1]{\mathbf{Models}^{\mathsf{g}}_{#1}}
\newcommand{\Mpos}[1]{\mathbf{GStates}}
\newcommand{\States}{\mathbf{States}}

% Operations on stacks / heaps
\newcommand{\subheap}{\subseteq}

\newcommand{\danglinglocs}[1]{\mathsf{dangling}(#1)}

% Stack equivalences
% \newcommand{\eqclasses}[1]{\mathsf{cls}_{=}(#1)}
\newcommand{\eqclasses}[1]{\mathsf{aliasing}(#1)}
\newcommand{\eqclass}[2]{{[#2]}^{#1}_{=}}
\newcommand{\scls}{\mathbf{ac}}
%\newcommand{\scls}{\Sigma}
\newcommand{\EqClassesKW}{\mathbf{AC}}
\newcommand{\EqClasses}[1]{\EqClassesKW^{#1}}
\newcommand{\eqrestr}[2]{\left.#1\right|_{#2}}
% \newcommand{\eqextensionsKW}{\mathsf{extensions}}
% \newcommand{\eqextensions}[2]{\eqextensionsKW_{#1}(#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IJCAR macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SLstar}{\mathbf{SL}^{*}_{\mathsf{data}}}

\DeclareMathOperator{\sort}{sort}
\newcommand{\Fld}{\mathsf{Fld}}

\newcommand{\ptols}[2]{#1 \ptoArrow_{\fnext} #2}
\newcommand{\ptotree}[2]{#1 \ptoArrow_{\fleft,\fright} #2}
\newcommand{\ptolsd}[2]{#1 \ptoArrow_{\lsDS} #2}
\newcommand{\ptotreed}[2]{#1 \ptoArrow_{\treeDS} #2}
\newcommand{\ptodsd}[2]{#1 \ptoArrow_{\anyDS} #2}
\newcommand{\pptols}[2]{(#1 \ptoArrow_{\fnext} #2)}
\newcommand{\pptotree}[2]{(#1 \ptoArrow_{\fleft,\fright} #2)}
\newcommand{\pptolsd}[2]{(#1 \ptoArrow_{\lsDS} #2)}
\newcommand{\pptotreed}[2]{(#1 \ptoArrow_{\treeDS} #2)}
\newcommand{\pptodsd}[2]{(#1 \ptoArrow_{\anyDS} #2)}

%\newcommand{\ptof}[3]{#2 \ptoArrow_{#1} #3}
%\newcommand{\pptof}[3]{(#2 \ptoArrow_{#1} #3)}
%\newcommand{\ptoM}[2]{\ptof{\M}{#1}{#2}}
%\newcommand{\ptoMstar}[2]{#1 \ptoArrow^{*}_{\M} #2}
%\newcommand{\ptoMplus}[2]{#1 \ptoArrow^{+}_{\M} #2}
\newcommand{\holesdistinct}[1]{\mathsf{distinct}(#1)}

% Sorts
\newcommand{\sbool}{\mathbf{Bool}}
\newcommand{\sint}{\mathbf{Int}}
% \newcommand{\sdata}{\mathsf{data}}
\newcommand{\sdata}{\mathbf{Data}}
\newcommand{\streelocKW}{\mathsf{loc}_\tree}
\newcommand{\streeloc}[1]{\mathsf{loc}_\tree(#1)}
\newcommand{\slistlocKW}{\mathsf{loc}_\ls}
\newcommand{\slistloc}[1]{\mathsf{loc}_\ls(#1)}
%\newcommand{\spredloc}{\mathsf{loc}_\pred}
%\newcommand{\sbothloc}{\mathsf{loc}}
\newcommand{\sbothloc}{\mathbf{Loc}}
\newcommand{\sarray}{\mathbf{Array}}

% Fields
\newcommand{\fld}[1]{\mathsf{#1}}
\newcommand{\fany}{\fld{f}}
\newcommand{\fanyb}{\fld{g}}
\newcommand{\fleft}{\fld{l}}
\newcommand{\fright}{\fld{r}}
\newcommand{\fnext}{\fld{n}}
\newcommand{\fprev}{\fld{p}}
\newcommand{\fdata}{\fld{d}}

% Data
\newcommand{\Tdata}{\mathcal{T}_{\sdata}}
\newcommand{\Tloc}{\mathcal{T}_{\sbothloc}}
\newcommand{\predvara}{\alpha}
\newcommand{\predvarb}{\beta}

% Semantics
%\newcommand{\Models}{\mathbf{M}}
%\newcommand{\M}{\mathcal{M}}
%\newcommand{\Rest}[2]{ \sfrac{#1}{#2} }
%\newcommand{\submodels}{\mid\!\subseteq}
%\newcommand{\supmodels}{\mid\!\supseteq}
%\newcommand{\MC}{\mathcal{C}}
\newcommand{\comp}{\oplus}

\newcommand{\boundnodata}[3]{2#1 + (2+#3)#2}
% \newcommand{\boundwithdata}[5]{2#1 + (3 + k)#2 + 2#3 + 2#4}
\newcommand{\boundwithdata}[4]{2#1 + (2+#4)#2 + 2#3}

% Encoding
% \newcommand{\zthree}{\texttt{z3}}
% \newcommand{\smtsort}[1]{\mathsf{#1}}
% \newcommand{\CAL}{\mathbf{CAL}}
% \newcommand{\EUF}{\mathbf{EUF}}
% \newcommand{\unroll}{\mathsf{unroll}}
% \newcommand{\encode}{\mathsf{enc}}
% \newcommand{\boundf}{\mathsf{bound}}
% \newcommand{\sat}{\mathsf{sat}}
% \newcommand{\arr}[2]{\mathbf{A}_{#1}^{#2}}
% \newcommand{\FP}{Y}
% \newcommand{\store}[1]{\mathsf{store}(#1)}
% \newcommand{\singletonstore}[1]{\store{\Kfalse, #1, true}}
% \newcommand{\Kcomb}[1]{\mathbf{K}\left(#1\right)}
% \newcommand{\Kfalse}{\Kcomb{\bot}}
% \newcommand{\Map}[2]{\mathsf{map}_{#1}\left({#2}\right)}
% \newcommand{\MapAnd}[1]{\Map{\wedge}{#1}}
% \newcommand{\MapOr}[1]{\Map{\vee}{#1}}
% \newcommand{\bound}{\mathbf{B}}

%\newcommand{\SLLB}{SLL\mathbb{B}} % GRASS
%\newcommand{\infer}{\textsc{Infer}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SSL SL macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\loc}{\ell}
\newcommand{\locAlt}{k}

% Syntactic categories
\newcommand{\phiAtom}{\phi_{\mathsf{atom}}}
\newcommand{\phiSpatial}{\phi_{\mathsf{spatial}}}
\newcommand{\phiPos}{\phi_{\mathsf{pos}}}
\newcommand{\phiWSpatial}{\phi^{\mathbf{w}}_{\mathsf{spatial}}}
\newcommand{\phiWPos}{\phi^{\mathbf{w}}_{\mathsf{pos}}}

% Disjoint-union operators
\newcommand{\anyunion}{\oplus}
\newcommand{\ourunion}{\uplus}
\newcommand{\oursunion}{\uplus^{\S}}
\newcommand{\ourspunion}{\uplus^{\S'}}

% Strong and weak model relationships
% \newcommand{\oursup}{\scriptscriptstyle\mathsf{st}}
% \newcommand{\stdsup}{~\scriptscriptstyle\mathsf{wk}}
% \newcommand{\imodels}[1]{\oset[-0.6ex]{#1}{\models}}
% \newcommand{\notimodels}[1]{\oset[-0.3ex]{#1}{\not\models}}
% \newcommand{\stdmodels}{\imodels{\stdsup}}
% \newcommand{\ourmodels}{\imodels{\oursup}}
% \newcommand{\nourmodels}{\notimodels{\oursup}}
% \newcommand{\anymodels}{\models}
\newcommand{\ourmodels}{\models}
\newcommand{\stdmodels}{\models}
\newcommand{\anymodels}{\models}
\newcommand{\nmodels}{\not\models}

%\newcommand{\ientails}[1]{\imodels{\oursup}_{#1}}
%\newcommand{\notientails}[1]{\notimodels{\oursup}_{#1}}
\newcommand{\entailsx}{\entails_{\vec{x}}}

% chunks etc
\newcommand{\chunks}{\mathsf{chunks}}
\newcommand{\goodchunksKW}{\mathsf{chunks}^{+}}
\newcommand{\goodchunks}[1]{\goodchunksKW(#1)}
\newcommand{\badchunksKW}{\mathsf{chunks}^{-}}
\newcommand{\badchunks}[1]{\badchunksKW(#1)}

% AMS abstraction
\newcommand{\AMS}{\mathbf{AMS}}
\newcommand{\AMSs}{\mathbf{AMS}_{\S}}
\newcommand{\AMSks}{\mathbf{AMS}_{k,\S}}
\newcommand{\amsofKW}{\mathsf{ams}} % Used to be mabst
\newcommand{\amsof}[1]{\mathsf{ams}(#1)} % Used to be mabst
\newcommand{\Compose}{\bullet}

\newcommand{\iedge}{\mathsf{edges}_\S}
% \newcommand{\eqone}{=\!1}
% \newcommand{\geqtwo}{\geq\!2}
\newcommand{\eqone}{[\!=\!\!1\!]}
\newcommand{\geqtwo}{[\!\geq\!\!2\!]}
\newcommand{\somesize}{[\!\sim\!\!n\!]}
\newcommand{\domV}{\dom_\V}
\newcommand{\fields}[2]{\mathsf{fields}_#1(#2)}

\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\V}{V}
\newcommand{\E}{E}
\newcommand{\garb}{\gamma}
\newcommand{\Rset}{\rho}
%\newcommand{\mfc}{\mu}
%\newcommand{\mfccomps}{\tuple{\Rset,\garb}}
%\newcommand{\mfccompsi}[1]{\tuple{\Rset_{#1},\garb_{#1}}}

%\newcommand{\mabst}{\mathsf{ams}}
\newcommand{\abst}[2]{\mathsf{abst}_{#1}(#2)}
\newcommand{\lift}[3]{\mathsf{lift}_{#1 \nearrow #2}(#3)}
\newcommand{\liftKW}[2]{\mathsf{lift}_{#1 \nearrow #2}}

\newcommand{\Aset}{\mathbf{A}}

% SSL
\newcommand{\csize}[1]{\ensuremath{\lceil #1\rceil}} % chunk size

%\newcommand{\succs}[2]{\mathsf{succs}_{#1}(#2)}
%\newcommand{\pres}[2]{\mathsf{pres}_{#1}(#2)}
%\newcommand{\rootsAMS}[1]{\mathsf{roots}(#1)}
%\newcommand{\sourcesAMS}[1]{\mathsf{sources}(#1)}
%\newcommand{\rootvarsAMS}[2]{\mathsf{rootvs}_{#1}(#2)}
\newcommand{\sourcevarsKW}{\mathsf{sourcevars}}
\newcommand{\sourcevars}[2]{\mathsf{sourcevars}_{#1}(#2)}
\newcommand{\sinkvarsKW}{\mathsf{sinkvars}}
\newcommand{\sinkvars}[2]{\mathsf{sinkvars}_{#1}(#2)}
\newcommand{\sources}[1]{\mathsf{sources}(#1)}
\newcommand{\sinkseqKW}{\mathsf{sinkseq}}
\newcommand{\sinkseq}[1]{\mathsf{sinkseq}(#1)}

\newcommand{\allocAMSKW}{\mathbf{alloc}}
\newcommand{\allocAMS}[1]{\mathbf{alloc}(#1)}
\newcommand{\mfallocKW}{\mathsf{alloc}^{-}}
\newcommand{\mfalloc}[1]{\mfallocKW(#1)}

\newcommand{\AMquadruple}{\tuple{\V,\E,\Rset,\garb}}
\newcommand{\AMquadruplei}[1]{\tuple{\V_{#1},\E_{#1},\Rset_{#1},\garb_{#1}}}
% \newcommand{\eqclassesAMS}[1]{\mathsf{cls}_{=}(#1)}
\newcommand{\eqclassesAMS}[1]{\mathsf{classes}(#1)}
\newcommand{\eqclassAMS}[2]{{[#2]}^{#1}_{=}}
\newcommand{\phiabstkw}{\mathsf{ams}}
\newcommand{\phiabsts}[2]{\phiabstkw_{#1}(#2)}
\newcommand{\phiabstx}[2]{\phiabstkw_{#1}(#2)}

\newcommand{\rsizeKW}{\mathsf{rsize}}
\newcommand{\rsize}[1]{\rsizeKW(#1)}
\newcommand{\sslpdatabound}[1]{\mathsf{bound}(#1)}

% QBF encoding
\newcommand{\qbftr}[1]{\mathsf{qbf\_to\_sl}(#1)}
\newcommand{\qbfaux}[1]{\mathsf{aux}(#1)}

% Data SSL chapter
\newcommand{\istepA}[3]{#2 \overset{#1}{\rightarrow}_\A #3}
\newcommand{\stepA}[2]{#1 \rightarrow_\A #2}
\newcommand{\stepregexA}[3]{#2 \xrightarrow{#1}_\A #3}
\newcommand{\stepviaA}[3]{\stepregexA{#1 *}{#2}{#3}}
\newcommand{\stepplusA}[2]{#1 \overset{+}{\rightarrow}_\A #2}
%\newcommand{\stepstarA}[2]{#1 \overset{*}{\rightarrow}_\A #2}

\newcommand{\suppairs}[2]{\mathsf{S}_{#2}(#1)}
\newcommand{\EA}{\mathcal{E}}

\newcommand{\dfunAMS}{\delta}
\newcommand{\EAMpair}{\tuple{\A,\dfunAMS}}
\newcommand{\fset}{\mathbf{f}}
\ifdefined\vv\renewcommand{\vv}{v}\else\newcommand{\vv}{v}\fi
\newcommand{\ww}{\vec{w}}
\newcommand{\eamsofKW}{\mathsf{eams}}
\newcommand{\eamsof}[1]{\mathsf{eams}_{\Iset,\Pset}(#1)}
\newcommand{\sdcof}[1]{\mathsf{dconstraint}_{\phi}(#1)}
\newcommand{\sdcofs}{\mathsf{dconstraint}_{\phi}(\S)}
\newcommand{\sdc}{\mathsf{S}}
\newcommand{\SDCphix}{\mathbf{SDC}(\phi,\vec{x})}

\newcommand{\ltAP}{\prec}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Part B macros **BBBB**
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\Sort}{S}
%\newcommand{\Sorts}{\mathcal{S}}
\newcommand{\FData}{\mathcal{F}_\sdata}
\newcommand{\sortofKW}{\mathsf{sort}}
\newcommand{\sortof}[1]{\sortofKW(#1)}

\newcommand{\lstwo}{\ls_{\geq2}}
\newcommand{\treetwo}{\tree_{\geq2}}
\newcommand{\anyDStwo}{\anyDS_{\geq2}}

\newcommand{\DS}{\mathcal{D}}
\newcommand{\lsDS}{\ls}
\newcommand{\treeDS}{\tree}
\newcommand{\anyDS}{\mathsf{ds}}

\newcommand{\nodeSigKw}{\mathsf{sig}}
\newcommand{\nodeSig}[1]{\nodeSigKw(#1)}

\newcommand{\datamodels}{\models_{\sdata}}

\newcommand{\weakenKW}{\mathsf{weaken}}
\newcommand{\weaken}[1]{\mathsf{weaken}(#1)}
\newcommand{\strenghten}[1]{\mathsf{strengthen}(#1)}

\newcommand{\ptoH}[2]{#1 \ptoArrow_\H #2 }
\newcommand{\ptoHstar}[2]{#1 \ptoArrow^{*}_{\H} #2}
\newcommand{\ptoHplus}[2]{#1 \ptoArrow^{+}_{\H} #2}

\newcommand{\remloc}[2]{#1 - #2}

\newcommand{\AbstListsKW}{\mathbf{AbstLists}}
\newcommand{\AbstLists}[3]{\AbstListsKW(#1,#2,#3)}
\newcommand{\AbstGeqtwoLists}[3]{\AbstListsKW_{\geq 2}(#1,#2,#3)}
\newcommand{\AbstTreesKW}{\mathbf{AbstTrees}}
\newcommand{\AbstTrees}[3]{\AbstTreesKW(#1,#2,#3)}
\newcommand{\AbstGeqtwoTrees}[3]{\AbstTreesKW_{\geq 2}(#1,#2,#3)}

% Data predicates

% \newcommand{\anyqf}{Q}
\newcommand{\anyqf}{\mathord{\rotatebox[origin=c]{180}{$\mathsf{Q}$}}}
\newcommand{\Pset}{\mathcal{P}}
\newcommand{\dform}{F}
\newcommand{\Dforms}{\vec{D}}
\newcommand{\DFset}{\mathcal{F}}
\newcommand{\dpred}{P}
\newcommand{\exbdp}[2]{ {[#1\colon #2]}^{\exists}  }
\newcommand{\fabdp}[2]{ {[#1\colon #2]}^{\forall}  }
\newcommand{\anybdp}[2]{ {[#1\colon #2]}^{\anyqf}  }
\newcommand{\exudp}[1]{ {[#1]}^{\exists}  }
\newcommand{\faudp}[1]{ {[#1]}^{\forall}  }
\newcommand{\anyudp}[1]{ {[#1]}^{\anyqf}  }
\newcommand{\Iset}{\mathcal{I}}

\newcommand{\dpsof}[1]{\Pset(#1)}
\newcommand{\callsof}[1]{\Iset(#1)}

\newcommand{\exbdpofKW}{\mathsf{binary}^{\exists}}
\newcommand{\exbdpof}[1]{\exbdpofKW(#1)}
\newcommand{\fabdpofKW}{\mathsf{binary}^{\forall}}
\newcommand{\fabdpof}[1]{\fabdpofKW(#1)}
\newcommand{\exudpofKW}{\mathsf{unary}^{\exists}}
\newcommand{\exudpof}[1]{\exudpofKW(#1)}
\newcommand{\faudpofKW}{\mathsf{unary}^{\forall}}
\newcommand{\faudpof}[1]{\faudpofKW(#1)}

\newcommand{\decidesslpKW}{\mathsf{decide}^{+}}
\newcommand{\decidesslp}[1]{\mathsf{decide}^{+}(#1)}

\newcommand{\DataConstraintsKW}{\mathbf{DataConstraints}}
\newcommand{\DataConstraints}[2]{\DataConstraintsKW(#1,#2)}
\newcommand{\ConsistentConstraintsKW}{\mathbf{ConsistentEAMS}}
\newcommand{\ConsistentConstraints}[2]{\ConsistentConstraintsKW_{#1}(#2)}
\newcommand{\subsumedAMSKW}{\mathsf{subsumed}}
\newcommand{\subsumedAMS}[2]{\mathsf{subsumed}(#1,#2)}
\newcommand{\saturateAMSKW}{\mathsf{saturate}}
\newcommand{\saturateAMS}[3]{\mathsf{saturate}_{#1,#2}(#3)}
\newcommand{\saturateAMSIP}[1]{\mathsf{saturate}_{\Iset,\Pset}(#1)}
\newcommand{\eabstKW}{\mathsf{eabst}}
\newcommand{\eabst}[4]{\eabstKW_{#1,#2,#3}(#4)}
\newcommand{\eabstSIP}[1]{\eabst{\S}{\Iset}{\Pset}{#1}}
\newcommand{\eabstDIP}[1]{\eabst{\sdc}{\Iset}{\Pset}{#1}}
\newcommand{\eabsttop}[2]{\eabstKW_{#1}(#2)}
\newcommand{\dropdpKW}{\mathsf{dropdata}}
\newcommand{\dropdp}[1]{\mathsf{dropdata}(#1)}

\newcommand{\EAMS}{\mathbf{EAMS}_{\Iset,\Pset}}
%\newcommand{\EAMSk}[1]{\mathbf{EAMS}_{\Iset,\Pset,#1}}
\newcommand{\EAMSks}[2]{\mathbf{EAMS}_{\Iset,\Pset,#1,#2}}
\newcommand{\REAMSphis}{\mathbf{REAMS}_{\phi,\S}}
\newcommand{\REAMSphix}{\mathbf{REAMS}_{\phi,\vec{x}}}
\newcommand{\Eset}{\mathbf{E}}
\newcommand{\phieabstKW}{\mathsf{eams}}
\newcommand{\phieabsts}[2]{\phieabstKW_{#1}(#2)}
\newcommand{\phieabstx}[1]{\phieabstKW_{\vec{x}}(#1)}
\newcommand{\charformKW}{\mathsf{char}}
\newcommand{\charform}[1]{\charformKW(#1)}
\newcommand{\sdcmodels}{\models_{\mathbf{SDC}}}
% \newcommand{\stackof}[1]{\mathsf{stack(#1)}}
\newcommand{\realization}[1]{\mathsf{realization}(#1)}
\newcommand{\dconstraintphi}[1]{\mathsf{dconstraint}(#1)}
\newcommand{\encsdc}[1]{\mathsf{encode}^{\mathbf{SDC}}_\phi(#1)}

\newcommand{\DCompose}{\Compose_{\sdata}}
\newcommand{\Dgmw}{\gmw_{\sdata}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SID / BTW SL macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Syntax
\newcommand{\phiGuarded}{\phi}
%\newcommand{\phiGuarded}{\phi_{\mathsf{g}}}
\newcommand{\phiQf}{\phi_{\mathsf{qf}}}
\newcommand{\phiSH}{\phi_{\mathsf{sh}}}

\newcommand{\PredsKW}{\mathbf{Preds}}
\newcommand{\Preds}[1]{\PredsKW(#1)}
\newcommand{\pred}{\PredName{pred}}
\newcommand{\arity}[1]{\arityKW(#1)}
\newcommand{\arityKW}{\mathsf{ar}}
\newcommand{\Sid}{\Phi}
%\newcommand{\fpredsKW}{\mathsf{preds}}
%\newcommand{\fpreds}[1]{\fpredsKW(#1)}

\newcommand{\Rule}{\Leftarrow}

\newcommand{\prootKW}{\mathsf{predroot}}
\newcommand{\proot}[1]{\prootKW(#1)}
\newcommand{\sidrootvarsKW}{\mathsf{rootvars}}
\newcommand{\sidrootvars}[1]{\sidrootvarsKW_{\Sid}(#1)}
\newcommand{\dushrootsKW}{\mathsf{dushroots}}
\newcommand{\dushroots}[1]{\dushrootsKW_\S(#1)}

\newcommand{\rewreq}{\equiv}

\newcommand{\sel}[1]{#1} % Selector

% Model relationship / semantics
\newcommand{\locsKW}{\mathsf{locs}}
\newcommand{\locs}[1]{\locsKW(#1)}
% \newcommand{\nilloc}{\mathbf{0}}
\newcommand{\nilloc}{0}

\newcommand{\valuesKW}{\mathsf{values}}
\newcommand{\values}[1]{\valuesKW(#1)}

\newcommand{\la}{l}
\newcommand{\lb}{l'}

\newcommand{\sidmodels}{\modelswith{\Sid}}
\newcommand{\modelswith}[1]{\models_{#1}}

\newcommand{\RuleInst}[1]{\mathbf{RuleInst}(#1)}

\newcommand{\lallocKW}{\mathsf{lalloc}}
\newcommand{\lrefKW}{\mathsf{lref}}
\newcommand{\lusedKW}{\mathsf{lused}}
\newcommand{\lfunKW}{\mathsf{lfun}}
\newcommand{\lalloc}[1]{\lallocKW(#1)}
\newcommand{\lref}[1]{\lrefKW(#1)}
\newcommand{\lused}[1]{\lusedKW(#1)}

% Forests
\newcommand{\ftree}{\mathfrak{t}}
\newcommand{\bartree}{\bar{\ftree}}
\newcommand{\subtree}{\ftree_{\mathsf{sub}}}
\newcommand{\remtree}{\ftree_{\mathsf{rem}}}
\newcommand{\subpred}{\pred_{\mathsf{sub}}}
\newcommand{\frst}{\mathfrak{f}}
\newcommand{\barfrst}{\bar{\frst}}
\newcommand{\frstb}{\mathfrak{g}}
\newcommand{\barfrstb}{\bar{\mathfrak{g}}}
\newcommand{\ktrees}{\set{\ftree_1,\ldots,\ftree_k}}
\newcommand{\WitnessType}{\Loc \pfun \left(2^\Loc \times
    \RuleInst{\Sid} \right)}
%\newcommand{\subtree}{\sqsubseteq}

% Accessors for trees and forests
\newcommand{\tgraphKW}{\mathsf{graph}}
\newcommand{\tgraph}[1]{\tgraphKW(#1)}
\newcommand{\theadKW}{\mathsf{head}}
\newcommand{\thead}[2]{\theadKW_{#1}(#2)}
%\newcommand{\tbodyKW}{\mathsf{body}}
%\newcommand{\tbody}[2]{\tbodyKW_{#1}(#2)}
\newcommand{\tcallsKW}{\mathsf{calls}}
\newcommand{\tcalls}[2]{\tcallsKW_{#1}(#2)}
\newcommand{\truleinstKW}{\mathsf{rule}}
\newcommand{\truleinst}[2]{\truleinstKW_{#1}(#2)}
\newcommand{\locheapofKW}{\mathsf{heap}}
\newcommand{\locheapof}[2]{\locheapofKW_{#1}(#2)}
\newcommand{\tholesKW}{\mathsf{holes}}
\newcommand{\tholes}[2]{\tholesKW_{#1}(#2)}
\newcommand{\tholepredsKW}{\mathsf{holepreds}}
\newcommand{\tholepreds}[2]{\tholepredsKW_{#1}(#2)}
\newcommand{\tsuccKW}{\mathsf{succ}}
\newcommand{\tsucc}[2]{\tsuccKW_{#1}(#2)}

\newcommand{\trootKW}{\mathsf{root}}
\newcommand{\troot}[1]{\trootKW(#1)}
\newcommand{\trootpredKW}{\mathsf{rootpred}}
\newcommand{\trootpred}[1]{\trootpredKW(#1)}
\newcommand{\tallholesKW}{\mathsf{allholes}}
\newcommand{\tallholes}[1]{\tallholesKW(#1)}
\newcommand{\tallholepredsKW}{\mathsf{allholepreds}}
\newcommand{\tallholepreds}[1]{\tallholepredsKW(#1)}
\newcommand{\theapofKW}{\mathsf{heap}}
\newcommand{\theapof}[1]{\theapofKW(#1)}
\newcommand{\tptrlocsKW}{\mathsf{ptrvalues}}
%\newcommand{\tptrlocsKW}{\mathsf{ptrlocs}}
\newcommand{\tptrlocs}[1]{\tptrlocsKW(#1)}

\newcommand{\fgraphKW}{\mathsf{graph}}
\newcommand{\fgraph}[1]{\fgraphKW(#1)}
\newcommand{\frootsKW}{\mathsf{roots}}
\newcommand{\froots}[1]{\frootsKW(#1)}
\newcommand{\frootpredsKW}{\mathsf{rootpreds}}
\newcommand{\frootpreds}[1]{\frootpredsKW(#1)}
\newcommand{\fallholesKW}{\mathsf{allholes}}
\newcommand{\fallholes}[1]{\fallholesKW(#1)}
\newcommand{\fallholepredsKW}{\mathsf{allholepreds}}
\newcommand{\fallholepreds}[1]{\fallholepredsKW(#1)}
%\newcommand{\fptrsKW}{\mathsf{ptrs}}
%\newcommand{\fptrs}[1]{\fptrsKW(#1)}
% \newcommand{\fbodyKW}{\mathsf{body}}
% \newcommand{\fbody}[2]{\fbodyKW_{#1}(#2)}
\newcommand{\fruleinstKW}{\mathsf{rule}}
\newcommand{\fruleinst}[2]{\fruleinstKW_{#1}(#2)}

% Working with trees and forests
\newcommand{\theightKW}{\mathsf{height}}
\newcommand{\theight}[1]{\theightKW(#1)}
\newcommand{\subforest}{\subseteq}
\newcommand{\funion}{\uplus}
\newcommand{\fderive}{\blacktriangleright}
\newcommand{\fderivestar}{\blacktriangleright^{*}}
\newcommand{\tattachSYM}{\nearrow}
\newcommand{\tattach}[1]{\tattachSYM_{#1}}
\newcommand{\tunion}[1]{\mathsf{treeunions}(#1)}
\newcommand{\treach}[3]{\mathsf{reach}_{#1}(#2,#3) }
%\newcommand{\trestr}[3]{\left.#1\right|_{#2 \rightsquigarrow #3}}
\newcommand{\tsplit}[2]{\mathsf{split}(#1,#2)}
\newcommand{\fsplit}[2]{\mathsf{split}(#1,#2)}

\newcommand{\tentry}[4]{#1 \mapsto \tuple{#2, #3 \Rule #4}}

% Sets of forests
\newcommand{\frstsofKW}{\mathsf{forests}}
\newcommand{\frstsof}[2]{\frstsofKW_{#1}(#2)}
\newcommand{\sidfrstsof}[1]{\frstsof{\Sid}{#1}}

% Projection + derived sets of formulas
\newcommand{\fheapofKW}{\mathsf{heap}}
\newcommand{\fheapof}[1]{\fheapofKW(#1)}
\newcommand{\projKW}{\mathsf{project}}
\newcommand{\tproj}[1]{\projKW(#1)}
\newcommand{\ltproj}[2]{\projKW^{\Loc}(#2)}
\newcommand{\fproj}[1]{\projKW(#1)}
\newcommand{\lfproj}[2]{\projKW^{\Loc}(#2)}
\newcommand{\sfproj}[2]{\projKW(#1,#2)}

\newcommand{\USH}[1]{\USHKW_{#1}}
\newcommand{\USHKW}{\mathbf{USH}}
\newcommand{\DUSHKW}{\mathbf{DUSH}}
\newcommand{\DUSH}[1]{\DUSHKW_{#1}}
\newcommand{\DUSHx}[2]{\DUSHKW_{#1}^{#2}}

\newcommand{\FCompose}{\Compose_{\mathbf{F}}}
\newcommand{\PCompose}{\Compose_{\mathbf{P}}}
\newcommand{\euinst}[4]{#1 \xrightarrow{\eexistsSMALL #2 / \fforallSMALL #3} #4}
% \newcommand{\rescope}[2]{\mathsf{rescope}(#1, #2)}
\newcommand{\rescopeOP}{\bar{\sep}}
\newcommand{\rescope}[2]{#1 \rescopeOP #2}
\newcommand{\pinst}[3]{{#1}[#2/#3]}
\newcommand{\pinstINST}[2]{[#1/#2]}
\newcommand{\INSTxy}{\pinstINST{\vec{x}}{\vec{y}}}
\newcommand{\pinstSomeS}[2]{\pinst{#1}{\dom(#2)}{\img(#2)}}
\newcommand{\pinstS}[1]{\pinstSomeS{#1}{\S}}
\newcommand{\tinst}[4]{{#1}[#2:#3/#4]}
\newcommand{\tinstINST}[2]{[#1/#2]}
\newcommand{\AEQ}{\equiv_{\S}}
%\newcommand{\AEQ}{\equiv_{\alpha}}

% guarded quantifiers
% \newcommand{\fforall}{\forall^{\mathsf{unused}}}
%\newcommand{\eexists}{\exists^{\mathsf{used}}}
% \newcommand{\fforall}{\rotatebox[origin=c]{180}{$\mathbb{A}$}}
% \newcommand{\eexists}{\rotatebox[origin=c]{180}{$\mathbb{E}$}}
\newcommand{\fforall}{\mathord{\rotatebox[origin=c]{180}{$\mathbb{A}$}}}
\newcommand{\eexists}{\mathord{\rotatebox[origin=c]{180}{$\mathbb{E}$}}}
\newcommand{\EEX}[1]{\eexists #1\ldotp}
\newcommand{\SHEX}[1]{\exists #1\ldotp}
\newcommand{\FFA}[1]{\fforall #1\ldotp}
\newcommand{\fforallSMALL}{\mathord{\scalebox{0.5}{\rotatebox[origin=c]{180}{$\mathbb{A}$}}}}
\newcommand{\eexistsSMALL}{\mathord{\scalebox{0.5}{\rotatebox[origin=c]{180}{$\mathbb{E}$}}}}

% Proof system
\newcommand{\deriveqf}{\vartriangleright}
\newcommand{\derivestar}{\vartriangleright^{*}}
\newcommand{\rderiveqf}{\vartriangleleft}

\newcommand{\RuleId}{(id)}
\newcommand{\RuleMp}{(mp)}
\newcommand{\RuleGMp}{(gmp)}
\newcommand{\RuleMwMw}{(merge)}
\newcommand{\RuleMwTrans}{(mw-trans)}
\newcommand{\RuleEmp}{(emp)}
\newcommand{\RuleQf}{(qf)}
\newcommand{\RuleAInst}{(inst)}
\newcommand{\RuleQDrop}{(drop)}
% \newcommand{\RuleAIntro}{($\forall$-intro)}
% \newcommand{\RuleEIntro}{($\exists$-intro)}
% \newcommand{\RuleDistE}{($\exists$-dist)}
\newcommand{\RuleAIntro}{($\fforall$-intro)}
\newcommand{\RuleEIntro}{($\eexists$-intro)}
\newcommand{\RuleDistE}{($\eexists$-dist)}
%\newcommand{\RuleDistA}{($\forall$-dist)} % unsound for guarded
%quantifiers, but not needed anyway?
\newcommand{\RuleSym}{(sym)}
\newcommand{\RuleTrans}{(trans)}
\newcommand{\RuleComm}{(comm)}
\newcommand{\RuleAssoc}{(assoc)}
\newcommand{\RuleRen}{(ren)}
\newcommand{\RuleDrop}{(drop)}
\newcommand{\RuleMono}{(mono)}
\newcommand{\RuleAnti}{(anti)}
\newcommand{\RuleAdj}{(adj)}
\newcommand{\RuleEq}{(equiv)}

\newcommand{\finterface}[1]{\mathsf{interface}(#1)}
\newcommand{\ifsizeKW}{\mathsf{ifsize}}
\newcommand{\ifsize}[1]{\ifsizeKW(#1)}

% Type abstraction

\newcommand{\typeofKW}{\mathsf{type}}
\newcommand{\typeof}[2]{\typeofKW_{#1}(#2)}
\newcommand{\sidtypeof}[1]{\typeof{\Sid}{#1}}

\newcommand{\allsidtypesKW}{\mathbf{Types}}
\newcommand{\allsidtypes}[1]{\allsidtypesKW_{#1}}
\newcommand{\ssidtypes}[2]{\allsidtypesKW_{#2}^{#1}}

\newcommand{\phitypesKW}{\mathbf{Types}}
\newcommand{\phitypes}[2]{\phitypesKW^{#1}_{\Sid}(#2)}
\newcommand{\allphitypes}[1]{\phitypesKW^{#1}_{\Sid}}
\newcommand{\allxtypes}{\allphitypes{\vec{x}}}

\newcommand{\typ}{\mathcal{T}}
\newcommand{\typi}[1]{\mathcal{T}_{#1}}
\newcommand{\TypSet}{\mathbf{T}}

\newcommand{\typealloc}[1]{\mathsf{alloced}(#1)}

\newcommand{\ptrclosed}{pointer-closed}
\newcommand{\ptrpred}{\PredName{ptr}}

\newcommand{\ForgetKW}{\ensuremath{\mathsf{forget}}}
\newcommand{\Forget}[2]{\ForgetKW_{#1}(#2)}
\newcommand{\ForgetX}[1]{\Forget{\vec{x}}{#1}}
\newcommand{\ACompose}{\Compose}
\newcommand{\AForgetX}[1]{\AForget{\vec{x}}{#1}}
\newcommand{\ExtendKW}{\ensuremath{\mathsf{extend}}}
\newcommand{\Extend}[2]{\ensuremath{\ExtendKW_{#1}(#2)}}

% Examples

\newcommand{\even}{\PredName{even}}
\newcommand{\odd}{\PredName{odd}}
\newcommand{\lseg}{\PredName{lseg}}
\newcommand{\SidLs}{\Sid_{\ls}}
\newcommand{\SidTree}{\Sid_{\tree}}
\newcommand{\SidOddEven}{\Sid_{\odd/\even}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fixed-point computation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Abbreviations
\newcommand{\xx}{\vec{x}}
\newcommand{\xxfvs}[1]{\xx \cup \fvs{#1}}

% Proper new stuff
\newcommand{\PTypes}[2]{\allsidtypesKW_{\Sid}^{#1}(#2)}

% Iteration + fp functions
\newcommand{\ptypesofKW}{\mathsf{ptypes}}
% \newcommand{\ptypesof}[2]{\ptypesofKW^{#1}(#2)}
\newcommand{\ptypesof}[2]{\ptypesofKW^{\xx}_{\thefun}(#1,#2)}
\newcommand{\ptypesofgeneric}[3]{\ptypesofKW^{\xx}_{#3}(#1,#2)}
\newcommand{\thefun}{p}
\newcommand{\theop}{\mathsf{unfold}_{\xx}}
\newcommand{\fpimg}{2^{\allsidtypes{\Sid}}}
\newcommand{\thefuntype}{\Preds{\Sid} \times \EqClassesKW \to \fpimg}
\newcommand{\thelfp}{\mathsf{lfp}(\theop)}
\newcommand{\seedfun}{\lambda
  (\pred',\scls')\ldotp\emptyset}
\newcommand{\prefixi}[1]{\theop^{#1}(\seedfun)}

\newcommand{\ptrmodelKW}{\mathsf{ptrmodel}}
\newcommand{\ptrmodel}[2]{\mathsf{ptrmodel}_{#1}(#2)}

\newcommand{\goaltypes}[1]{\phitypes{\scls}{#1}}

% Top-level Types
\newcommand{\typesofKW}[1]{\mathsf{types}^{#1}}
\newcommand{\typesof}[2]{\typesofKW{#1}(#2)}
\newcommand{\ttypesofKW}{\mathsf{types}}
\newcommand{\ttypesof}[2]{\ttypesofKW(#1,#2)}
\newcommand{\typesofx}[1]{\typesofKW{\vec{x}}(#1)}

\newcommand{\extendscls}[3]{\mathsf{extend}(#1,#2=#3)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hoare logic
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\proga}{c}

\newcommand{\assn}[1]{\set{#1}}
\newcommand{\partialC}[3]{ \assn{#1} #2 \assn{#3} }
\newcommand{\deref}[1]{{^*{x}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CFG reduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CFG}{\mathbf{CFG}}
\newcommand{\Lang}[1]{\mathcal{L}(#1)}
\renewcommand{\G}{\mathbf{G}}
\newcommand{\GA}{\mathbf{G}_1}
\newcommand{\GB}{\mathbf{G}_2}
\newcommand{\NTerm}{\mathbf{N}}
\newcommand{\Term}{\mathbf{T}}
\newcommand{\NTwords}{{(\NTerm\cup\Term)}^{*}}
\newcommand{\Rules}{\mathbf{R}}
\newcommand{\Start}{\mathbf{S}}
\newcommand{\GRule}[2]{#1 \rightarrow #2}
\newcommand{\theG}{\tuple{\NTerm,\Term,\Rules,\Start}}
\newcommand{\theGi}[1]{\tuple{\NTerm_{#1},\Term,\Rules_{#1},\Start_{#1}}}

\newcommand{\RuleStep}{\Rightarrow}
\newcommand{\RuleSteps}{\Rightarrow^{+}}

% \newcommand{\cfg}{\PredName{cfg}}
% \newcommand{\cfgi}{\PredName{cfg}_i}
% \newcommand{\cfgA}{\PredName{cfg}_1}
% \newcommand{\cfgB}{\PredName{cfg}_2}
\newcommand{\cfg}{\Start}
\newcommand{\cfgi}{\Start_i}
\newcommand{\cfgA}{\Start_1}
\newcommand{\cfgB}{\Start_2}
\newcommand{\word}{\PredName{word}}
\newcommand{\wordA}{\PredName{word}_1}
\newcommand{\letter}[1]{\PredName{letter}_{#1}}
\newcommand{\wordB}{\PredName{word}_2}
\newcommand{\treeA}{\PredName{tree}_1}
\newcommand{\treeB}{\PredName{tree}_2}

\newcommand{\ForAllLetters}{1 \leq i \leq n}

\newcommand{\inducedW}[1]{\mathsf{letters}(#1)}
\newcommand{\inducedN}[2]{\mathsf{wordof}_{#1}(#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Equivalences / Heap Automaton chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\MM}{\mathbf{M}}

\newcommand{\Prop}{\mathcal{P}}

\newcommand{\Abst}{\mathcal{A}}
\newcommand{\AbstSupp}{\mathbf{A}}
\newcommand{\abstcls}{a}
\newcommand{\AbstFunKW}{\mathsf{abst}}
\newcommand{\AbstFun}[2]{\mathsf{abst}_{#1}(#2)}
\newcommand{\AbstPto}{\mathsf{abst}_\mathsf{pto}}
\newcommand{\AbstEq}{\mathsf{abst}_\mathsf{eq}}
\newcommand{\AbstComp}{\Compose}
\newcommand{\AbstInstKW}{\mathsf{instantiate}}
\newcommand{\AbstInst}[3]{\mathsf{instantiate}_{#1}(#2, #3)}
\newcommand{\AbstForgetKW}{\mathsf{forget}}
\newcommand{\AbstForget}[3]{\mathsf{forget}_{#1}(#2, #3)}
\newcommand{\AbstTuple}[1]{\tuple{#1, \AbstFunKW_{#1}, \AbstComp_{#1}, \AbstInstKW_{#1},
    \AbstForgetKW_{#1}}}
\newcommand{\CompProd}{\times}

\newcommand{\StrongSIncomp}[2]{#1 \bowtie_{\S} #2}

\newcommand{\modelsofsidKW}{\mathsf{models}}
\newcommand{\modelsofsid}[1]{\modelsofsidKW(#1)}
\newcommand{\renfuninstKW}{\mathsf{inst}}
\newcommand{\renfuninst}[2]{\mathsf{inst}_{#1}(#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sla}{\vec{v}}
\newcommand{\slb}{\vec{w}}
\newcommand{\slc}{\vec{u}}
\newcommand{\svx}{\vec{x}}
\newcommand{\svy}{\vec{y}}
\newcommand{\svz}{\vec{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SMT macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SMT sorts
%\newcommand{\sloc}{\mathsf{loc}}

% SMT Arrays
% \newcommand{\Arr}{A}
\newcommand{\Arr}{\vec{a}}
\newcommand{\Tarray}{\mathcal{T}_{\mathsf{array}}}
% array symbols
\newcommand{\aselect}[2]{#1[#2]}
\newcommand{\astoreKW}{\mathsf{store}}
\newcommand{\astore}[3]{\astoreKW(#1, #2, #3)}
\newcommand{\aKKW}{\mathbf{K}}
\newcommand{\aK}[1]{\aKKW(#1)}
\newcommand{\amapKW}{\mathsf{map}}
\newcommand{\amap}[2]{\amapKW_{#1}(#2)}
% derived array symbols
% \newcommand{\eqempty}[1]{\ensuremath{\textsf{empty}(#1)}}
\newcommand{\eqempty}[1]{#1 = \emptyset}
\newcommand{\ArraySort}[2]{\mathsf{array~#1~#2}}

% Encoding
\newcommand{\Msmt}{{\mathcal{M}_\textsc{smt}}}

\newcommand{\defineSLN}{\Delta^\Nsize_\SSL}

\newcommand{\enc}{\ensuremath{\textsf{T}_\Nsize}}       % Formula
\newcommand{\encx}{\ensuremath{\textsf{T}^x_\Nsize}}       % Formula
\newcommand{\encb}{\ensuremath{\textsf{T}^b_\Nsize}}   % Boolean
\newcommand{\encs}{\ensuremath{\textsf{T}^s_\Nsize}} % Spatial
%\newcommand{\encb}{\ensuremath{\textsf{T}^b}}   % Boolean
%\newcommand{\encs}{\ensuremath{\textsf{T}^s}} % Spatial

%\newcommand{\vecemptyset}{{\mbox{\boldmath$\emptyset$}}}
%\newcommand{\isset}{\mathsf{isset}}
%\newcommand{\parent}{\mathsf{parent}}
%\newcommand{\alloc}{\mathsf{alloc}}

% \newcommand{\btrue}{\top}
% \newcommand{\bfalse}{\bot}
\newcommand{\btrue}{\true}
\newcommand{\bfalse}{\false}

% Macros for the encoding itself
\newcommand{\Nsize}{n}
\newcommand{\FP}[1]{\vec{x}_{#1}}
% \newcommand{\GFP}{\vec{x}}
\newcommand{\GFP}{\vec{x}_{\mathsf{global}}}
\newcommand{\fsmt}{F}
\newcommand{\dsFP}{\vec{z}}
\newcommand{\rp}[1]{r^\dsFP_{#1}}
\newcommand{\rpf}{r^\dsFP_{\Nsize}}

\newcommand{\FanyDS}{\mathcal{F}_\anyDS}
\newcommand{\Fls}{\mathcal{F}_\lsDS}
\newcommand{\Ftree}{\mathcal{F}_\treeDS}
\newcommand{\FanyDSd}{\mathcal{F}_\anyDS^\sdata}
\newcommand{\Flsd}{\mathcal{F}_\lsDS^\sdata}
\newcommand{\Ftreed}{\mathcal{F}_\treeDS^\sdata}

\newcommand{\isleaf}{\mathsf{isleaf}}
\newcommand{\smtsucc}{\mathsf{succ}}
\newcommand{\defineY}{\mathsf{defineY}}
\newcommand{\smtreachability}{\mathsf{reachability}}
\newcommand{\smtfootprint}{\mathsf{footprint}}
%\newcommand{\emptyz}{\mathsf{empty}_{\dsFP}}
\newcommand{\smtstructure}{\mathsf{structure}}
\newcommand{\oneparent}{\mathsf{oneparent}}
\newcommand{\smtrootloc}{\mathsf{rootloc}}

\newcommand{\holeseq}{\mathsf{holeseq}}
\newcommand{\holesoccur}{\mathsf{holesoccur}}
\newcommand{\correctleaves}{\mathsf{correctleaves}}
\newcommand{\smtordered}{\mathsf{ordered}}
\newcommand{\fhole}[1]{\mathsf{fldhole}_{#1}}
\newcommand{\lsleafconstraints}{\mathsf{leafconstraints}^\ls}
\newcommand{\treeleafconstraints}{\mathsf{leafconstraints}^\tree}
\newcommand{\anyDSleafconstraints}{\mathsf{leafconstraints}^\anyDS}
\newcommand{\smtdata}{\mathsf{data}}
% \newcommand{\smtdataexu}{\mathsf{data}_{\exists u}}
% \newcommand{\smtdataexb}{\mathsf{data}_{\exists b}}
% \newcommand{\smtdatafau}{\mathsf{data}_{\forall u}}
% \newcommand{\smtdatafab}{\mathsf{data}_{\forall b}}
\newcommand{\smtalldata}{\mathsf{alldata}}
\newcommand{\depthtwo}{\mathsf{depth}\geq 2}



\newcommand{\Hoo}{\H_{1,1}}
\newcommand{\Hot}{\H_{1,2}}
\newcommand{\Hto}{\H_{2,1}}
\newcommand{\Htt}{\H_{2,2}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Thesis"
%%% End:

